Dynamic Graph Algorithms and Graph Sparsification: New Techniques and Connections

Graphs naturally appear in several real-world contexts including social networks, the web network, and telecommunication networks. While the analysis and the understanding of graph structures have been a central area of study in algorithm design, the rapid increase of data sets over the last decades has posed new challenges for designing efficient algorithms that process large-scale graphs. These challenges arise from two usual assumptions in classical algorithm design, namely that graphs are static and that they fit into a single machine. However, in many application domains, graphs are subject to frequent changes over time, and their massive size makes them infeasible to be stored in the memory of a single machine. Driven by the need to devise new tools for overcoming such challenges, this thesis focuses on two areas of modern algorithm design that directly deal with processing massive graphs, namely dynamic graph algorithms and graph sparsification. We develop new algorithmic techniques from both dynamic and sparsification perspective for a multitude of graph-based optimization problems which lie at the core of Spectral Graph Theory, Graph Partitioning, and Metric Embeddings. Our algorithms are faster than any previous one and design smaller sparsifiers with better (approximation) quality. More importantly, this work introduces novel reduction techniques that show unexpected connections between seemingly different areas such as dynamic graph algorithms and graph sparsification.

==> chapters/distanceminors/abstract.tex <==

%We study the following problem:
Given a graph where vertices are partitioned into $k$ terminals and non-terminals,
the goal is to compress the graph (i.e., reduce the number of non-terminals) using minor operations while preserving terminal distances approximately.
The distortion of a compressed graph is the maximum multiplicative blow-up of distances between all pairs of terminals.
We study the trade-off between the number of non-terminals and the distortion.
This problem generalizes the Steiner Point Removal (SPR) problem, in which all non-terminals must be removed.

We introduce a novel black-box reduction to convert any lower bound on distortion for the SPR problem
into a super-linear lower bound on the number of non-terminals, with the same distortion, for our problem.
%Precisely, given any graph $\Gs$ such that removing all its non-terminals will lead to a distortion of at least $\alpha$,
%we can use $\Gs$ to construct a new graph $G$ such that every minor of $G$ with distortion less than $\alpha$
%must have $\Omega(k^{1+\delta(G')})$ non-terminals, for some constant $\delta(G') > 0$.
This allows us to show that there exist graphs such that every minor with distortion less than $2$, $5/2$ and $3$
must have $\Omega(k^2)$, $\Omega(k^{5/4})$, and $\Omega(k^{6/5})$ non-terminals, respectively, plus more trade-offs in between.
The black-box reduction has an interesting consequence: if the tight lower bound on distortion for the SPR problem is super-constant,
then allowing any $\calO(k)$ non-terminals will \emph{not} help improving the lower bound to a constant.

We also build on the existing results on spanners, distance oracles and connected 0-extensions
to show a number of upper bounds for general graphs, planar graphs, graphs that exclude a fixed minor and bounded treewidth graphs.
Among others, we show that any graph admits a minor with $\calO(\log k)$ distortion and $\calO(k^{2})$ non-terminals,
and any planar graph admits a minor with $1+\epsilon$ distortion and $\tilde{O}(k^{2} \epsilon^{-2} \log^2 k)$ non-terminals.


==> chapters/distanceminors/conclusion.tex <==
\section{Conclusion}
%In this paper, we have shown a number of upper and lower bounds on the number of non-terminals needed in the minor to achieve a low distortion.
We note that there remain gaps between some of the best upper and lower bounds, e.g.,
for general graphs and distortion $3-\epsilon$, the lower bound is $\Omega(k^{6/5})$,
while for distortion $3$, our upper bound is $\calO(k^3)$.
Improving the bounds is an interesting open problem.

%For general graphs and some fixed distortion, there are still huge gaps between the best upper and lower bound on the size of the minor (see the table below). 

Our techniques for showing upper bounds rely heavily on the spanner reduction.
For planar graphs, Krauthgamer et al.~\cite{KrauthgamerNZ14} showed that to achieve distortion $1+o(1)$, $\Omega(k^2)$ non-terminals are needed;
we bypass the spanner reduction to construct an $(1+\varepsilon,\widetilde{\mathcal{O}}(k/\varepsilon)^{2})$-DAM,
which is tight up to a poly-logarithmic factor.
It is an interesting open question on whether similar guarantees can be achieved for general graphs.

==> chapters/distanceminors/introduction.tex <==
\section{Introduction}

\emph{Graph compression} generally describes a transformation of a \emph{large} graph $G$ into a \emph{smaller} graph $H$ that preserves,
either exactly or approximately, certain features (e.g., distance, cut, flow) of $G$.
Its algorithmic value is apparent, since the compressed graph can be computed in a preprocessing step of an algorithm,
so as to reduce subsequent running time and memory.
Some notable examples are graph spanners, distance oracles and cut/flow sparsifiers.

In this paper, we study compression using minor operations, which has attracted increasing attention in recent years.
Minor operations include vertex/edge deletions and edge contractions.
It is naturally motivated since it preserves certain structural properties of the original graph, e.g., any minor of a planar graph remains planar, while
reducing the size of the graph.
%, and generally the same holds for graphs that exclude a fixed minor.
We are interested in \emph{vertex sparsification}, where $G$ has a designated subset $K$ of $k$ vertices called the \emph{terminals},
and the goal is to reduce the number of non-terminals in $H$ while preserving some feature among the terminals.
Recent work in this field studied preserving cuts and flows.
%Recently, there are a number of beautiful results for the features of cuts and flows.
%\YKC{Gramoz, you will write something here about cut/flow sparsifiers (or in the related work section).}
Our focus here is on preserving terminal distances approximately in a multiplicative sense, i.e.,
we want that for any pairs of terminals $u,v \in K$, $\dist_G(u,v) \leq \dist_{H}(u,v) \leq \alpha \cdot \dist_G(u,v)$, for a small \emph{distortion} $\alpha$.
This problem, called {\em Approximate Terminal Distance Preservation (ATDP) problem}, has natural applications in
% end system
multicast routing~\cite{ChuRZ2000} and network traffic optimization~\cite{ScharfWZ2015}.
It was also suggested in~\cite{KrauthgamerNZ14} that to solve the \emph{subset travelling salesman problem},
one can compute a compressed minor with a small distortion as a preprocessing step for algorithms
that solve the travelling salesman problem for planar graphs.
%Krauthgamer et al. suggested that a compressed graph minor with a small distortion can be used as a preprocessing step
%for algorithms (which work for planar graphs or graphs excluding a fixed minor)
%that solve the \emph{subset travelling salesman problem}.% with dynamically changing subsets.

ATDP was initiated by Gupta~\cite{Gupta01}, who introduced the related {\em Steiner Point Removal (SPR) problem}:
Given a tree $G$ with both terminals and non-terminals,
output a weighted tree $G'$ {\em with terminals only} which minimizes the distortion.
Gupta gave an algorithm that achieves a distortion of $8$.
Chan et al.~\cite{ChanXKR06} observed that Gupta's algorithm returned always  a minor of $G$.
%and they showed that it is essentially the best possible, by exhibiting a sequence of trees with minimum distortion $8-o(1)$.
%On the other hand, Krauthgamer et. al.~\cite{distancepreserving} showed that by allowing $2k-2$ vertices in $G'$,
%all terminal distances can be preserved exactly, i.e., the distortion is $1$.
For general graphs, Kamma et al.~\cite{KammaKN15} gave an algorithm to construct a minor
% to construct a minor $G'$ on terminals only, i.e., $|V(G')| = |T|$, 
with distortion $\calO(\log^5 k)$. This bound has been recently improved to $O(\log^{2} k)$ by Cheung~\cite{Cheung18} and finally to $O(\log k)$ by Filtser~\cite{Filtser18}.
Krauthgamer et al.~\cite{KrauthgamerNZ14} studied ATDP and
showed that every graph has a minor with $\calO(k^4)$ non-terminals and distortion $1$.
It is then natural to ask, for different classes of graphs,
what is the trade-off between the distortion and the number of non-terminals.
In this paper, for different classes of graphs, and with respect to different allowed distortions, we provide lower and upper bounds on the number of non-terminals needed.

%\YKC{Then we define \emph{formally} our problem, and state all our results formally in the ``Preliminary'' section.}

%\smallskip

\paragraph*{Further Related Work.}

Basu and Gupta~\cite{BasuG2008} showed that for outer-planar graphs,
% (which strictly contains the class of trees, but is a proper subset of the class of planar graphs),
SPR can be solved with distortion $\calO(1)$.
When randomization is allowed, Englert et al.~\cite{EnglertGKRTT14} showed that for graphs that exclude a fixed minor,
one can construct a randomized minor  for SPR with $\calO(1)$ expected distortion.
It remains open whether similar guarantees can be obtained in the deterministic setting.
%
%Our problem generalizes the SPR problem.
Krauthgamer et al.~\cite{KrauthgamerNZ14} showed that solving ATDP with distortion $1$ for planar graphs
needs $\Omega(k^2)$ non-terminals.
%Indeed, if $G'$ is \emph{dominating} (i.e., for any two vertices $u_1,u_2$ retained in $G'$, $d_{G'}(u_1,u_2) \geq d_G(u_1,u_2)$),
%there exist planar graphs that improve the lower bound to $\Omega(k^4)$.
%Thee also showed that for graphs with bounded treewidth $p$, the two bounds are $\Omega(p|T|)$ and $\calO(p^3 |T|)$.





In the past few years, there has been a considerable amount of work on vertex sparsifiers that preserve cuts~\cite{Moitra09, leighton, charikar, mm10, EnglertGKRTT14, juliasteiner, andoni, RackeST14}. In this setting, the goal is to compress the graph only on the termials while approximately preserving all possible terminal minimum cuts. This problem is closely connected to distance sparsification, and there exist techniques to construct vertex sparsifiers for cuts using distance sparsifiers, and vice versa~\cite{Racke08, EnglertGKRTT14}. 

A related graph compression is spanners, where the objective is to reduce the number of edges by edge deletions only.
We will use a spanner algorithm (e.g.,~\cite{AlthoferDDJS93}) to derive our upper bound results for general graphs.
Although spanner operation enjoys much less freedom than minor operation,
proving a lower bound result for it is notably difficult.
Assuming the Erd\"{o}s girth conjecture~\cite{Erdos1963}, there are lower bounds that match the best known upper bounds,
but the conjecture seems far from being settled \cite{Wenger1991}.
Woodruff~\cite{Woodruff2006} showed a lower bound result bypassing the conjecture, but only for \emph{additive} spanners.

%One related graph compression problem is the spanner problem, in which only edge deletions are allowed (i.e., $G'$ is a sub-graph of $G$),
%and the objective is to preserve approximately the distance between every pair of vertices, with as few edges in $G'$ as possible.
%Indeed, we will use a spanner algorithm (e.g.,~\cite{AlthoferDDJS1993}) as a black-box to derive our upper bound results for general graphs.
%The best known spanner result is: for any integer $d\geq 1$, for any graph on $n$ vertices,
%there exists a sub-graph with $\calO(n^{1+1/d})$ edges with distortion at most $2d-1$.
%Although the sub-graph operation (which includes only edge deletion) for constructing spanner
%enjoys much less freedom than the minor operation, proving a lower bound result for spanner is notably difficult.
%Assuming the Erd\"{o}s girth conjecture~\cite{Erdos1963}, the $\calO(n^{1+1/d})$ upper bound above is tight;
%however, the conjecture is apparently far from settled, with only small cases solved
%(see~\cite{Wenger1991} and the references therein) since its birth in the 1960's.
%The other known lower bound result is given by Woodruff~\cite{Woodruff2006}, but for additive spanner.

%\smallskip

\paragraph*{Our Results.}

For various classes of graphs, we show lower and upper bounds on the number of non-terminals needed
in the minor for low distortion.
The table below summarizes our results. %(results with $\dagger$ are from \cite{distancepreserving});see the full version for a more detailed table.
%see Appendix \ref{app: discussion} for a more detailed table.
% Let $k=|T|$.
\begin{table}
\begin{center}
\begin{tabular}{l|c|c}
Graph &  Upper Bound & Lower Bound   \\ \hline
      &  (distortion, size) & (distortion, size)   \\ \hline  \hline
General &   $(2q-1,O(k^{2+2/q}))$ & $(2-\varepsilon, \Omega(k^2))$   \\
General & $-$ & $(2.5-\varepsilon, \Omega(k^{5/4}))$  \\
 &   & $(3-\varepsilon, \Omega(k^{6/5}))$ \\
 &  & \small{(see Theorem \ref{thm:lower-bound-distortion-25} for more guarantees)}    \\
B.-Treewidth $p$ &  $(2q-1,O(p^{1+2/q}k))$ &  $(1, \Omega(pk))$~\cite{KrauthgamerNZ14}    \\ 
Exc.-Fix.-Minor &  $(O(1),\tilde{O}(k^{2})$  & $-$    \\ 
Planar &  $(1+\varepsilon,\tilde{O}((k/\varepsilon)^{2})$ &  $(1+o(1), \Omega(k^{2}))$~\cite{KrauthgamerNZ14}    \\ \hline
General & $(O(\log k),0)$~\cite{Filtser18} & $-$ \\
Outerplanar & $(O(1),0)$~\cite{BasuG2008} & $-$ \\
Trees & $(8,0)$~\cite{Gupta01} & $(8-o(1),0)$~\cite{ChanXKR06} \\ \hline
General & $(O(\log k),0)$-rand~\cite{EnglertGKRTT14} & $-$ \\
Exc.-Fix.-Minor & $(O(1),0)$-rand~\cite{EnglertGKRTT14} & $(2-o(1),0)$-rand
\\
\end{tabular}
\caption{The results which are \emph{not} followed by a reference are shown in this paper.
The guarantees with the extension ``-rand'' refer to \emph{randomized} distance approximating minors;
``size'' refers to the number of non-terminals in the minor.}
\end{center}
\end{table}
For our lower bound results, we use a novel black-box reduction to convert any lower bound on distortion for the SPR problem
into a super-linear lower bound on the number of non-terminals for ATDP with the same distortion.
Precisely, we show that given any graph $G^*$ such that solving its SPR problem leads to a minimum distortion of $\alpha$,
we use $G^*$ to construct a new graph $G$ such that every minor of $G$ with distortion less than $\alpha$ must have
at least $\Omega(k^{1+\delta(\Gs)})$ non-terminals, for some constant $\delta(\Gs) > 0$.
The lower bound results in the above table are obtained by using for $G^*$ a complete ternary tree of height $2$,
which was shown that solving its SPR problem leads to minimum distortion $3$~\cite{Gupta01}.
More trade-offs are shown by using for $G^*$ a complete ternary tree of larger heights.
%similar results, with larger distortion and smaller lower bound (but still super-linear in $k$) on the number of non-terminals,
%are obtained ,
%for which its minimum distortion in SPR can be computed using the ideas of Chan et al.~\cite{chan}.

The black-box reduction has an interesting consequence.
For the SPR problem on general graphs, there is a huge gap between the best known lower and upper bounds, which are
$8$~\cite{ChanXKR06} and $\calO(\log k)$~\cite{Filtser18}; it is unclear what the asymptotically tight bound would be.
Our black-box reduction allows us to prove the following result concerning the tight bound:
for general graphs, if the tight bound on distortion for the SPR problem is super-constant,
then for any constant $c>0$, even if $ck$ non-terminals are allowed in the minor, the lower bound will remain super-constant.
See Theorem \ref{thm:spr-vs-lspr} for a formal statement of this result.

We also build on the existing results on spanners, distance oracles and connected 0-extensions to show a number of upper bound results for general graphs, planar graphs and graphs that exclude a fixed minor. Our techniques, combined with an algorithm in Krauthgamer et al.~\cite{KrauthgamerNZ14}, yield an upper bound result for graphs with bounded treewidth. In particular, our upper bound on planar graphs implies that allowing quadratic number of non-terminals, we can construct a deterministic minor with arbitrarily small distortion. %This is in contrast to minors only on the terminal, where distortion must be at least $8-o(1)$.

%The objectives of the above upper bounds results are to reduce vertices, but the minor constructed may be dense.
%For applications which want the numbers of both vertices and edges being small, simply apply spanner algorithm to the minor constructed,
%which will induce a multiplicative blow-up of the distortion, but getting a sparser minor.

==> chapters/distanceminors/lower-bound.tex <==
\section{Deterministic Lower Bounds}\label{sect:lower-bound}

For all the lower bound results, we use a tool in combinatorial design called \emph{Steiner system}
(or alternatively, \emph{balanced incomplete block design}). Let $[k]$ denote the set $\{1,2,\cdots,k\}$.

\begin{definition}
Given a ground set $K = [k]$, an $(s,2)$-Steiner system (abbr.~$(s,2)$-SS) of $K$ is a collection of $s$-subsets of $K$,
denoted by $\calT = \left\{K_1,\cdots,K_r\right\}$,
where $r = \binom{k}{2}\left/\binom{s}{2}\right.$,
such that every $2$-subset of $K$ is contained in \emph{exactly} one of the $s$-subsets.
\end{definition}

\begin{lemma}[\cite{Wilson75}]\label{lem:SSS-exist}
For any integer $s\geq 2$, there exists an integer $M_s$ such that for every $q\in\nn$,
the set $[M_s + qs(s-1)]$ admits an $(s,2)$-\emph{SS}.
\end{lemma}

Our general strategy is to use the following black-box reduction, which proceeds by taking a \emph{small} connected graph $\Gs$ as input,
and it outputs a \emph{large} graph $G$ which contains many disjoint embeddings of $\Gs$.
Here is how it exactly proceeds:
\begin{itemize}
\item Let $\Gs$ be a graph with $s\geq 2$ terminals and $q\geq 1$ non-terminals.
Let $k$ be an integer, as given in Lemma \ref{lem:SSS-exist}, such that the terminal set $K = [k]$ admits an $(s,2)$-SS $\calT$.
\item We construct $\calT' \subseteq \calT$ that satisfies \emph{certain} property depending on the specific problem.
For each $s$-set in $\calT'$, we add $q$ non-terminals to the $s$-set, which altogether form a \emph{group}.
The union of vertices in all groups is the vertex set of our graph $G$.
We note that each terminal may appear in many groups, but each non-terminal appears in one group only.
\item \emph{Within} each of the groups, we embed $\Gs$ in the natural way.%This completes the construction of $G$.
%we will often refer to this graph as $G(\calT',G')$.
\end{itemize}

The following two lemmas describe some basic properties of all minors of $G$ output by the black-box above. Before presenting their proofs, we need to introduce some helpful notation. Let $G$ be an output graph from the black-box. In any minor $H$ of $G$, we say a super-node is of Type-A if $S(u)$ contains only non-terminals in $G$;
any other super-node $u$, for which $S(u)$ contains \emph{exactly} one terminal, is of Type-B. Here are two simple facts:
\begin{enumerate}
\item[(a)] If $u$ is of Type-A, since $G[S(u)]$ is connected, the non-terminals in $S(u)$ must belong to the same group.
\item[(b)] If $u$ is of Type-B, let $t$ be the terminal in $S(u)$. If $S(u)$ contains a vertex from some group $R$, then $t\in R$.
\end{enumerate}

%Their proofs are deferred to the full version.
%Note the following simple observation: two terminals are in the same group if and only if
%there exists a group
%
%Suppose two terminals are in the same group (which is unique by definition of Steiner-system),
%
%By the definition of Steiner-system, given any pair of terminals, there is at most one group that contains both of them.
%Suppose two terminals are in the same group,
%
%Note the following simple observation: for any $G$ constructed using the black-box reduction,
%two terminals are in the same group if and only if there is a simple path connecting the two terminals that contains no other terminal.

\begin{lemma}\label{lem:unique-group-for-edge}
Let $H$ be a minor of $G$. Then for each edge $(u_1,u_2)$ in $H$, there exists exactly one group $R$ in $G$
such that $S(u_1)\cap R$ and $S(u_2)\cap R$ are both non-empty.
\end{lemma}
\begin{proof}
Existence of $R$ is easy to prove by a simple induction on the minor operation sequence that generates $H$ from $G$.
To show the uniqueness, we proceed to a case analysis.
In the first case, either $u_1$ or $u_2$ is of Type-A. Then the uniqueness is trivial by fact (a).

In the second case, both $u_1,u_2$ are of Type-B. For $i=1,2$, let $v_i$ be the terminal in $S(u_i)$.
Suppose there are two groups $R_a,R_b$ that intersect both $S(u_1)$ and $S(u_2)$.
Then by fact (b), $v_1,v_2$ are in both $R_a$ and $R_b$, a contradiction.
\end{proof}
The above lemma permits us to legitimately define the notion $R$-edge:
an edge $(u_1,u_2)$ in $H$ is an $R$-edge if $R$ is the unique group that intersects both $S(u_1)$ and $S(u_2)$.

\begin{lemma}\label{lem:interchange-at-terminal}
Suppose that in a minor $H$ of $G$,
$(u_1,u_2)$ is a $R_1$-edge and $(u_2,u_3)$ is $R_2$-edge, where $R_1\neq R_2$.
Then $R_1$ and $R_2$ intersect, and $S(u_2)$ contains the terminal in $R_1\cap R_2$.
\end{lemma}
\begin{proof}
Since $S(u_2)$ contains vertices from both $R_1$ and $R_2$, $u_2$ must be of Type-B, i.e., $S(u_2)$ contains exactly one terminal $v$.
By fact (b), $v$ is in both $R_1$ and $R_2$.
\end{proof}

We will show that for any minor $H$ with low distortion, at least one of the non-terminals in each group must be retained,
and thus $H$ must have at least $|\calT '|$ non-terminals.
We first present some of our main theorems on lower bounds and then prove them;
two more theorems are given in Section \ref{subsect:full-general}.

\begin{theorem} \label{thm:lower-bound-star}
For infinitely many $k\in \nn$, there exists a bipartite graph with $k$ terminals
which does not have a $(2-\epsilon,k^2/7)$-\emph{DAM}, for all $\epsilon > 0$.
\end{theorem}

\begin{theorem}\label{thm:lower-bound-distortion-25}
There exists a constant $c_1 > 0$, such that for infinitely many $k\in \nn$,
there exists a quasi-bipartite graph with $k$ terminals
which does not have an $(\alpha-\epsilon,c_1 k^\gamma)$-\emph{DAM}, for all $\epsilon>0$,
where $\alpha,\gamma$ are given in the table below.

\begin{center}
\begin{tabular}{c|c|c|c|c|c|c|c}
$\alpha$ & $2.5$ & $3$ & $10/3$ & $11/3$ & $4$ & $4.2$ & $4.4$ \\
\hline
$\gamma$ & $5/4$ & $6/5$ & $10/9$ & $11/10$ & $12/11$ & $21/20$ & $22/21$\\
\end{tabular}
\end{center}
\end{theorem}

%\begin{theorem} \label{thm:rand-lower-bound-star}
%For infinitely many $k\in \nn$, there exists a bipartite graph with $k$ terminals
%which does not have a $\left(2-\epsilon, \epsilon^3 k^2 / 150\right)$-\emph{rDAM}, for any $1\geq \epsilon>0$.
%%\YKC{There should be an upper bound for the admissible $\epsilon$. For instance, it surely cannot be greater than $1$.
%%And indeed, since in Lemma \ref{lm: randomGupta}, when $k=3$, the lower bound is $4/3$, so $\epsilon$ should not much greater than $2/3$.}
%\end{theorem}

%For our concrete results, $\Gs$ is a tree, which allows us to apply the lower bound results on distortion for SPR problem on trees~\cite{gupta01,chan}.
%We note that in our construction, there is no edge across two different groups, i.e., the endpoints of each edge in $G$ must belong to the same group.

\subsection{Distortion $2$ Lower Bound}

\begin{figure}[t]
\centering
\begin{minipage}{.3\textwidth}
  \centering
\begin{tikzpicture}
\tikzstyle{vertex}=[circle, fill=white, draw = black, minimum size = 6pt, inner sep=2pt]
\tikzstyle{vertex1}=[fill = white, draw = white]

\tikzstyle{edge}=[-,thick ]
\tikzstyle{elipse}=[-,thick ]
	
  \node[vertex] (n1) at (0,0) {$1$} ;
  \node[vertex] (n2) at (3,0)  {$6$} ;
  \node[vertex] (n3) at (1.5,3)  {$2$} ;
  \draw[edge] (n1) -- (n2) ;
  \draw[edge] (n2) -- (n3) ;
  \draw[edge] (n3) -- (n1) ;
  \draw[elipse] (1.5,0.92) ellipse (0.91 and 0.91) ;
  \node[vertex] (n4) at (1.5,0) {$5$};
  \node[vertex] (n5) at (0.7,1.35) {$4$};
  \node[vertex] (n6) at (2.3,1.35) {$7$};
  

  \draw[edge] (n3) -- (n4) ;
  \draw[edge] (n2) -- (n5) ;
  \draw[edge] (n1) -- (n6) ;
  \node[vertex] (n7) at (1.5,0.9)  {$3$} ;

  
 
\end{tikzpicture}
\end{minipage}%
\begin{minipage}{.65\textwidth}
  \centering
\begin{tikzpicture}
\tikzstyle{vertex}=[circle,draw = white, fill=black, minimum size = 8pt, inner sep=2pt]
\tikzstyle{vertex1}=[fill = white, draw = white]

\tikzstyle{edge}=[-,thick]
\tikzstyle{edge1}=[-,thick, gray]
\tikzstyle{vertex2}=[thick, draw = black, fill = gray!30, line width = 0.3mm] 
 
  \node[vertex] (n1) at (0,0) {} ;
  \node[vertex] (n2) at (1.25,0) {} ;
  \node[vertex] (n3) at (2.5,0) {} ;
  \node[vertex] (n4) at (3.75,0) {} ;
  \node[vertex] (n5) at (5,0) {};
  \node[vertex] (n6) at (6.25,0) {};
  \node[vertex] (n7) at (7.5,0) {} ;
  
  \node[vertex2] (n124) at (0,2) {} ;
  \node[vertex2] (n235) at (1.25,2) {} ;
  \node[vertex2] (n346) at (2.5,2) {} ;
  \node[vertex2] (n457) at (3.75,2) {} ;
  \node[vertex2] (n561) at (5,2) {} ;
  \node[vertex2] (n672) at (6.25,2) {} ;
  \node[vertex2] (n713) at (7.5,2) {} ;
  
  \draw[edge] (n124) -- (n1) node[below = 2.5pt] {$1$};
  \draw[edge] (n124) -- (n2) node[below = 2.5pt] {$2$};
  \draw[edge] (n124) -- (n4) node[below = 2.5pt] {$4$};
  
  \draw[edge] (n235) -- (n2) ;
  \draw[edge] (n235) -- (n3) node[below = 2.5pt] {$3$};
  \draw[edge] (n235) -- (n5) node[below = 2.5pt] {$5$};
  
  \draw[edge] (n346) -- (n3) ;
  \draw[edge] (n346) -- (n4) ;
  \draw[edge] (n346) -- (n6) node[below = 2.5pt] {$6$};
  
  \draw[edge] (n457) -- (n4) ;
  \draw[edge] (n457) -- (n5) ;
  \draw[edge] (n457) -- (n7) node[below = 2.5pt] {$7$};
  
  \draw[edge] (n561) -- (n5) ;
  \draw[edge] (n561) -- (n6) ;
  \draw[edge] (n561) -- (n1) ;
  
  \draw[edge] (n672) -- (n6) ;
  \draw[edge] (n672) -- (n7) ;
  \draw[edge] (n672) -- (n2) ;
  
  \draw[edge] (n713) -- (n7) ;
  \draw[edge] (n713) -- (n1) ;
  \draw[edge] (n713) -- (n3) ;
\end{tikzpicture}
\end{minipage}
\caption{On the left side: a Fano plane corresponding to a $(3,2)$-SS with $k=7$. On the right side: the bipartite graph of the Fano plane constructed using our black-box reduction. Numbered vertices are \emph{terminals} while square-shaped vertices are \emph{non-terminals}.}
\end{figure}

We next prove Theorem \ref{thm:lower-bound-star}. Let us start by reviewing the lower bound for SPR problem on stars due to Gupta~\cite{Gupta01}.
 
\begin{lemma}\label{lm: gupta1}
Let $\Gs = (K \cup \{v\}, E)$ be an unweighted star with $k \geq 3$ terminals, in which $v$ is the center of the star.
Then, every edge-weighted graph only on the terminals $K$ with fewer than $\binom{k}{2}$ edges has distortion at least $2$.
\end{lemma}

We construct $G$ using the black-box reduction above. Let $k\in\nn$ be such that the terminals $K=[k]$ admits a $(3,2)$-SS, denoted by $\calT$ (see the figure above).
Here, we set $\calT' = \calT$ and $\Gs$ to be the star with $3$ terminals, as described in Lemma \ref{lm: gupta1}.

By the definition of Steiner system, the shortest path between every pair of terminal $u,v$ in $G$ is unique,
which is the $2$-hop path within the group that contains both terminals, i.e., $\dist_G(u,v) = 2$ for all $u,v \in K$.
Every other simple path between $u,v$ must pass through an extra terminal, so the length of such simple path is at least $4$.


%Further, we can alternatively view $G$ as a concatenation of unweighted stars on the terminals, where every $T_i$ forms a star with $n_i$ being the center and connected to $3$ leaves corresponding to the terminals from $T_i$. 

%We associate $\calT$ with a bipartite graph $G=(V,E,\ell)$ which we define below. 
%\begin{itemize}
%\item We set $V = T \cup N$, where $T$ is the terminal set and $N = \{n_1,\ldots,n_r\}$ is the set of non-terminal vertices corresponding to each $T_i \in \calT$, $i=1,\ldots,r$. 
%\item For $n_i \in N$ and $t_j \in T_i$, where $i = 1,\ldots,r$ and $j = 1,2,3$, we add $(n_i,t_j)$ to $E$. We define $G$ to be unweighted, i.e. $\ell_1 = 1$, for all $e \in E$. 
%\end{itemize}

Let $H$ be a minor of $G$. Suppose that the number of non-terminals in $H$ is less than $r$, then there exists a group $R$ in which
its non-terminal is not retained (which means that it is either deleted, or contracted into a terminal in that group).
By Lemma \ref{lm: gupta1}, there exists a pair of terminals in that group
such that every simple path within $R$ (which means a path comprising of $R$-edges only) between the two terminals has length at least $4$.
And every other simple path must pass through an extra terminal (just as in $G$), so again it has length at least $4$.
Thus, the distortion of the two terminals is at least $2$.

Therefore, every $(2-\epsilon)$-DAM of $G$ must have $r > k^{2}/7$ non-terminals.

%Let $H$ be a minor of $G$ with at most $r$ non-terminals. Depending on the number of non-terminals in $H$, we distinguish the following cases.
%
%If the number of non-terminals in $H$ is exactly $r$, then the only minor operations performed on $G$ were edge deletions (this follows since every non-terminal in $G$ lies in some terminal shortest paths). Since $H$ is a non-trivial minor, at least one edge deletions from $G$ must have occurred. Let $e = (n_i,t_j)$ denote such an edge. We will show that $d_H(t_j,t_k) \geq 4$ for some $t_k \in T_i$, thus implying that distortion is of $H$ at least $2$.  
%
%To this end, fix an assignment of edge lengths $\ell'$ in $H$ and consider the terminal pair $(t_j,t_k)$ as defined above. By definition of Steiner-system and construction of $H$, every shortest path between $t_j$ and $t_k$ in $H$ uses at least $4$ edges. Further, by the 2-hop path property of the remaining terminal pairs in $H$, each such shortest path is a concatenation of exactly two terminal shortest paths that share some terminal $t_l$. Since all terminal distances must be dominating in $H$, i.e. $d_H(t_j, t_l) \geq 2$ and  $d_H(t_l,t_h) \geq 2$, we get that $\ell'$ must assigns lengths of at least $1$ to all the edges belonging to these shortest paths. Thus, $d_H(t_j,t_k) \geq 4$, as desired.  
%
%If $H$ contains fewer than $r$ non-terminals, then in any sequence of minor operations performed on $G$, some vertex deletion or edge contraction must have occurred. If a vertex deletion was performed, then in a similar way to the edge deletion case, one can show that there exists at least one terminal pair whose shortest path is at least $4$ in $H$, thus giving a distortion of at least $2$ for $H$. If an edge contraction was performed, then we invoke Lemma \ref{lm: gupta1} to the star whose edge was contracted (note that the lemma can be invoked independently to every star, since non-terminals of $G$ form an independent set). Since contracting an edge of a star gives another star lying only on the terminals with $2$ edges, Lemma \ref{lm: gupta1} shows that distortion of $H$ is at least $2$. 
%
%Combining all the above cases, we get that for every $\epsilon > 0$, graph $G$ does not admit a non-trivial distance approximating minor of size less than $\binom{k}{2}/3 + k > k^{2}/6$ and distortion $2-\epsilon$.

%---------------------------%


\subsection{Higher Distortion Lower Bounds}
We now prove Theorem \ref{thm:lower-bound-distortion-25}. Concretely, we will give the proof for the case $\alpha = 2.5$ here, and discuss how to generalize this proof for other distortions.
We will first define the notions of \emph{detouring graph} and \emph{detouring cycle},
and then use them to construct the graph $G$ that allows us to show the lower bound.

\paragraph*{Detouring Graph and Detouring Cycle.}
For any $s\geq 3$, let $k\in\nn$ be such that the terminal set $K = [k]$ admits an $(s,2)$-SS.
Let $\calT = \{K_1,\cdots,K_r\}$ be such an $(s,2)$-SS.
%; recall that $r = \binom{k}{2}\left/\binom{s}{2}\right. \sim \frac{k^2}{s(s-1)}$.
A \emph{detouring graph} has the vertex set $\calT$.
By the definition of Steiner system, $\left|K_i\cap K_j\right|$ is either zero or one.
In the detouring graph, $K_i$ is adjacent to $K_j$ if and only if $\left|K_i\cap K_j\right| = 1$.
Thus, in the detouring graph, it is legitimate to give each edge $(K_i,K_j)$ a \emph{terminal label}, which is the terminal in $K_i\cap K_j$.
A \emph{detouring cycle} is a cycle in the detouring graph such that no two neighboring edges of the cycle have the same terminal label.

\begin{fact} Suppose that two edges in the detouring graph have a common vertex,
and their terminal labels are different, denoted by $u,v$.
Then the common vertex must be an $s$-set in $\calT$ containing both $u,v$.
By the definition of Steiner system, the $s$-set is uniquely determined.
\end{fact}

%Next, we define a \emph{detouring cycle}. $T_{a_1},T_{a_2},\cdots,T_{a_\ell},T_{a_{\ell+1}} = T_{a_1}$ form a detouring cycle of size $\ell\geq 3$
%if the followings hold: (i) they form a cycle of size $\ell$ in the detouring graph; and
%(ii) for each two neighboring vertices $T_{a_i},T_{a_{i+1}}$ in the cycle,
%suppose the edge connecting them is labelled by the terminal in $T_{a_i} \cap T_{a_{i+1}}$,
%then no two adjacent edges in the cycle are labelled by the same terminal.
%\begin{enumerate}
%\item[(i)] They form a cycle of size $\ell$ in the detouring graph.
%\item[(ii)] For each two neighboring vertices $T_{a_i},T_{a_{i+1}}$ in the cycle,
%suppose the edge connecting them is labelled by the terminal in $T_{a_i} \cap T_{a_{i+1}}$.
%Then no two adjacent edges in the cycle are labelled by the same terminal.
%\end{enumerate}

\begin{claim}\label{claim:no-dcycle}
In the detouring graph, number of detouring cycles of size $\ell\geq 3$ is at most $k^\ell$.
\end{claim}

\begin{proof}
Let $(u_1,\cdots,u_\ell)$ be an $\ell$-tuple, where each entry is a terminal, that represents the terminal labels of a detouring cycle.
By the Fact above, the $\ell$-tuple determines uniquely all the vertices in the detouring cycle.
By trivial counting, the number of possible $\ell$-tuples is at most $k^\ell$,
and hence also the number of detouring cycles of size $\ell$.
\end{proof}

%For each possible labelling on the edges as defined in (ii),
%the two terminal labels on any two adjacent edges determine uniquely their common adjacent vertex in the detouring cycle,
%which is the unique set in $\calT$ that contains both labels.
%Thus, for each such possible labelling, there is \emph{at most} one detouring cycle of size $\ell$.
%As there can be at most $k^\ell$ possible labellings, the number of detouring cycles is at most $k^\ell$.

Our key lemma is shows that for any $L\geq 3$, we can retain $\Omega_s(k^{L/(L-1)})$ vertices in the detouring graph,
such that the induced graph on these vertices has \emph{no} detouring cycle of size $L$ or less.

\begin{lemma}\label{lem:large-detouring-graph}
For any integer $L\geq 3$, given a detouring graph with vertex set $\calT = \{K_1,\cdots,K_r\}$,
there exists a subset $\calT '\subset \calT$ of cardinality $\Omega_{s}(k^{L/(L-1)})$
such that the induced graph on $\calT '$ has no detouring cycle of size $L$ or less.
\end{lemma}

\begin{proof}
%Firstly, we note that $|r| = \binom{k}{2} \left/ \binom{q}{2} \right. \sim \frac{k^2}{q(q-1)}$.
We choose the subset $\calT '$ by the following randomized algorithm:
\begin{enumerate}
\item Each vertex is picked into $\calT '$ with probability $\delta k^{-(L-2)/(L-1)}$, where $\delta = \delta(s) < 1$ is a positive constant
which we will derive explicitly later.
\item While (there is a detouring cycle of size $L$ or less in the induced graph of $\calT '$)\\
\hspace*{0.3in}Remove a vertex in the detouring cycle from $\calT '$
\end{enumerate}

After Step 1, $\expect{|\calT '|} = r \cdot \delta k^{-(L-2)/(L-1)} \ge \frac{\delta}{2s(s-1)} k^{L/(L-1)}$.
Using Claim \ref{claim:no-dcycle}, the expected number of detouring cycles of size $L$ or less is at most
$$\sum_{\ell=3}^L k^\ell \cdot (\delta k^{-(L-2)/(L-1)})^\ell \leq 2 \delta^3 k^{L/(L-1)}.$$
Thus, the expected number of vertices removed in Step 2 is at most $2 \delta^3 k^{L/(L-1)}$.
Now, choose $\delta = 1/\sqrt{8s(s-1)}$. By the end of the algorithm,
$$\expect{|\calT '|} \geq \frac{\delta}{2s(s-1)} k^{L/(L-1)} - 2 \delta^3 k^{L/(L-1)} = \Omega(k^{L/(L-1)}).\vspace*{-0.2in}$$
\end{proof}

\paragraph*{Construction of $G$ and the proof.}
Recall the black-box reduction.
Let $k$ be an integer such that $K=[k]$ admits a $(9,2)$-SS $\calT$.
By Lemma \ref{lem:large-detouring-graph}, we choose $\calT '$ to be a subset of $\calT$ with $|\calT'| = \Omega(k^{5/4})$,
such that the induced graph on $\calT '$ has no detouring cycle of size $5$ or less.
We choose $\Gs$ to be a complete ternary tree of height $2$, in which the $9$ leaves are the terminals.
For each $K_i\in \calT '$, we add four non-terminals to $K_i$, altogether forming a \emph{group}.

The following lemma is a direct consequence that the induced graph on $\calT'$ has no detouring cycle of size $5$ or less.

\begin{lemma}\label{lem:types-of-simple-paths}
For any two terminals $u,v$ in the same group, let $R$ denote the group.
Then, in any minor $H$ of $G$, every simple path from $u$ to $v$ either comprises of $R$-edges only,
or it comprises of edges from at least $5$ groups other than $R$.
\end{lemma}

%\begin{proof}
%Consider a simple path from $t$ to $u$ in $H$, which comprises of at least one edge from a group other than $R$.
%Let $R_1,\cdots,R_q$ be the groups that contribute an edge to the simple path, and for $i=1,\codts,q$,
%let $e_i$ be the first $R_i$-edge that appears in the simple path, in the direction from $t$ to $u$.
%By Lemma \ref{lem:interchange-at-terminal}

%Walking through the edges in the simple path from $t$ to $u$, suppose that $R_1,\cdots,R_q$ are the groups 


%not, i.e., there exists a simple path from $t$ to $u$ which comprises of edges from at most $4$ groups,
%and at least one of such groups is not $R$.
%Let $R_1,\cdots,R_q$ denote such groups, in the order of when their edges appear in the path from $t$ to $u$.
%\end{proof}

%We claim that if a minor of the desired graph has distortion $<2.5$, then in each group there exists at least one Steiner point.

%We prove the above claim by contradiction. Suppose in contrary, there exists a group with all Steiner points removed.
%By what we already knew about the ternary tree, there exists a pair of terminals $\{u,v\}$ in the group such that its distance \emph{within the group}
%is three times its original distance in the desired graph.

%We next show that any other simple path between $u$ and $v$ has length at least $12$. \YKC{The argument below is very rough and for myself currently;
%I will improve the writing later.}

%All other simple paths must pass through other groups. Note that by construction, there is no backtrack (the simple path visits a group twice).
%Since the desired graph has girth $\geq 7$, so the simple path must passes through $6$ other groups,
%and thus it must passes through at least $6$ other terminals.
%So the simple path has length $\geq 12$.

\begin{proof}[Proof of Theorem~\ref{thm:lower-bound-distortion-25}]
Let $H$ be a $(2.5-\epsilon)$-DAM of $G$, for some $\epsilon>0$.
Suppose that there exists a group such that all its non-terminals are not retained in $H$.
By \cite{Gupta01}, there exists a pair of terminals $u,v$ in that group such that
every simple path between $u$ and $v$, which comprises of edges of that group only, has length at least $3 \cdot \dist_G(u,v)$.

By Lemma \ref{lem:types-of-simple-paths} and Lemma \ref{lem:interchange-at-terminal},
any other simple path $P$ between $u$ and $v$ passes through at least $4$ other terminals,
say they are $u_a,u_b,u_c,u_d$ in the order of the direction from $u$ to $v$.
We denote this path by $P := u\ra u_a\ra u_b\ra u_c\ra u_d\ra v$, by ignoring the non-terminals along the path.
Between every pair of consecutive terminals in $P$, the length is at least $2$.
Thus, the length of $P$ is at least $10$.
Since $\dist_G(u,v)\leq 4$, the length of $P$ is at least $2.5 \cdot \dist_G(u,v)$.

Thus, the length of \emph{every} simple path from $u$ to $v$ in $H$ is at least $2.5\cdot \dist_G(u,v)$, a contradiction.
Therefore, at least one non-terminal in each group is retained in $H$. As there are $\Omega(k^{5/4})$ groups, we are done.
\end{proof}

For the other results in Theorem \ref{thm:lower-bound-distortion-25},
we follow the above proof almost exactly, with the following modifications.
Set $s=3^h$ for some $h\geq 2$, and set $\Gs$ to be a complete ternary tree with height $h$, in which the leaves are the terminals.
Let $\alpha_h$ be a lower bound on the distortion for the SPR problem on $\Gs$.
Apply Lemma \ref{lem:large-detouring-graph} with some integer $h < L \leq \lceil\alpha_h h\rceil$.\footnote{Any choice of $L$
larger than $\lceil\alpha_h h\rceil$ will not improve the result.}
Following the above proof, attaining a distortion of $\min\left\{\frac{L}{h},\alpha_h\right\}-\epsilon$ needs $\Omega(k^{L/(L-1)})$ non-terminals.

The last puzzle we need is the values of $\alpha_h$.
Chan et al.~\cite{ChanXKR06} considered unweighted complete binary tree with height $h$, and showed that as $h$ tends to infinity, the minimum distortion of SPR problem tends to $8$. However, it is not clear from their proof how the minimum distortion depends on $h$,
which is needed for Theorem \ref{thm:lower-bound-distortion-25}.
In what follows, we use their ideas on unweighted complete ternary trees to derive such a dependence.

\newcommand{\drl}{\text{\textsf{DRL}}}
\newcommand{\calS}{\mathcal{S}}

Let $T_h$ denote a unweighted complete ternary tree of height $h$, where the leaves are the terminals.
Let $\calS_h$ denote the collection of all minors of $T_h$.
For each of its node $u$, let $T(u)$ denote the sub-tree rooted at $u$, and let $t(u)$ denote the terminal which $u$ contracts into.
Denote the root by $r$, and its three children by $x,y,z$.
Without loss of generality, we assume that $r$ is contracted into a terminal $t_r$ in $T(x)$, i.e., $t(r) = t_r$.
Then, let\footnote{Formally speaking,
there can be infinitely many minors (with weights) of $T_h$ with distortion at most $\alpha$,
so we should use $\inf$ instead of $\min$ in the definition.
Yet, for each fixed minor without weight, the standard restriction~\cite[Definition 1.3]{KammaKN15} is the optimal weight assignment.
Since there are only finitely many minors of $T_h$ (without weights), we can replace $\inf$ by $\min$.}
$$\drl(h,\alpha) := \min_{H\in \calS_h,\text{ distortion }\leq \alpha}~~\max_{\text{terminal }t\in T(y)\cup T(z)}~~\dist_H(t_r,t).$$
If there is not such a minor $H$, then $\drl(h,\alpha) = +\infty$ by default.
Note that when $\alpha$ increases, $\drl(h,\alpha)$ decreases.


%\begin{figure}
%\begin{center}
%\includegraphics[width=\textwidth]{chapters/distanceminors/figure_tree.pdf}
%\input{chapters/distanceminors/figure_tree.pdf_tex}
%\caption{The definitions of nodes in $T_h$. The blue polygon includes all nodes in $S(t_r) = S(r) = S(w)$.}
%\label{fig:tree}
%\end{center}
%\end{figure}


Let $H\in\calS_h$ be a minor of $T_h$ with distortion $\leq \alpha$.
Let $w$ denote a deepest node in $T(y)\cup T(z)\cup \{r\}$ such that $t(w) = t_r$.
Let $\ell$ be the distance between $r$ and $w$ in $T_h$.
Let $w_1,w_2$ be two children of $w$ which are not in $T(x)$.
%See Figure \ref{fig:tree} above for a picture of all the above definitions.

Then, by the definition of $\drl$, there exist two terminals $t_1\in T(w_1)$ and $t_2\in T(w_2)$ such that for $i=1,2$,
$\dist_H(t_i,t(w_i)) \geq \drl(h-\ell-1,\alpha)$.
Also, for $i=1,2$, $\dist_H(t(w_i),t_r) \geq \dist_{T_h}(t(w_i),t_r) = 2h$.
Hence,
\begin{align*}
	\dist_H(t_1,t_2) & =  \dist_H(t_1,t(w_1)) + \dist_H(t(w_1),t_r) + \dist_H(t_r,t(w_2)) \\ 
	& \quad + \dist_H(t(w_2),t_2)  \\
	& \geq  2\left[\drl(h-\ell-1,\alpha) + 2h\right] .
\end{align*}


%$$d_H(t_1,t_2) = d_H(t_1,t(w_1)) + d_H(t(w_1),t_r) + d_H(t_r,t(w_2)) + d_H(t(w_2),t_2) \geq 2\left[\drl(h-\ell-1,\alpha) + 2h\right].$$

Recall that $\dist_{T_h}(t_1,t_2) = 2(h-\ell)$.
Hence, the distortion w.r.t.~$t_1,t_2$ is at least
$$\frac{\drl(h-\ell-1,\alpha) + 2h}{h-\ell}.$$
This quantity cannot be larger than $\alpha$.

We are ready to give a recurrence relation that bounds $\drl(h,\alpha)$ from below:
\begin{equation}\label{eq:drl-recur}
\drl(h,\alpha) \geq \min_{\ell\in [0,h-1]:~\frac{\drl(h-\ell-1,\alpha) + 2h}{h-\ell} \leq \alpha} \drl(h-\ell-1,\alpha) + 2h,
\end{equation}
while the initial conditions are: $\forall \alpha\geq 1,~\drl(0,\alpha) = 0$, and
$$\drl(1,\alpha) =
\begin{cases}
+\infty, & \text{if }\alpha < 2;\\
2, & \text{if }\alpha \geq 2.
\end{cases}$$

Let $\alpha_h$ denote the minimum distortion of $T_h$.
By letting $\ell$ run over all possible distances between $r$ and $w$, we obtain the following lower bound on $\alpha_h$:
\begin{equation}\label{eq:alpha-recur}
\alpha_h \geq \min_\alpha~~\max\left\{\alpha , \left(\min_{\ell\in [0,h-1]} \frac{\drl(h-\ell-1,\alpha) + 2h}{h-\ell}\right)\right\}.
\end{equation}

We compute the lower bounds in \eqref{eq:drl-recur} and \eqref{eq:alpha-recur} using math software.
In the table below, we give the lower bounds on $\alpha_h$ for $h\in [3,10]$ and $h=1000$.

\smallskip

%By a simple induction using the recurrence \eqref{eq:drl-recur}, it is easy to prove that
%$$Z(\alpha) := \min_{\ell\in [0,h-1]} \frac{\drl(h-\ell-1,\alpha) + 2h}{h-\ell}$$
%is always a rational number (if not infinity),
%and all discontinuous points of $Z(\alpha)$ are rational numbers. Also, when $\alpha$ increases, $Z(\alpha)$ decreases.
%So the lower bound on $\alpha_h$ can be computed by bisection method up to some sufficiently small precision,
%and then round the approximate solution to a rational number, which is the \emph{exact} value of the lower bound.
%We give a few lower bounds on $\alpha_h$ in the table below.
\begin{center}
\begin{tabular}{c|c|c|c|c|c|c|c}
$h$ & 2 & 3,4 & 5 & 6,7 & 8 & 9,10 & 1000\\
\hline
$\alpha_h$ & 3 & 4 & $22/5$ & $14/3$ & 5 & $26/5 $ & $257/35$\\
\end{tabular}
\end{center}


%but they did not give explicit values of $\alpha_h$.
%We apply their ideas to complete ternary tree of height $h$, to obtain explicit values for $h\leq 5$,
%which are used to prove all the results in Theorem \ref{thm:lower-bound-distortion-25}.
%The explicit values are $\alpha_2 = 3$, $\alpha_3 = \alpha_4 = 4$ and $\alpha_5 = 4.4$.
%We discuss the details for computing these values in Appendix \ref{app:explicit-tree-value}.
%We discuss the details for computing these values in the full version.
%\begin{tabular}{|c||c|c|c|}
%\hline
%$\mathbf{h}$ & 2 & 3,4 & 5\\
%\hline
%$\mathbf{\alpha_h}$ & 3 & 4 & $4.4$\\
%\hline
%\end{tabular}

%The above proof can be generalized to yield the lower bounds in Table , with a few simple modifications.
%In \cite{placeholder}, they showed that for a ternary tree of height $h\geq 2$,
%in which the $3^h$ leaves are terminals and all the internal nodes are non-terminals,
%any terminal-preserving minor of the tree with all Steiner points removed must have distortion of at least $\alpha_h = something$.
%
%We consider $(3^h,2)$-SS on the terminals, and then construct a detouring graph with no detouring cycle of size $L$ or less,
%where $2\alpha_{h-1} h \leq L \leq 2\alpha_h h$.
%With such modifications, we then follow the above proof closely to show that there exists a graph $G$ with $k$ terminals
%which does not have a deterministic $\left(\frac{L}{2h}-\epsilon,c_4 k^{L/(L-1)}\right)$-DAM.

\subsection{Generalizing the Lower Bound and its Implication}

Indeed, we can set $\Gs$ as \emph{any} graph.
In our above proofs we used a tree for $\Gs$  because the only known lower bounds on distortion for the SPR problem are for trees.
If one can find a graph $\Gs$ (either by a mathematical proof, or by computer searches)
such that its distortion for the SPR problem is at least $\alpha$,
applying the black-box reduction with this $\Gs$, and  reusing the above proof show that
there exists a graph $G$ with $k$ terminals such that attaining a distortion of $\alpha-\epsilon$
needs $\Omega(k^{1+\delta(\Gs)})$ non-terminals, for some $\delta(\Gs) > 0$.

%Indeed, the graph within each group can be \emph{anything}, not necessarily a tree. Here is the result in full generality:
%Suppose there exists a graph with $q$ terminals and at least one non-terminal, such that its Steiner Point Removal problem has distortion at least $\alpha$,
\begin{theorem}\label{thm:lower-bound-superlinear}
Let $\Gs$ be a graph with $s$ terminals, and the distance between any two terminals is between $1$ and $\beta$.
Suppose the distortion for the \emph{SPR} problem on $\Gs$ is at least $\alpha$.
Then, for any positive integer $\max\{2,\lceil\beta\rceil\} \leq L\leq \left\lceil \alpha\beta \right\rceil$,
there exists a constant $c_4 := c_4(s) > 0$, such that for infinitely many $k\in \nn$,
there exists a graph with $k$ terminals which does not have a
$\left(\min\left\{L/\beta,\alpha\right\}-\epsilon,c_4 k^{L/(L-1)}\right)$-\emph{DAM}, for all $\epsilon>0$.
\end{theorem}

The above theorem has an interesting consequence. For the SPR problem on general graphs, the best known lower bound is $8$,
while the best known upper bound is $\calO(\log k)$~\cite{Filtser18}.
There is a huge gap between the two bounds, and it is not clear where the tight bound locates in between.
Suppose that the tight lower bound on SPR is super-constant.
Then for any positive constant $\alpha$, there exists a graph $\Gs_\alpha$ with $s(\alpha)$ terminals and some non-terminals, such that the distortion is larger than $\alpha$.
By Theorem \ref{thm:lower-bound-superlinear}, $\Gs_\alpha$ can be used to construct a family of graphs with $k$ terminals,
such that to attain distortion $\alpha$, the number of non-terminals needed is super-linear in $k$.
Recall that in SPR, no non-terminal can be retained. In other words, Theorem \ref{thm:lower-bound-superlinear} implies that:
\emph{if retaining no non-terminal will lead to a super-constant lower bound on distortion,
then having the power of retaining any linear number of non-terminals will not improve the lower bound to a constant}.

\newcommand{\lspr}{\text{\textsf{LSPR}}}

Formally, we define the following generalization of SPR problem.
Let $\lspr_y$ denote the problem that for an input graph with $k$ terminals,
find a DAM with at most $yk$ non-terminals so as to minimize the distortion;
the SPR problem is equivalent to $\lspr_0$.
\begin{theorem}\label{thm:spr-vs-lspr}
For general graphs, \emph{SPR} has super-constant lower bound on distortion
if and only if for any constant $y\geq 0$, \emph{$\lspr_y$} has super-constant lower bound on distortion.
\end{theorem}

%\newpage

%\subsection*{Proof of Theorem \ref{thm:lower-bound-clumping}}
%
%\newcommand{\cover}{\text{\textsf{Cov}}}
%\newcommand{\PP}[1]{\mathbb{P}\left[#1\right]}
%
%There are a rich number of literature that studies the power of compressing a graph via sub-graph operations (i.e., by performing edge and/or vertex deletions).
%The main focus of this paper is about minor operations, which are more powerful than sub-graph operations, since it also allows edge contraction.
%In this section, we would like to understand the strength of an even more powerful operation, which we call it \emph{clumping}.
%Briefly speaking, clumping operations have all the abilities of minor operations, and in addition,
%it allows contraction between two non-terminals even if there is no edge between them.
%For any graph $G$, a graph that can be yielded by performing clumping operations on $G$ is called a \emph{clump}.
%\YKC{motivation, either in intro, or here}
%
%Our main technical result in this section is that, even with the more powerful clumping operations, there exists graphs $G$ with $k$ terminals,
%such that any $(2-\epsilon)$-DP clump of $G$ has $\Omega(k^{2-\delta})$ vertices, for some small constant $\delta > 0$.
%Indeed, we will be using graph instances similar to those for proving Theorems \ref{thm:lower-bound-star} and \ref{thm:lower-bound-distortion-25},
%and all these graph instances are bipartite graphs.
%
%
%\begin{theorem}\label{thm:lower-bound-clumping}
%\YKC{The ``clumping'' result.}
%\end{theorem}
%
%\newcommand{\calP}{\mathcal{P}}
%\renewcommand{\dh}[1]{d_H(#1,w)}
%
%Given an integer $k$ such that the set $T = \{1,2,\cdots,k\}$ has a $(3,2)$-SS,
%let $\calT = \{T_1,T_2,\cdots,T_r\}$ be explicitly such a $(3,2)$-SS.
%Our aim is to select a \emph{large} subset $\calT' \subset \calT$ such that \emph{any clumping of two non-terminals will lead to a bad distortion}.
%
%As a simple example, we discuss why $\calT'$ cannot be $\calT$.
%Suppose $\calT' = \calT$, then the distance between every pair of terminals is exactly $2$.
%We can clump all the non-terminals together into a single vertex $w$, and the clump formed will be a star with center vertex $w$.
%Then, by setting the length of each edge between $w$ and a terminal to be $1$, the clump has only one non-terminal, and its distortion is $1$.
%
%To see what property $\calT'$ needs to satisfy for achieving our aim, we first focus on two groups $T_k,T_\ell\in \calT'$,
%and let their terminals be $t_1,t_2,t_3$ and $u_1,u_2,u_3$ respectively.
%We say that any other group $T_r\in\calT$ with $|T_r\cap (T_k\cup T_\ell)| = 2$ is a \emph{cover} of $T_k,T_\ell$,
%and let $\cover(T_k,T_\ell)$ denote the collection of all covers of $T_k,T_\ell$.
%
%Suppose that there exists two sets in $\cover(T_k,T_\ell)$ which are NOT in $\calT'$.
%In other words, there exists two pairs $(t_i,u_j)$ and $(t_q,u_r)$ such that $d_G(t_i,u_j)\geq 4$ and $d_G(t_q,u_r)\geq 4$.
%Then, suppose that the non-terminals in $G_1$ and $G_2$ are clumped into $w$.
%There are two cases that we will discuss. In the discussion below, we will focus \emph{locally} on the two groups, i.e.,
%we do not consider any simple paths that pass through other groups;
%as we will see later, such paths are always too long so it is safe to ignore them.
%
%\noindent\textbf{Case 1: $t_i\neq t_q$ and $u_j\neq u_r$.}\\
%Then we must have the followings: $\dh{t_i} + \dh{u_j} \geq 4$ and $\dh{t_q} + \dh{u_r} \geq 4$.
%Hence, either $\dh{t_i} + \dh{t_q} \geq 4$, or $\dh{u_j} + \dh{u_r} \geq 4$;
%WLOG, suppose the former inequality holds. Note that $d_G(t_i,t_q) = 2$, so this pair has distortion of at least $2$.
%
%\noindent\textbf{Case 2: otherwise; WLOG, assume that $t_i = t_q$.}\\
%WLOG, say $t_i = t_3$. Then we must have the followings: $\dh{t_3} + \dh{u_j} \geq 4$ and $\dh{t_3} + \dh{u_r} \geq 4$.
%Let $z := \dh{u_j} + \dh{u_r}$. If $z \geq \frac{10}{3}$, since $d_G(u_j,u_r) = 2$, this pair has distortion of at least $\frac 53$.
%If $z < \frac{10}{3}$, then at least one of $\dh{u_j},\dh{u_r}$ is less than $\frac 53$, which then forces $\dh{t_3} > \frac 73$.
%On the other hand, note that $\dh{t_1} + \dh{t_2} \geq 2$, hence one of $\dh{t_1},\dh{t_2}$ is at least $1$, say $\dh{t_1}$.
%Then $\dh{t_1} + \dh{t_3} \geq \frac{10}{3}$, but $d_G(t_1,t_3) = 2$, so this pair has distortion of at least $\frac 53$.
%
%Thus, we require that $\calT'$ to satisfy the following property:
%
%\begin{enumerate}[leftmargin=2.2cm]
%\item[Property $\calP$.] For any $T_k,T_\ell \in \calT'$, $\left|\cover(T_k,T_\ell) \cap (\calT\setminus \calT')\right| \geq 2$,
%i.e., at least two of the covers of $T_k,T_\ell$ are not in $\calT'$.
%\end{enumerate}
%
%\begin{lemma}
%There exists $\calT '\subset \cal T$ such that $\calT '$ satisfies Property $\calP$ and $|\calT '| = \Omega(k^{7/4})$.
%\end{lemma}
%
%
%\begin{pf}
%%To start, we introduce the following notion. For any $T_k,T_\ell \in \calT$, let $\cover(T_k,T_\ell)$ denote
%%the collection of all covers of $T_k,T_\ell$.
%%$$\cover(T_k,T_\ell) := \left\{ T_r\in \calT ~\left| ~T_r\neq T_k,~T_r\neq T_\ell~\text{and}~|(T_k\cup T_\ell) \cap T_{r_j}| = 2 \right. \right\}.$$
%%In other words, if $T_k,T_\ell\in \calT'$, to satisfy Property $\calP$, only two sets in $\cover(T_k,T_\ell)$ is allowed to be in $\calT '$;
%If $T_k,T_\ell\in \calT'$ and if $\left|\cover(T_k,T_\ell) \cap (\calT\setminus \calT')\right| \leq 1$,
%we say that $T_k,T_\ell$ \emph{violate} Property $\calP$.
%
%We choose the subset $\calT'$ by the following randomized algorithm, and we will show that $\expect{|\calT '|} = \Omega(k^{7/4})$:
%\begin{enumerate}
%\item Each $T'\in \calT$ is added to $\calT'$ with probability $\delta k^{-1/4}$, where $1 \geq \delta >0$ is a sufficiently small positive constant.
%\item While (there exists $T_k,T_\ell\in calT'$ that violate Property $\calP$)\\
%\hspace*{0.3in}Remove two sets in  $\cover(T_k,T_\ell) \cap \calT'$ from $\calT'$.
%\end{enumerate}
%
%Note that if $T_k$ and $T_\ell$ are disjoint, then $|\cover(T_k,T_\ell)| = 9$.
%Thus, the probability that $T_k,T_\ell$ violate Property $\calP$ is
%\begin{align*}
%& \PP{T_k\in \calT'}\cdot \PP{T_\ell\in \calT'} \cdot \PP{\text{at least eight sets in }\cover(T_k,T_\ell)\text{ is added to }\calT')}\\
%\leq & \delta k^{-1/4} \cdot \delta k^{-1/4} \cdot 9 (\delta k^{-1/4})^8 = 9 \delta^{10} k^{-5/2};
%\end{align*}
%the inequality holds due to a simple union bound.
%Observe that there are $\calO(k^4)$ choices of disjoint $T_k,T_\ell$,
%so the expected number of sets removed from $\calT'$ in Step 2 is at most
%$2 \cdot \calO(k^4) \cdot 9 \delta^{10} k^{-5/2} = \calO(\delta^{10} k^{3/2})$.
%
%If $T_k$ and $T_\ell$ are not disjoint, then then $|\cover(T_k,T_\ell)| = 4$.
%Then, by an argument similar to the last paragraph, we show that
%the probability that $T_k,T_\ell$ violate Property $\calP$ is at most $4 \delta^5 k^{-5/4}$.
%Observe that there are $\calO(k^3)$ choices of $T_k,T_\ell$ that are not disjoint,
%so the expected number of sets removed from $\calT'$ in Step 2 is at most $2 \cdot \calO(k^3) \cdot 4 \delta^5 k^{-5/4} = \calO(\delta^5 k^{7/4})$.
%\end{pf}
%
%\YKC{Formal proof about the graph distortion here.}
%
%\begin{pfof}{Theorem \ref{thm:lower-bound-clumping}}
%Let $H$ be a clump of $G$. For any two terminals $t_1,t_2$ in the same group $T\in\calT'$, consider a path which is not in the group,
%i.e., a path that consists of a vertex $v$ such that $f^{-1}(v)\cap G(T)$ is empty.
%\end{pfof}

%Now, I construct a graph, which I call it ``\emph{helping graph}'' $\calH$, which has its vertex set $\calG$.
%For any $G,G'\in \calG$, they are adjacent in $\calH$ if and only if $G\cap G' \neq \emptyset$.

%By a simple counting argument, we know that for any $G\in \calG$, its degree in $\calH$ is
%$$9\left(\frac{k-1}{8} - 1\right) \sim \frac{9}{8} k.$$

%It is not difficult to see that the diameter of $\calH$ is $2$ \footnote{I don't believe this is relevant, but I put it down just in case we need it.},
%and the girth of $\calH$ is $3$.
%I want to remove vertices from $\calH$ (and hence also all edges adjacent to these vertices),
%such that the resultant graph will have girth $6$; this is my \emph{desired graph}.

%We use the following algorithm to construct a \emph{desired graph}:

%Then we estimate how many vertices are removed by repeating Step 2.
%In expectation, for $\ell=3,4,5,6$, the number of cycles with length $\ell$ which is retained after Step 1 is at most
%$$\O(k^\ell) \cdot (\delta k^{-4/5})^\ell = \delta^\ell \cdot \O(k^{\ell/5}) \leq \delta^3 \cdot \O(k^{6/5}).$$
%Hence, in expectation, there number of cycles with length $\leq 6$ which is retained after Step 1 is at most
%$$4\cdot \delta^3 \cdot \O(k^{6/5}) = \delta^3 \cdot \O(k^{6/5}).$$

%Thus, in expectation, the number of vertices retained at the end of the algorithm is at least
%$$\frac{\delta}{72} k^{6/5} - \delta^3 \cdot \O(k^{6/5}).$$
%By setting $\delta$ to be sufficiently small, this is $\Omega(k^{6/5})$.
%And by the construction of the algorithm, the girth of the resultant graph is at least $7$, i.e.,
%any cycle in the resultant graph has length at least $7$, thus \emph{desired}.


==> chapters/distanceminors/preliminary.tex <==
\section{Preliminaries}

Let $G=(V,E,\ww)$ denote an undirected graph with terminal set $K \subset V$ of cardinality $k$,
where $\ww: E \ra \rr^+$ is the weight~(length) function over edges $E$. %For any $(u,v) \in V(G)$, let $\dist_G(u,v)$ denote the the shortest path distance between $u$ and $v$ in $G$. 
A graph $H$ is a \emph{minor} of $G$ if $H$ can be obtained from $G$ by performing a sequence of vertex/edge deletions and edge contractions,
but no terminal can be deleted, and no two terminals can be contracted together.
In other words, all terminals in $G$ must be \emph{preserved} in $H$.

Besides the above standard description of minor operations,
there is another equivalent way to construct a minor $H$ from $G$~\cite{KammaKN15},
which will be more convenient for presenting some of our results.
A partial partition of $V(G)$ is a collection of pairwise disjoint subsets of $V(G)$ (but their union can be a proper subset of $V(G)$).
Let $S_1,\cdots,S_m$ be a partial partition of $V(G)$ such that (1) each induced graph $G[S_i]$ is connected,
(2) each terminal belongs to exactly one of these partial partitions, and (3) no two terminals belong to the same partial partition.
Contract the vertices in each $S_i$ into one single ``super-node'' in $H$.
For any vertex $u\in V(G)$, let $S(u)$ denote the partial partition that contains $u$;
for any super-node $u\in V(H)$, let $S(u)$ denote the partial partition that is contracted into $u$.
In $H$, super-nodes $u_1,u_2$ are adjacent \emph{only if} there exists an edge in $G$ with one of its endpoints in $S(u_1)$ and the other in $S(u_2)$.
We denote the super-node that contains terminal $u$ by $u$ as well.

\begin{definition}
The graph $H=(V',E',\ww')$ is an $\alpha$-distance approximating minor (abbr.~$\alpha$\emph{-DAM}) of $G=(V,E,\ww)$
if $H$ is a minor of $G$ and for any $u,v \in K$,  $\dist_G(u,v) \leq \dist_H(u,v) \leq \alpha \cdot \dist_G(u,v)$.
$H$ is an $(\alpha,y)$\emph{-DAM} of $G$ if $H$ is an $\alpha$\emph{-DAM} of $G$ with at most $y$ non-terminals.%,
%i.e., $|V'\setminus T| \leq y$.
%A class of graphs $\mathcal{G}$ is $(\alpha,f(k))$-distance-approximating-compressible (abbr.~$(\alpha,f(k))$-DAC)
%if for any graph $G\in \mathcal{G}$ with $k$ terminals, $G$ has an $(\alpha,f(k))$-DAM.
\end{definition}

We note that the SPR problem is equivalent to finding an $(\alpha,0)$-DAM.
One can also define a randomized version of distance approximating minor:

\newcommand{\calD}{\eta}

\begin{definition}
Let $\calD$ be a probability distribution over minors of $G=(V,E,\ww)$.
We call $\calD$  an $\alpha$-randomized distance approximating minor (abbr.~$\alpha$\emph{-rDAM}) of $G$
if for any $u,v \in K$,
 \[ \mathbb{E}_{H\sim\calD}\left[\dist_H(u,v)\right] \leq \alpha \cdot \dist_G(u,v), \]
and for every minor $H$ in the support of $\calD$, $\dist_H(u,v) \geq \dist_G(u,v)$.
Furthermore, we call $\calD$ an $(\alpha,y)$\emph{-rDAM} if $\calD$ is an $\alpha$\emph{-rDAM} of $G$,
and every minor in the support of $\calD$ has at most $y$ non-terminals.
%A class of graphs $\mathcal{G}$ is $(\alpha,f(k))$-randomized distance approximating compressible (abbr.~$(\alpha,f(k))$-rDAC)
%if for any graph $G\in \mathcal{G}$ with $k$ terminals, $G$ has an $(\alpha,f(k))$-rDAM.
\end{definition}

%Kamma et al.~\cite{KammaKN2015} showed that for any graph, it's always possible to solve the SPR problem with $\alpha = \calO(\log^5 k)$.
%For tree graphs, Gupta~\cite{gupta01} gave an algorithm that solves the SPR problem with $\alpha=8$,
%and he exhibited a family of trees for which the SPR problem cannot be solved with any $\alpha < 4$.
%Chan et al.~\cite{chan} showed that Gupta's algorithm is essentially best,
%by exhibiting another family of trees for which the SPR problem cannot be solved with any $\alpha < 8$.
%
%It is known that the class of general graphs is $(1,\calO(k^4))$-DAC~\cite{distancepreserving}.
%For some restricted classes of graphs, the number of non-terminals needed can be much less than $\calO(k^4)$;
%for instance, the class of tree graphs is $(1,2k-2)$-DAC~\cite{distancepreserving}.

%\YKC{Discuss how this result was obtained, and state the generalized result that
%if we sample $L$ shortest paths, then after minor operations, at most $2\cdot \binom{L}{2}$ Steiner points.}

==> chapters/distanceminors/upper-bound-excluding-minor.tex <==
\section{Minor Construction for Fixed Minor-Free Graphs}
In this section we give improved guarantees for distance approximating minors for special families of graphs. Specifically, we show that graphs that exclude a fixed minor admit an $(O(1),\tilde{O}(k^{2}))$-DAM. This family of graphs includes, among others, planar graphs. 

The reduction to spanner in Section \ref{sect:UB-general} does not consider the structure of $Q_K$, which is inherited from the input graph.
We exploit this structure by employing the randomized Steiner Point Removal Problem, which is equivalent to finding an $(\alpha, 0)$-rDAM. Let us start by reviewing the following result of Englert et al.~\cite{EnglertGKRTT14},
which shows that for graphs that exclude a fixed minor, there exists a randomized minor with constant distortion.
\begin{theorem}[\cite{EnglertGKRTT14}, Theorem 14]
\label{thm2}
Let $\alpha = \calO(1)$. Given a graph that excludes a fixed minor $G = (V,E, \ww)$ with $K \subset V$,
there is a probability distribution $\calD$ over minors $H = (K,E', \ww')$ of $G$,
such that for all $u,v$ in $K$, $\mathbb{E}_{H\sim\calD} [\dist_H(u,v)] \leq \alpha \cdot \dist_G(u,v)$ and for every minor $H$ in the support of $\calD$, $\dist_H(u,v) \geq \dist_G(u,v)$.
\end{theorem}

Given a graph $G$ that excludes a fixed minor, any minor $H$ of $G$ only on the terminals also excludes the same fixed minor. Thus $H$ has $\calO(k)$ edges~\cite{Thomason1984}. This leads to the corollary below.

\begin{corollary}
\label{cor1} Let $\alpha = \calO(1)$. Given a graph that excludes a fixed minor $G = (V,E, \ww)$ with $K \subset V$ and $Q_K$ previously defined,
there exists a probability distribution $\calD$ over subgraphs $H=(K,E', \ww')$ of $Q_K$, each having at most $O(k)$ edges, such that for all
$u,v$ in $K$, $\mathbb{E}_{H\sim\calD}[\dist_H(u,v)] \leq \alpha \cdot \dist_{Q_K}(u,v)$.
%\begin{equation} \label{eq}
%	\forall \; t,v \in T, \quads \mathbb{E}_{H\sim\calD}[d_H(t,v)] \leq \alpha \cdot d_{Q_K}(t,v).
%\end{equation}
\end{corollary}
\begin{proof}
Let $\calD$ be the distribution over minors of $G$ from Theorem \ref{thm2}, then every minor in its support is clearly a subgraph of $Q_K$ with $\calO(k)$ edges. Since during the construction of these minors we may assume that for all $(u,v)$ in E'$,~\ww'(u,v) = \dist_G(u,v)$, the corollary follows.
\end{proof}

\begin{lemma} \label{lemma: planar 1}
Given a graph that excludes a fixed minor $G = (V,E, \ww)$ with $K \subset V$, and $Q_K$ as previously defined, there exists an $\calO(1)$-spanner $S$ of size $O (k \log k)$ for $Q_K$.
\end{lemma}
\begin{proof}
Let $\calD$ be the probability distribution over subgraphs $H$ from Corollary \ref{cor1}. Set $S = \emptyset$.
First, we sample independently $q = 3 \log k$ subgraphs $H_1, \ldots, H_q$ from $\calD$.
We then add the edges from all these subgraphs to the graph $S$, i.e., $E_S = \bigcup_{i=1}^{q} E_{H_i}$.
Fix an edge $(t,t')$ from $Q_K$ and a subgraph $H_i$. By Corollary \ref{cor1} and the Markov inequality,
$\mathbb{P} [\dist_{H_i}(u,v) \geq 2 \alpha \cdot \dist_{Q_K}(u,v)] \leq  2^{-1}$, and hence
%The later implies that, for any edge $(u,v)$ from $Q_K$
\begin{align*}
	\mathbb{P}[\dist_{S}(u,v) \geq 2 \alpha \cdot & d_{Q_K}(u,v)] \\
	&  = \prod_{i=1}^{q} \mathbb{P}[\dist_{H_i}(u,v) \geq 2 \alpha \cdot d_{Q_K}(t,t')]  \leq 2^{-q} = k^{-3}.
\end{align*}
Applying union bound overall all edges from $Q_K$ yields
$$
	\mathbb{P}[\exists (u,v) \in E(Q_K) \text{ with } \dist_{S}(u,v) \geq 2\alpha \cdot \dist_{Q_K}(u,v)] \leq k^{2} \cdot k^{-3} = k^{-1}.
$$
Hence, for all edges $(u,v)$ from $Q_K$, with probability at least $1 - 1/k$, we preserve the shortest path distance between $u$ and $v$
up to a factor of $2 \alpha = \calO(1)$ in $S$. Since $S$ is a subgraph of $Q_K$, this implies that there exists a $\calO(1)$-spanner $S$ of size $\calO(k \log k)$ for $Q_K$.
\end{proof}
Similar to the last section, the set of shortest paths corresponding to edges of $S$ is an $(\calO(1), \calO(k \log k))$-TPc  $\mathcal{P}'$ of $G$.
Using  $\mathcal{P}'$ with Lemma \ref{lemma: branching} gives the following theorem.
\begin{theorem}
Any graph that excludes a fixed minor $G = (V,E, \ww)$ with $K \subset V$ admits an $(O (1),\tilde{O} (k^{2}))$-\emph{DAM}.
\end{theorem}


==> chapters/distanceminors/upper-bound-general.tex <==
\section{Minor Construction for General Graphs}\label{sect:UB-general}
In this section we give  minor constructions that present numerous trade-offs between the distortion and size of DAMs.
Our results are obtained by combining the work of Coppersmith and Elkin~\cite{CoppersmithE06} on sourcewise distance preservers with the well-known notion of spanners.% (see \cite{AlthoferDDJS1993}).

Given an undirected graph $G=(V,E, \ww)$, we let $\pi_{u,v}$ denote the shortest path  between $u$ and $v$ in $G$.
Without loss of generality, we assume that for any pair of vertices $(u,v)$, the shortest path connecting $u$ and $v$ is \textit{unique}.
This can be achieved by slightly perturbing the original edge lengths of $G$ such that no paths have exactly the same length (see \cite{CoppersmithE06}). The perturbation implies a \emph{consistent} tie-breaking scheme: whenever $\pi$ is chosen as the shortest path, every subpath of $\pi$ is also chosen as the shortest path.

Let $N_G(u)$ denote the vertices incident to $u$ in a graph $G$. We say that two paths $\pi$ and $\pi'$ branch at a vertex $u \in V(\pi) \cap V(\pi')$ iff $|N_{\pi \cup \pi'}(u)| > 2$. We call such a vertex $u$ a \textit{branching} vertex.
Let $\mathcal{P}$ denote the set of shortest paths corresponding to every pair of vertices in $G$. 
We review the following result proved in \cite[Lemma 7.5]{CoppersmithE06}. 
\begin{lemma} \label{lemma: elkin} 
%Let $G$ be a graph with consistent tie-breaking scheme among shortest paths.
%Then,
Any pair of shortest paths $\pi, \pi' \in \mathcal{P}$ has at most \emph{two} branching vertices.
\end{lemma}

To simplify our exposition, we introduce the notion of \emph{terminal path covers}.

\begin{definition}[Terminal Path Cover] Given $G = (V,E, \ww)$ with terminals $K$, a set of shortest paths $\mathcal{P}' \subset \mathcal{P}$ is an $(\alpha, f(k))$-terminal path cover (abbr.~$(\alpha, f(k))$-TPc) of $G$ with respect to $K$ if
\begin{enumerate} 
\item $\mathcal{P}'$ covers the terminals, i.e. $K \subseteq V(H)$, where $H = \bigcup_{\pi \in \mathcal{P}'} E(\pi)$, 
\item  $|\mathcal{P}'| \leq f(k)$ and for all $u,v \in K$, $\dist_G(u,v) \leq \dist_H (u,v) \leq \alpha \cdot \dist_G(u,v)$.
\end{enumerate}
\end{definition}
We remark that the endpoints of the shortest paths in $\mathcal{P}'$ are not necessarily terminals. The above definition naturally leads to the following algorithm, which is a slight generalization of the upper-bound technique employed by Krauthgamer et al.~\cite{KrauthgamerNZ14}.

\begin{algorithm2e}
\label{algo: minor}
\caption{\textsc{MinorSparsifier}$(G,K,\mathcal{P}')$}
\Input{Graph $G=(V,E,\ww)$, terminals $K$, $(\alpha, f(k))$-TPc $\mathcal{P'}$ of $G$}
\Output{Distance Approximating Minor $H$ of $G$}
 Set $H = \emptyset$ \;
 Add all shortest paths from the path cover $\mathcal{P}'$ to $H$ \;
 
 \While{there exists a degree two non-terminal $v$ incident to edges $(v,u)$ and $(v,w)$} { 
 Contract the edge $(u,v)$ \;
 Set the length of the edge $(u,w)$ to $\dist_G(u,w)$ \;
}
 \Return $H$

\end{algorithm2e}

The following lemma gives an upper bound on the size of the DAM output by Algorithm \ref{algo: minor}. It is an easy generalization of a lemma in \cite[Lemma 2.2]{KrauthgamerNZ14} and we review it here for the sake completeness.

\begin{lemma} \label{lemma: branching}
For a given graph $G = (V,E, \ww)$ with terminals $K \subset V$ and an $(\alpha,f(k))$-\emph{TPc} $\mathcal{P}'$ of $G$, \textsc{MinorSparsifier($G$,$T$,$\mathcal{P}'$)} outputs an $(\alpha,f(k)^2)$-\emph{DAM} of $G$. 
\end{lemma}
\begin{proof}
First, it is clear that the union over paths of $\mathcal{P}' \subset \mathcal{P}$ is a minor of $G$ (this can be alternatively viewed as deleting non-terminals and edges that do not participate in any of the shortest paths in $\mathcal{P}'$). Further, the algorithm performs only edge contractions. Thus, the produced graph $H$ is a minor of $G$. 

Since contracting edges incident to non-terminals of degree two does not affect any distance in $H$, the distortion guarantee follows directly from that of the cover $\mathcal{P}'$. Thus, it only remains to show the bound on the size of $H$.

To this end, consider any two paths $\pi, \pi'$ from $\mathcal{P}'$. From Lemma \ref{lemma: elkin}, we know that $\pi$ and $\pi'$ branch in at most two vertices. Let $u_1$ and $u_2$ denote such vertices. Due to the tie-breaking scheme in $G$, we know that the shortest path $\pi_{u_1,u_2}$ is unique, and thus it must be shared by both $\pi$ and $\pi'$. The latter implies that every vertex in the subpath must have degree degree exactly $2$. Therefore, the only non-terminals in $\pi \cup \pi'$ are vertices $u_1$ and $u_2$, since non-terminals of degree two are removed from the edge contractions performed in the algorithm. 

There are $O (f(k)^2)$ pairs of shortest paths from $\mathcal{P}'$, each having at most $2$ non-terminals. Hence, the number of non-terminals in $H$ is $O (f(k)^2)$.
\end{proof}

A trivial \textit{exact} terminal path cover for any $k$-terminal graph is to take the union of all terminal shortest paths,
which we refer to as the $(1,\calO(k^{2}))$-TPc $\mathcal{P}'$ of $G$.
Krauthgamer et al.~\cite{KrauthgamerNZ14} used this $(1,\calO(k^{2}))$-TPc to construct an $(1,O(k^{4}))$-DAM.
Here, we study the question of whether increasing the distortion slightly allows us to obtain a cover of size $o(k^2)$.
We answer this question positively, by reducing it to the well-known spanner problem.

Let $q \geq 1$ be an integer and let $G = (V,E,\ww)$ be an undirected graph. A $q$-spanner of $G$ is a subgraph $S = (V,E_S, \ww)$ such that
for all $u,v$ in $V$, $\dist_G(u,v) \leq \dist_S(u,v) \leq q \cdot \dist_G(u,v)$. We refer to $q$ and $|E_S|$ as the \textit{stretch} and \textit{size} of spanner $S$, respectively. It is well-known that a simply greedy algorithm achieves the following guarantees.
\begin{lemma}[\cite{AlthoferDDJS93}] \label{lemma: spanner}
Let $q \geq 1$ be an integer. Any graph $G = (V,E,\ww)$ admits a $(2q-1)$-spanner $S$ of size $O(|V|^{1+1/q})$.
\end{lemma}

We use the above lemma as follows. Given a graph $G=(V,E,\ww)$ with terminals $K$, we compute the complete graph $Q_K = (K,\binom{K}{2},d_G|K)$, where $d_G|K$ denotes the distance metric of $G$ restricted to the point set $K$ (In other words, for any pair of terminals $u,v \in K$, the weight of the edge connecting them in $Q_K$ is given by $w_{Q_K}(u,v) = d_G(u,v)$). Recall that all shortest paths in $G$ are unique.

Using Lemma \ref{lemma: spanner}, we construct a $(2q-1)$-spanner $S$ of size $O (k^{1+1/q})$ for $Q_K$. Observe that each edge of $S$ corresponds to a unique (terminal) shortest path in $G$ since $S$ is a subgraph of $Q_K$. Thus, the set of shortest paths corresponding to edges of $S$ form a $(2q-1, O (k^{1+1/q}))$-TPc $\mathcal{P}'$ of $G$. Using $\mathcal{P}'$ with Lemma \ref{lemma: branching} gives the following theorem.

\begin{theorem}
Let $q \geq 1$ an integer. Any graph $G=(V,E,\ww)$ with $K \subset V$ admits a $(2q-1,O (k^{2+2/q}))$-\emph{DAM}.
\end{theorem}
We mention two trade-offs from the above theorem. When $q=2$, we get an $(3,O (k^3))$-DAM. When $q=\log k$, we get an $(O(\log k),O(k^2))$-DAM. The above method allows us to have improved guarantees for bounded treewidth graphs. In particular, we prove that any graph $G$ with treewidth at \sloppy most $p$ admits an $(O(\log p),O(p k))$-DAM.

\begin{theorem}\label{thm:treewidth}
Let $q \geq 1$ be an integer. Any graph $G=(V,E,\ww)$ with treewidth at most $p$, terminals $K \subset V$ and $k \geq p$
admits a $(2q-1,O(p^{1+2/q} k))$-\emph{DAM}.
\end{theorem}
\begin{proof}
We crucially exploit the fact that such graphs admit small separators:
given a graph $G$ of bounded treewidth $p$ and any nonnegative vertex weight function $w(\cdot)$, there exists a set $S \subset V(G)$ of at most $p+1$ vertices
whose removal separates the graph into two connected components, $G_1$ and $G_2$, each with $w(V(G_i)) \leq 2/3 w(V(G))$ (see \cite{bodlaender95}).

Krauthgamer et al.~\cite{KrauthgamerNZ14} use the above fact to construct an $(1, \mathcal{O}(p^{3}k))$-DAM for graphs of treewidth at most $p$.
We show that with two modifications, their algorithm can be extended to constructing distance approximating minors. The first modification is Step 2 of the algorithm \textsc{ReduceGraphTW} in \cite{KrauthgamerNZ14}.
For any integer $q\geq 1$, we replace their call to \textsc{ReduceGraphNaive}$(H,K \cup B)$\footnote{We remark that they use $R$ to denote the set of terminals.}
by our procedure \textsc{MinorSparsifier}$(H,K \cup B, \mathcal{P}')$, where $ \mathcal{P}'$ is a $(2q-1, \mathcal{O}(p^{1+1/q}))$-TPc of $G$.

The second modification is a generalization of Lemma 4.2 in \cite{KrauthgamerNZ14}. The main idea is to use the small separator set $S$ to decompose the graph into smaller almost-disjoint graphs $G_1$ and $G_2$, compute their DAMs recursively, and then combine them using the separator $S$ into a DAM of $G$. This implies that the separator $S$ must belong to each $G_i$, i.e. all non-terminal vertices of $S$ must be counted as additional terminals in each $G_i$. Below we give a formal definition of this decomposition/composition process.
%The small separator set $S$ allows us to decompose $G$ into two smaller graphs, which we can work on recursively, and at the end we \emph{knit} them with the separator vertices. It is not hard to see that if the smaller graphs have distortions $\alpha_1,\alpha_2$, then after the knitting, the distortion is at most $\max\{\alpha_1,\alpha_2\}$.

%The main idea lies in decomposing the graph into smaller networks, say $G_1$ and $G_2$, computing independently minors for such graphs, and then combining the minors back into a minor of $G$. 
Let $G_1 = (V_1, E_1, \ww_1)$ and $G_2 = (V_2,E_2, \ww_2)$ be graphs on disjoint sets of non-terminals, having terminal sets $K_1 = \{s_1,s_2,\ldots,s_{a_1}\}$ and $K_2 = \{t_1,t_2,\ldots,t_{a_2}\}$, respectively. Further, let $\phi(s_i)=t_i$, for all $i=1,\ldots,c$ be an one-to-one correspondence between some subset of $K_1$ and $K_2$ (this correspondence is among the separator vertices). The \textit{$\phi$-merge} (or $2$-sum) of $G_1$ and $G_2$ is the graph $G = (V,E,\ww)$ with terminal set $K = K_1 \cup \{t_{c+1},\ldots,t_{a_2}\}$ formed by identifying the terminals $s_i$ and $t_i$, for all $i=1,\ldots,c$, where $\ww(e) = \min\{\ww_1(e),\ww_2(e)\}$ (assuming infinite length when $\ww_i(e)$ is undefined). We denote this operation by $ G := G_1 \oplus_{\phi} G_2$.

Below we state the main lemma whose proof goes along the lines of \cite[Lemma 4.2]{KrauthgamerNZ14}.

\begin{lemma} Let $G = G_1 \oplus_{\phi} G_2$. For $j=\{1,2\}$, let $H_j$ be an $(\alpha_j,f(a_j))$-\emph{DAM} for $G_j$. Then the graph $H = H_1 \oplus_{\phi} H_2$ is an $(\max\{\alpha_1,\alpha_2\}, f(a_1) + f(a_2))$-\emph{DAM} of G.  
\end{lemma}

In~\cite{KrauthgamerNZ14} it is shown that the size of the minor returned by the algorithm \textsc{ReduceGraphTW} is bounded by the number of leaves the in the recursion tree of the algorithm. Further, they prove that there are at most $\calO(k/p)$ such leaves. Plugging our bounds from the modification of Step 2 along with the above lemma yields our claimed result.
\end{proof}
%We defer the proof of the above theorem to the full version. 
%We defer the proof of the above theorem to Appendix \ref{app:treewidth}. 



%\medskip
%
%\noindent\textbf{Extension to Bounded Treewidth Graphs.~}
%Next, we present better guarantees for bounded treewidth graphs.
%These improvements make crucial use of the fact that such graphs admit small separators:
%given a graph $G$ of bounded treewidth $p$, there exists a set $S \subset V(G)$ of at most $p+1$ vertices
%whose removal separates the graph into two connected components, each of size at most $2/3 \cdot |V(G)|$ (see \cite{bodlaender95}).
%
%Krauthgamer et al.~\cite{distancepreserving} use the above fact to construct an $(1, O(p^{3}k))$-DAM for graphs of treewidth at most $p$.
%We show that with two modifications, their algorithm can be extended for the constructions of DAMs.
%The first modification is to Step 2 of the algorithm \textsc{ReduceGraphTW} in \cite{distancepreserving}.
%For any integer $q\geq 1$, we replace their call to \textsc{ReduceGraphNaive}$(H,T \cup B)$\footnote{We remark that they use $R$ to denote the set of terminals}
%by our procedure \textsc{MinorSparsifier}$(H,T \cup B, \mathcal{P}')$, where $ \mathcal{P}'$ is a $(2q-1, O(p^{1+1/q}))$-TPc of $G$.
%
%The second modification is a generalization of Lemma 4.2 in \cite{distancepreserving}.
%The small separator set $S$ allows us to decompose $G$ into two smaller graphs, which we can work on recursively,
%and at the end we \emph{knit} them with the separator vertices.
%It is not hard to see that if the smaller graphs have distortions $\alpha_1,\alpha_2$, then after the knitting,
%the distortion is at most $\max\{\alpha_1,\alpha_2\}$.

%The main idea lies in decomposing the graph into smaller networks, say $G_1$ and $G_2$, computing independently minors for such graphs, and then combining the minors back into a minor of $G$. We remark that such decomposition/composition will be carried out only on the terminal vertices. Formally, let $G_1 = (V_1, E_1, \ell_1)$ and $G_2 = (V_2,E_2, \ell_2)$ be graphs on disjoint sets of non-terminals, having terminal sets $T_1 = \{s_1,s_2,\ldots,s_{a_1}\}$ and $T_2 = \{t_1,t_2,\ldots,t_{a_2}\}$, respectively. Further, let $\phi(s_i)=t_i$, for all $i=1,\ldots,c$ be an one-to-one correspondence between some subset of $T_1$ and $T_2$. The \textit{$\phi$-merge} (or $2$-sum) of $G_1$ and $G_2$ is the graph $G = (V,E,\ell)$ with terminal set $T = T_1 \cup \{t_{c+1},\ldots,t_{a_2}\}$ formed by identifying the terminals $s_i$ and $t_i$, for all $i=1,\ldots,c$, where $\ell(e) = \min\{\ell_1(e),\ell_2(e)\}$ (assuming infinite length when $\ell_i(e)$ is undefined). We denote this operation by $ G := G_1 \oplus_{\phi} G_2$.
%
%Below we state the the generalized lemma whose proof goes along the lines of Lemma 4.2 from their paper.
%
%\begin{lemma} Let $G = G_1 \oplus_{\phi} G_2$. For $j=\{1,2\}$, let $H_j$ be an $(\alpha_j,f(a_j))$-\emph{DAM} for $G_j$. Then the graph $H = H_1 \oplus_{\phi} H_2$ is an $(\max\{\alpha_1,\alpha_2\}, f(a_1) + f(a_2))$-\emph{DAM} of G.  
%\end{lemma}
%
%In ~\cite{distancepreserving} it is shown that the size of the minor returned by the algorithm \textsc{ReduceGraphTW} is bounded by the number of leaves the in the recursion tree of the algorithm. Further, they prove that there are at most $O(k/p)$ such leaves. Plugging our bounds from the modification of Step 2 along with the above lemma leads to the following result.

==> chapters/distanceminors/upper-bound-planar.tex <==
\section{Minor Construction for Planar Graphs}\label{sect:UB-planar}
In this section, we show that for planar graphs one can improve the constant guarantee bound on the
distortion to $3$ and $1+\epsilon$, respectively,
without affecting the size of the minor. Our work builds on existing techniques used in the context of approximate distance oracles,
thereby bypassing our previous spanner reduction. Both results use essentially the same ideas
and rely heavily on the fact that planar graphs admit separators with special properties.

We say that a graph $G=(V,E,\ww)$ admits a $\lambda$-separator if there exists a set $R \subseteq V$
whose removal partitions $G$ into connected components, each of size at most $\lambda n$, where $1/2 \leq \lambda <1$.
Lipton and Tarjan~\cite{lipton79} showed that every planar graph has a $2/3$-separator $R$ of size $O (\sqrt{n})$.
Later on, Gupta et al.~\cite{guptaKR04} and Thorup~\cite{ThorupJACM04} independently observed that one can modify their construction
to obtain a $2/3$-separator $R$, with the additional property that $R$ consists of vertices belonging to shortest paths from $G$
(note that this $R$ is not guaranteed to be small). We briefly review the construction of such \textit{shortest path separators}. 

Let $G=(V,E,\ww)$ be a triangulated planar graph (the triangulation is guaranteed by adding infinity edge lengths among the missing edges). Further, let us fix an arbitrary shortest path tree $A$ rooted at some vertex $r$. Then, it can be inferred from the work of Lipton and Tarjan~\cite{lipton79} that there always exists a non-tree edge $e=(u,v)$ of $A$ such that the fundamental cycle $\mathcal{C}$ in $A \cup \{e\}$, formed by adding the non-tree edge $e$ to $A$, gives a $2/3$-separator for $G$. Because $A$ is a tree, the separator will consist of two paths from the $\text{lca}(u,v)$ to $u$ and $v$. We denote such paths by $P_1$ and $P_2$, respectively. Both paths are shortest paths as they belong to $A$. We will show how to use such separators to obtain terminal path covers. Before proceeding, we give the following preprocessing step.

\paragraph*{Preprocessing Step.} Given a planar graph $G = (V,E,\ww)$ with $K \subset V$, the algorithm \textsc{MinorSparsifier}($G$, $T$, $\mathcal{P}'$) with $\mathcal{P}'$ being the $(1,O(k^{2}))$-TPc of $G$, produces an $(1,O(k^{4}))$-DAM $G'$ for $G$. To simplify our notation, we will use $G$ instead of $G'$ in the following, i.e., we assume that $G$ has at most $O(k^{4})$ vertices.

%\smallskip

\subsection{Distortion-$3$ Guarantee}

%\noindent\textbf{Stretch-$3$ Guarantee.~}
When solving a graph problem it is often the case that the solution is much easier on simpler graph instances, e.g., trees.
%there exist simpler graph instances, e.g., trees, for which the problem can be more easily solved.
Driven by this, it is desirable to reduce the problem from arbitrary graphs to one or several tree instances, possibly allowing a small loss in the quality of the solution. Along the lines of such an approach, Gupta et al.~\cite{guptaKR04} gave the following definition in the context of shortest path distances.
\begin{definition}[Forest Cover] Given a graph $G=(V,E,\ww)$, a forest cover (with stretch $\alpha$) of $G$ is a family $\mathcal{F}$ of subforests $\{F_1,F_2,\ldots,F_k\}$ of $G$ such that for every $u,v \in V$, there is a forest $F_i \in \mathcal{F}$ such that $\dist_{G}(u,v) \leq \dist_{F_i}(u,v) \leq \alpha \cdot \dist_G(u,v)$.
\end{definition}

If we restrict our attention to planar graphs, Gupta et al.~\cite{guptaKR04} used shortest path separators (as described above) to give a divide-and-conquer algorithm for constructing forest covers with small guarantees on the stretch and size. Here, we slightly modify and adopt their construction for our specific application. 
Before proceeding to the algorithm, we give the following useful definition.
\begin{definition}
Let $t$ be a terminal and let $\pi$ be a shortest path in $G$. Then $t_{\min}^{\pi}$ denotes the vertex of $\pi$ that minimizes $\dist_G(t,p)$, for all $p \in V(\pi)$, breaking ties lexicographically. 
\end{definition}

\begin{algorithm2e}
\label{algo: forestcover}
\caption{\textsc{ForestCover}$(G,K)$}
\Input{Planar graph $G=(V,E,\ww)$, terminals $K$}
\Output{Forest cover $\mathcal{F}$ of $G$}
\If{$|V(G)| \leq 1$} {	\Return $V(G)$ \; }
Compute a $2/3$-separator $\mathcal{C}$ consisting of shortest paths $\pi_1$ and $\pi_2$ for $G$ \;
\For{$i=1,2$}{ 
Contract $\pi_i$ to a single vertex $p_i$ and compute a shortest path tree $L_i$ from $p_i$ \;
Expand back the contracted edges in $L_i$ to get the tree $L_i'$ \;
\For{every terminal $t \in T$}{
  Add $t_{\min}^{\pi_i}$ as a terminal in the tree $L_i'$ \;
}
}
Let $(G_1,K_1)$ and $(G_2,K_2)$ be the resulting connected graphs from $G \setminus \mathcal{C}$, \; 
\nonl where $K_1$ and $K_2$ are disjoint subsets of the terminals $K$ induced by $\mathcal{C}$ \;
\tcp{Note that all distances involving terminals from $\mathcal{C}$ are taken care of}
\Return $\bigcup_{i=1}^{2} L_i' \cup \bigcup_{i=1}^{2} \textsc{ForestCover}(G_i,K_i)$ \;
\end{algorithm2e}

\begin{algorithm2e}
\label{algo: minor1}
\caption{\textsc{PlanarTPc-1} $(G,K)$}
\Input{Planar graph $G=(V,E,\ww)$, terminals $K$}
\Output{Terminal path cover $\mathcal{P}'$ of $G$}
Set $\mathcal{P}' = \emptyset$ \;
Set $\mathcal{F} = \text{\textsc{ForestCover}}(G,K)$ \; %Apply Theorem \ref{thm: guptacover} on $G$ and let $\mathcal{F}$ be the resulting forest cover.
\For{each forest $F_i \in \mathcal{F}$} {
Let $R_i$ be the terminal set of $F_i$ and let $\mathcal{P}'_i$  be the (trivial) $(1,O(k^{2}))$-TPc of $F_i$ \;
Compute $F_i'$ = \textsc{MinorSparsifier}($F_i$, $R_i$, $\mathcal{P}_i'$) \;
Add the shortest paths corresponding to the edges of $F_i'$ to $\mathcal{P}'$ \;
}
\Return $\mathcal{P}'$ \;
\end{algorithm2e}

Gupta et al.~\cite{guptaKR04} showed the following guarantees for Algorithm \ref{algo: forestcover}.

\begin{theorem}[\cite{guptaKR04}, Theorem 5.1] \label{thm: guptacover}
Given a planar graph $G=(V,E,\ww)$ with $K \subset V$, \textsc{ForsetCover}$(G,K)$ produces a stretch-$3$ forest cover with $O (\log |V|)$ forests. 
\end{theorem} 

We note that the original construction does not consider terminal vertices, but this does not worsen neither the stretch nor the size of the cover. The only difference here is that we need to add at most $k$ new terminals to each forest compared to the original number of terminals in the input graph. This modification affects our bounds on the size of a minor only by a constant factor. 

Below we show that using the above theorem one can obtain terminal path covers for planar graphs. 

\begin{lemma} Given a planar graph $G = (V,E, \ww)$ with $K \subset V$, \textsc{PlanarTPc-1}$(G,K)$ produces an $(3,O (k \log k))$-\emph{TPc} $\mathcal{P}'$ for $G$. 
\end{lemma}
\begin{proof}
We first review the following simple fact, whose proof can be found in \cite{KrauthgamerNZ14}.
\begin{fact} \label{fact: treecover}
Given a forest $F=(V,E,\ww)$ with terminals $K \subset V$ and $\mathcal{P}'$ being the (trivial) $(1,O(k^{2}))$-\emph{TPc} of $F$, the procedure \textsc{MinorSparsifier}$(F,K,\mathcal{P}')$ outputs an $(1,k)$-\emph{DAM}.  
\end{fact}

Let us proceed with the analysis. Observe that from the Preprocessing Step our input graph $G$ has at most $O(k^{4})$ vertices. Thus, applying Theorem \ref{thm: guptacover} on $G$ gives a stretch-$3$ forest cover $\mathcal{F}$ of size $O(\log k)$. In addition, recall that all shortest paths are unique in $G$.

Next, let $F_i$ by any forest from $\mathcal{F}$. By construction, we note that each tree belonging to $F_i$ has the nice property of being a concatenation of a given shortest path with another shortest path tree. We will exploit this in order to show that every edge of the minor $F_i'$ for $F_i$ corresponds to the (unique) shortest path between its endpoints in $G$.

%\GG{The pathological case is resolved! We need to only make some changes!}


To this end, let $e' = (u,v)$ be an edge of $F_i'$ that does not exist in $F_i$. Since $F_i'$ is a minor of $F_i$, we can map back $e'$ to the path $\pi_{u,v}$ connecting $u$ and $v$ in $F_i$. Because of the additional terminals $u_{\min}^{P_i}$ added to $F_i$, we claim that $\pi_{u,v}$ is entirely contained either in some shortest path tree $L_j$ or some shortest path separator $P_j$. Using the fact that subpaths of shortest paths are shortest paths, we conclude that the length of the path $\pi_{u,v}$ (or equivalently, the length of edge $e'$) corresponds to the unique shortest path connecting $u$ and $v$ in $G$. The same argument is repeatedly applied to every such edge of $F_i'$.

By construction we know that $F_i$ has at most $2k$ terminals. Using Fact \ref{fact: treecover} we get that $F_i'$ contains at most $4k$ edges. Since there are $O (\log k)$ forests, we conclude that the terminal path cover $\mathcal{P}'$ consists of $O (k \log k)$ shortest paths. The stretch guarantee follows directly from that of cover $\mathcal{F}$, since $F_i'$ exactly preserves all distances between terminals in $F_i$.
\end{proof}

\begin{theorem}
Any planar graph $G=(V,E,\ww)$ with $K \subset V$ admits a $(3, \tilde{O}(k^{2}))$-\emph{DAM}.
\end{theorem}

%Indeed, there is another distance oracle that yields better distortion $(1+\epsilon)$ (see~\cite{ThorupJACM04,sommer11}).
%Similar to the above, we prove the following theorem; its proof is deferred to the full version.

\subsection{Distortion-$(1+\epsilon)$ Guarantee}
%\noindent\textbf{Stretch-$(1+\epsilon)$ Guarantee.~}

Next we present our best trade-off between distortion and size of minors for planar graphs. Our idea is to construct terminal path covers using the construction of Thorup~\cite{ThorupJACM04} in the context of approximate distance oracles in planar graphs. Here, we modify a simplified version due to Kawarabayashi et al.~\cite{sommer11}. 

The construction relies on two important ideas. Similarly to the distortion-$3$ result, the first idea is to recursively use shortest path separators to decompose the graph. The second consists of approximating shortest paths that cross a shortest path separator. Below we present some necessary modification to make use of such a construction for our purposes.

Let $\pi$ be a shortest path in $G$. For a terminal $t \in K$, we let the pair $(p,t)$, where $p \in V(\pi)$, denote the \textit{portal} of $t$ with respect to the path $\pi$. An $\epsilon$-cover $C(t,\pi)$ of $t$ with respect to $\pi$ is a set of portals with the following property:
\begin{itemize}
\item for all $p \in V(\pi)$, thee exsits $q \in C(t,\pi)$ such that \[ \dist_G(t,q) + \dist_G(q,p) \leq (1+\epsilon) \dist_G(t,p). \]
\end{itemize}
Let $(t,t')$ by any terminal pair in $G$. Let $\pi_{t,t'}$ be the (unique) shortest path that crosses the path $\pi$ at vertex $w$. Then using the $\epsilon$-covers $C(t,\pi)$ and $C(t',\pi)$, there exist portals $(t,p)$ and $(p',t')$ such that the new distance between $t$ and $t'$ is
\begin{align} \label{eqn: stretch}
\begin{split}
	\dist_G(t,p) & + \dist_G(p,p')  + \dist_G(p',t') \\
	& \leq \dist_G(t,p) + \dist_G(p,w) + \dist_G(w,p') + \dist_G(p',t') \\
	& \leq (1+\epsilon) \dist_G(t,t').
\end{split}
\end{align}
The new distance clearly dominates the old one. The next result due to Thorup~\cite{ThorupJACM04} shows that maintaining a small number of portals per terminal suffices to approximately preserve terminal shortest paths.

\begin{lemma} \label{lemm: portal} 
Let $\epsilon > 0$. For a given terminal $t \in K$ and a shortest path $\pi$, there exists an $\epsilon$-cover $C(t,\pi)$ of size $O(1/\epsilon)$.
\end{lemma}

The above lemma leads to the following recursive procedure.

\begin{algorithm2e}
\label{algo: minor2}
\caption{\textsc{PlanarTPc-2} $(G,K)$}
\Input{Planar graph $G=(V,E,\ww)$, terminals $K$}
\Output{Terminal path cover $\mathcal{P}'$ of $G$}
\If{$|V(G)| \leq 1$ or $K = \emptyset$}
{	\Return $\emptyset$ \; }

Set $\mathcal{B} = \emptyset$ \; 

Compute a $2/3$-separator $\mathcal{C}$ consisting of shortest paths $\pi_1$ and $\pi_2$ \;
Add $\pi_1$ and $\pi_2$ to $\mathcal{B}$ \;
\For{every terminal $t \in K$}{
Compute $\epsilon$-covers $C(t,\pi_1)$ and $C(t,\pi_2)$ \;
\For{every portal $(t,p) \in C(t,\pi_1) \cup C(t,\pi_2)$}{
 Add the shortest path $\pi_{t,p}$ to $\mathcal{B}$ \;
}
}
Let $(G_1,K_1)$ and $(G_2,K_2)$ be the resulting connected graphs from $G \setminus \mathcal{C}$, \;
\nonl where $K_1$ and $K_2$ are disjoint subsets of the terminals $K$ induced by $\mathcal{C}$ \;
\tcp{ Note that all distances involving terminals from $\mathcal{C}$ are taken care of}
\Return $\mathcal{B} \cup \bigcup_{i=1}^{2} \textsc{PlanarTPc-2}(G_i,K_i)$ \;
\end{algorithm2e}

\begin{lemma}\label{lem:tpc-1-plus-ep}
Given a planar graph $G = (V,E, \ww)$ with $K \subset V$, \textsc{PlanarTPc-2}$(G,K)$ outputs an $(1+\epsilon,O (k \epsilon^{-1} \log k ))$-\emph{TPc} $\mathcal{P}'$ for $G$. 
\end{lemma}

\begin{proof}
From the Preprocessing Step we know that $G$ has at most $O(k^{4})$ vertices. Further,  recall that removing the vertices that belong to the shortest path separators from $G$ results into two graphs $G_1$ and $G_2$, whose size is at most $2/3 \cdot |G|$. Thus, there are at most $O(\log k)$ levels of recursion for the above procedure.  

Let $\mathcal{P}'$ be the terminal path cover output by \text{PlanarTPc-2}$(G,K)$. We first bound the number of separator shortest paths added in Step 3. Note that at any level of the recursion there at most $k$ terminals and, thus the number of recursive calls per level is at most $k$. Since we added two paths per recursive call, we get that there are at most $O (k \log k)$ paths overall.

We now continue with the counting or portals. Let $t \in K$ be any terminal and consider any recursive call applied on the current graph $(G',K')$. If $t \not\in K'$, then we simply ignore $t$. Otherwise, $t$ either belongs to one of the separator shortest paths in $G'$ or one of the partitions induced by the separators. In the first case, we know that $t$ is retained because we added $\pi_1$ and $\pi_2$ to $\mathcal{P}'$ and these are already counted. In the second case, using Lemma \ref{lemm: portal}, we add $O(1/\epsilon)$ shortest paths connecting portals from $C(t,\pi_1)$ and $C(t,\pi_2)$. Therefore, in any recursive call, we maintain at most $O(1/\epsilon)$ shortest paths per terminal. Since every terminal can participate in at most $O(\log k)$ recursive calls, we get that the total number of portal-shortest paths is at most $O (k \log k / \epsilon)$. Combining both bounds, it follows that the size of $\mathcal{P}'$ is at most $O(k \log k / \epsilon)$. 

It remains to show the stretch guarantee of $\mathcal{P}'$. Let $R$ be the recursion tree of the algorithm, where every node corresponds to a recursive call. For any pair $t,t' \in L$, let $a \in V(R)$ associated with $(G_a, K_a)$ be the leafmost node such that $t,t' \in K_a$. Then, it follows that among all ancestors of $a$ in the tree $R$, there must exist a separator path $\pi_i$, $i=1,2$ that crosses $\pi_{t,t'}$ and attains the minimum length. The stretch guarantee follows directly from (\ref{eqn: stretch}).
\end{proof}

\begin{theorem}\label{thm:planar-oneplus}
%Any planar graph $G=(V,E,\ww)$ with $T \subset V$ admits an $(1+\epsilon, \tilde{O}(\frac{k^2}{\epsilon^2}))$-\emph{DAM}.
Any planar graph $G=(V,E,\ww)$ with $K \subset V$ admits an $(1+\epsilon,O(k^{2} \epsilon^{-2} \log^{2} k))$-\emph{DAM}.
\end{theorem} 

==> chapters/lowstretchtree/LDD.tex <==
\section{Dynamic Low-Diameter Decomposition}\label{sec:LDD}

In this section we develop our dynamic algorithm for maintaining a low-diameter decomposition following three steps.
First, we review the static algorithm for constructing a low-diameter decomposition using the clustering due to Miller et al.~\cite{MillerPX13}.
Second, we design a decremental algorithm by extending the Even-Shiloach algorithm~\cite{EvenS81} in a suitable way.
Third, we lift our decremental algorithm to a fully dynamic one by using a ``lazy'' approach for handling insertions.


\subsection{Static Low-Diameter Decomposition}~\label{sec:staticLDD}

In the following, we review the static algorithm for constructing a low-diameter decomposition clustering due to Miller et al.~\cite{MillerPX13}. Let $G=(V,E)$ be an unweighted, undirected multigraph $G$, and let $\beta \in (0,1)$ be some parameter. Our goal is to assign each node $u$ to exactly one node $c(u)$ from $V$. Let $C(u) \subset V$ denote the set of nodes assigned to node $u$, i.e., $C(u) \coloneqq \set{v \in V}{ c(v) = u}$. For each node $u$, we initially set $C(u)= \varnothing $ and pick independently a \emph{shift} value $\delta_u$ from $\expdis(\beta)$. Next, we assign each node $u$ to a node $v$, i.e., set $c(u) = v$ and add $u$ to $C(v)$, if $v$ is the node that minimizes the \emph{shifted distance} $m_v(u)\coloneqq \dist(u,v) - \delta_v$. Finally, we output all clusters that are non-empty. The above procedure is summarized in Algorithm~\ref{alg:partition}.

\begin{algorithm2e}[htb!]
\caption{Partitioning Using Exponentially Shifted Shortest Paths}
\label{alg:partition}

\BlankLine
\KwData{Multigraph $G=(V,E)$, parameter $\beta \in (0,1)$}
\KwResult{Decomposition of $G$}
\BlankLine

For each $u \in V$, set $C(u)=\varnothing$ and pick $\delta_u$ independently from $\expdis(\beta)$ \;
Assign each $u \in V$ to $c(u) \gets \arg \min_{v \in V} \{\dist(u,v) - \delta_v\}$\;
For each $v \in V$, set $C(u) \gets \set{v \in V}{c(v) = u}$\;
Return the clustering $\set{C(u)}{C(u) \neq \varnothing}$
\end{algorithm2e}

The following theorem gives bounds on the strong diameter and the number of inter-cluster edges output by the above partitioning.

\begin{theorem}[\cite{MillerPX13}, Theorem~1.2] \label{thm: Miller_LDD} Given an undirected, unweighted multigraph graph $G=(V,E)$ and a parameter $\beta \in (0,1)$, Algorithm~\ref{alg:partition} produces a $(\beta, 2 d \cdot(\log n/\beta))$-decomposition such that the guarantee on the number of inter-cluster edges holds in expectation, while the diameter bound holds with probability at least $1-1/n^d$, for any $d \geq 1$.
\end{theorem}

Here, the the diameter bound holds when the maximum shift value of any node is at most $ d \log n/\beta $, which happens with probability $1-1/n^d$.
We remark that in the work of Miller et al., the above guarantees are stated only for undirected, unweighted \emph{simple} graphs. However, by~Lemma 4.4 in~\cite{MillerPX13}, we get that each edge $e \in E$~(regardless of whether $E$ allows parallel edges) is an inter-cluster edges with probability at most $\beta$. By linearity of expectation, it follows that the (expected) number of inter-cluster edges in the resulting decomposition is at most $\beta m$, thus showing that the algorithm naturally extends to multigraphs.

For technical reasons, it is not sufficient in the analysis of our decremental LDD algorithm to apply Theorem~\ref{thm: Miller_LDD} in a black-box manner.
We thus review the crucial properties of the clustering algorithm, which we will exploit for bounding the number of changes made to inter-cluster edges in the decremental algorithm. Following~\cite{MillerPX13}, for each edge $e=(u,v) \in E$, let $w$ be the \emph{mid-point} of $e$, i.e., the imaginary node in the ``middle'' of edge $ e $ that is at distance $ \tfrac{1}{2} $ to both $ u $ and $ v $. Lemma~4.3 in \cite{MillerPX13} states that if $u$ and $v$ belong to two different clusters, i.e., $c(u) \neq c(v)$, then the shifted-distances $m_{c(u)}(w)$ and $m_{c(v)}(w)$ are within $1$ of the minimum shifted distance to $w$.

\begin{lemma}[\cite{MillerPX13}]\label{lem:inter cluster edge implies mid-point condition}
Let $e=(u,v)$ be an edge with mid-point $w$ such that $c(u) \neq c(v)$ in Algorithm~\ref{alg:partition}. Then $m_{c(u)}(w)$ and $m_{c(v)}(w)$ are within $1$ of the minimum shifted distance to $w$. 
\end{lemma}

Lemma 4.4 of~\cite{MillerPX13} shows that the probability that the smallest and the second smallest shifted distances to $w$ are within $c$ of each other is at most $c \cdot \beta$.

\begin{lemma}[\cite{MillerPX13}]\label{lem:probability of mid-point condition}
Let $ e = (u,v) $ be an edge with mid-point $ w $.
Then \[ \Pr [| m_{c(u)}(w) - m_{c(v)}(w) | \leq c] \leq c \cdot \beta. \]
\end{lemma}

Setting $c=1$, this gives the desired bound of $ \beta $ for the probability of an edge being an inter-cluster edge in Theorem~\ref{thm: Miller_LDD}.


\paragraph*{Implementation.} 
Na\"ively, we could implement Algorithm~\ref{alg:partition} by computing $c(u)$ for each node $u \in V$ in $\tilde{O}(m)$, thus leading to a $\tilde{O}(mn)$ time algorithm. In the following, using standard techniques, we show that this running time can be reduced to $\tilde{O}(m)$.

To this end, let $\delta_{\max} \coloneqq \max_{u \in V} \{ \delta_u \}$. We begin with the following augmentation of the input graph $G$: add a new source $s$ to $G$ and edges $(s,u)$ of weight $(\delta_{\max} - \delta_u) \geq 0$, for every $u \in V$. Let $\hat{G}=(V \cup \{s\},\hat{E},\hat{\ww})$ denote the resulting graph. We claim that the sub-trees below the source $s$ in the shortest path tree of $\hat{G}$ rooted at $s$ give us the clustering output by Algorithm~\ref{alg:partition} for the graph $G$. To see this, suppose that we instead added edges of weight $-\delta_u$ to $s$, for every $u \in V$. Then it is easy to check that for every $u \in V$, the distance between $s$ and $u$ is exactly $ \min_{v \in V} (\dist(u,v) - \delta_v) = \min_{v \in V} m_v(u)$. Thus the node $v$ attaining the minimum is exactly the root of the sub-tree below the source $s$ that contains $v$. Now, adding $\delta_{\max}$ to all edges incident to the source increases all distances to $s$ by $\delta_{\max}$, and thus does not affect the shortest path tree.

Now, note that we could use Dijkstra's algorithm to construct the shortest path tree of $\hat{G}$, and modify it appropriately to output the clustering. However, for reasons that will become clear in the next section, we need to modify Dijkstra's algorithm in a specific way. This modification can be viewed as mimicking a BFS computation on a graph with special \emph{integral} edge lengths. 

We start by observing that due to the random shift values, the weight of the edges incident to the source $s$ in $\hat{G}$ are not integers. Since we only want to deal with \emph{integral} weights, we round down all the $\delta_u$ values to $\floor{\delta_u}$ and modify the weights of these edges using the new rounded values. Let $G'=(V \cup \{s\}, \hat{E}, \ww')$ denote the modified graph. Note that due to the rounding, we need to introduce some tie-breaking scheme in $G'$, such that  every clustering of $G'$ matches exactly the same clustering in $\hat{G}$, and vice versa. Naturally, the fractional parts of the rounded values, i.e., $\delta_u - \floor{\delta_u}$, define an ordering on the nodes (if they are sorted in ascending order), and this ordering can be in turn used to break ties whenever two rounded distances are equal in $G'$. In their PRAM implementation, Miller et al.~\cite{MillerPX13} observed that this ordering can emulated by a random permutation. This is due to the fact that the shifts are generated independently, and that the exponential distribution is memoryless. 

The main motivation for using random permutations in previous works was to avoid errors that might arise from the machine precision. In our work, breaking ties according to a random permutation on the nodes is one of their algorithmic ingredients that allows us to obtain an efficient dynamic variant of the clustering. Below, we give specific implementation details about how our clustering interacts with random priorities in the static setting. 

Given the graph $G'$ and a distinguished source node $s \in V'$,  Dijkstra's classical algorithm maintains an upper-bound on the shortest-path distance between each node $u \in V$ and $s$, denoted by $\ell(u)$. Initially, it sets $\ell(u) = \infty$, for each $u \in V$ and $\ell(s) = 0$. It also marks every node unvisited. Moreover, for each node $u \in V$, the algorithm also maintains a pointer $p(u)$ (initially set to $\nil$), which denotes the parent of $u$ in the current tree rooted at $s$. Using these pointers, we can maintain the cluster pointer $c(u)$, for each $u \in V$. This follows from the observation that in order to compute the cluster of $u$, it suffices to know the cluster of its parent. Formally we have the following rule.

\begin{observation} \label{obs: clusterUpdate}
Let $p(\cdot)$ be the parent pointers. Then for each $u \in V$, we can determine the cluster pointer $c(u)$ using the following rule:

\[
	c(u) =  \begin{cases} 
    u & \text{\emph{if} } p(u)=s \\
    c(p(u))      & \text{\emph{otherwise}}.
  \end{cases}
\]
\end{observation}

Now, at each iteration, Dijkstra's algorithm selects an unvisited node $u$ with the smallest $\ell(u)$, marks it as visited, and \emph{relaxes} all its edges. In the standard relaxation, for each edge $(u,v) \in E'$ the algorithm sets $\ell(v) \gets \min\{\ell(v), \ell(u) + w'(u,v)\}$ and updates $p(v)$ accordingly. Here, we present a relaxation according to the following tie-breaking scheme. Let $\pi$ be a random permutation on $V$. For $u, v \in V$, we write $\pi(u) < \pi(v)$ if $u$ appears before $v$ in the permutation $\pi$.
Now, when relaxing an edge $(u,v) \in E'$, we set $u$ to be the parent of $v$, i.e., $p(v) = u$, and $\ell(v) = \ell(u) + w'(u,v)$, if the following holds
\begin{align} \label{eq: breakingTies}
\begin{split}
\ell(v) & > \ell(u) + w'(u,v), \text{ or} \\
\ell(v) & = \ell(u) + w'(u,v) \text{ and } \pi(c(v)) > \pi(c(u)).
\end{split}
\end{align}

After each edge relaxation, we also update the cluster pointers using  Observation~\ref{obs: clusterUpdate}. We continue the algorithm until every node is visited. As usual, we maintain the unvisited nodes in a heap $Q$, keyed by the their estimates $\ell(v)$. This procedure is summarized in Algorithm~\ref{alg:ModDijkstra}.

\begin{algorithm2e}[htb!]
\caption{Modified Dijkstra}
\label{alg:ModDijkstra}
\KwData{Graph $G'=(V \cup \{s\},E',\ww')$}
\KwResult{Decomposition of $G$}
\BlankLine

Generate random permutation $\pi$ on $V$\;
%\BlankLine
\ForEach{$u \in V$}{
Set $\ell(u) = \infty$\;
Set $p(u) = \nil$\;
Set $c(u) = \nil$\;
}

Set $\ell(s) = 0$\;
\BlankLine

Add every $u \in V \cup \{s\}$ into heap $Q$ with key $\ell(u)$\;
\While{heap $ Q $ is not empty}{
	    Take node $ u $ with minimum key $ \lev (u) $ from heap $ Q $ and remove it from $ Q $ \;
		\ForEach{neighbor $ v $ of $ u $}{
		\Relax{$u$, $v$, $w'$, $\fraction$} \;
		\eIf{$ p(v) = s $}{
			Set $ c (v) = v  $\;
		}{
			Set $ c (v) = c( p(v)) $\;
		}
	}
}

\Procedure{\Relax{$u$, $v$, $w'$, $\fraction$}}{
	\uIf{$\ell(v) > \ell(u) + w'(u,v)$}{
		Set $\ell(v) = \ell(u) + w'(u,v)$\;
		Set $p(v) = u$\;
		}
	\uElseIf{$\ell(v) = \ell(u) + w'(u,v)$ \emph{and} $\pi(c(v)) > \pi(c(u))$}{
     Set $p(v) = u$ \;}
}
\end{algorithm2e}


Correctness of Algorithm~\ref{alg:ModDijkstra} follows by our above discussion. Moreover, the running time of the algorithm is asymptotically bounded by the running time of Dijkstra's classical algorithm and the time to generate a random permutation. It is well known that the former runs in $\tilde{O}(m)$ time and the latter can be generated in $O(n)$ time (see e.g., Knuth Shuffle~\cite{BermanK76}), thus giving us a total $\tilde{O}(m)$ time.



\subsection{Decremental Low-Diameter Decomposition}\label{sec:ES tree}\label{sec:decremental LDD}

We now show how to maintain a lower-diameter decomposition under deletion of edges. Recall that in the previous section we observed that computing a lower-diameter decomposition of a undirected, unweighted graph can be reduced to the single-source shortest path problem in some modified graph. In the same vein, we observe that maintaining a low-diameter decomposition under edge deletions amounts to maintaining a bounded-depth single-source shortest path tree of some modified graph under edge deletions. 

Even and Shiloach~\cite{EvenS81} devised a data-structure for maintaining a bounded-depth SSSP-tree under edge deletions, which we refer to as \emph{ES-tree}. The ES-tree initially worked only for undirected, unweighted graphs. However, later works~\cite{HenzingerK95,King99} observed that it can be extended even to directed, weighted graphs with positive integer edges weights. The mere usage of the ES-tree as a sub-routine will not suffice for our purposes, due to the constraints that our clustering imposes. In the following we show how to augment and modify an ES-tree that maintains a valid clustering, without degrading its running time guarantee. 

Let $G=(V,E)$ be an undirected, unweighted graph for which we want to maintain a decremental $(\beta, \log n/ \beta)$ decomposition, for any parameter $\beta \in (0,1)$. Further, let $G'=(V\cup \{s\},E',\ww')$ be the undirected graph with integral edge weights, as defined in Section~\ref{sec:staticLDD}.
Let $\pi$ be a random permutation on $V$. By discussion in Section~\ref{sec:staticLDD}, in order to maintain a low-diameter decomposition of $G$ it suffices to maintain a clustering of $G'$ with $\pi$ used for tie-breaking.

We describe an ES-tree that efficiently maintains a clustering of $G'$ for a given root node $s$ and a given distance parameter $\Delta$. Here we set $\Delta = O(\log n / \beta)$, as by Theorem~\ref{thm: Miller_LDD}, the maximum distance that we run our algorithm to is bounded by $O(\log n / \beta)$. Our data-structure handles arbitrary edge deletions, and maintains the following information. First, for each node $u \in V \cup \{s\}$, we maintain a label $\lev(u)$, referred to as the \emph{level} of $u$. This level of $u$ represents the shortest path between the root $s$ and $u$, i.e., $\lev(u) = \dist(s,u)$. Next, for each node $u \in V$, we maintain pointers $p(u)$ and $c(u)$, which represent the parent of $u$ in the tree and the node that $u$ is assigned to, respectively. Finally, we also maintain the set of \emph{potential} parents $P(u)$, for each $u \in V$, which is the set of all neighbors of $u$ that are in the same level with the parent of $u$, and share the same clustering with $u$, i.e., a neighbor $v$ of $u$ belongs to $P(u)$ if $v$ minimizes $(\ell(v) + \ww'(u,v), \pi(c(v)))$ lexicographically, and $c(v) = c(u)$. Edge deletions in $G'$ can possibly affect the above information for several nodes. Our algorithm adjusts these information on the nodes so as to make them valid for the modified graph.


\paragraph*{Algorithm Description and Implementation.}
We give an overview and describe the implementation of Algorithm~\ref{alg:ES_tree}. The data-structures $\ell(\cdot)$, $p(\cdot)$ and $c(\cdot)$ are initialized using Algorithm~\ref{alg:ModDijkstra} in Section~\ref{sec:staticLDD}. Note that for each $u \in V$, $P(u)$ can be computed by simply considering all neighbors of~$u$ in turn, and adding a neighbor $v$ to $P(u)$ if $v$ is a potential parent. The algorithm also maintains a heap $Q$ whose intended use is to store nodes whose levels or clustering might need to be updated. (see procedure \Initialize{}). 

In our decremental algorithm, each node tries to maintain its level $\ell(u)$, which corresponds to its current distance to the root $s$, together with its cluster pointer $c(u)$ in the current graph. Concretely, we maintain the following invariant for each node $u \in V$:
\begin{align}
\ell(u)&=\min\set{\ell(v)+\ww'(u, v)}{v \text{ is a neighbor of } u} \label{eq:ES tree level condition}
\end{align}
where ties among neighbors are broken according to~(\ref{eq: breakingTies}). This invariant allows to compute the cluster pointer $c(u)$ using Observation~\ref{obs: clusterUpdate}. Deleting an edge incident to $u$ might lead to a change in the values of $\ell(u)$ and $c(u)$. If this occurs, all neighbors of $u$ are notified by $u$ about this change, since their levels and cluster points might also change. It is well-known that the standard ES-tree can efficiently deal with changes involving the levels $\ell(\cdot)$. However, in our setting, it might be the case that an edge deletion forces a node $u$ to change its cluster while the level $\ell(u)$ still remains the same under this deletion. This is the point where our algorithm differs from the standard ES-tree, and we next show that (1) such changes can be handled efficiently, and (2) the number of cluster changes per node, within the same level, is small in expectation.

Let us consider the deletion of an edge $(u,v)$ (see procedure $\Delete()$); assume without loss of generality that $\ell(v) \leq \ell(u)$. Now note that an edge deletion might lead to a cluster change only if $v \in P(u)$. If this is the case, the algorithm first removes $v$ from the set $P(u)$. If $P(u)$ is still non-empty, the clustering remains unaffected. However, if $P(u)$ is empty, the clustering of $u$ will change, and the algorithm inserts $u$ into the heap $Q$ with key $\ell(u)$. Observe that a change in clustering of $u$ might potentially lead to cluster changes for children of $u$, given that $u$ was their only potential parent. In this way, we observe that deleting $(u,v)$ might force changes in the clustering for many descendants of $v$. The algorithm handles such changes using procedure $\UpdateLevels()$, which we describe below.

Procedure $\UpdateLevels()$ considers the nodes in $Q$ in the order of their current level. At each iteration, it takes the node $y$ with the smallest level $\ell(y)$ from $Q$. The node $y$ computes the set of potential parents $P(y)$, by examining each neighbor of $y$ in turn, and then adding to $P(y)$ all neighbors $z$ that minimize $(\ell(z) + \ww'(y,z), \pi(c(z)))$ lexicographically. Next, $y$ sets $p(y)$ as one of nodes in $P(y)$, and updates its level by setting $\ell(y) = \ell(p(y)) + \ww'(y,p(y))$. Having computed its parent pointer, $y$ updates the cluster pointer using Observation~\ref{obs: clusterUpdate}. Specifically, if the parent of $y$ is the source node $v$, then $y$ form a new cluster itself, i.e., $c(y) = y$. Otherwise, $y$ shares the same cluster with its parent and sets $c(y) = c(p(y))$. Finally, the algorithm determines whether the change in the clustering of $y$ affected its neighbors. Concretely, for each neighbor $x$ of $y$, it checks whether $y \in P(x)$. If this is not the case, then there is no change in the clustering of $x$. Otherwise, $y$ is removed from $P(x)$, and if $P(x)$ becomes empty after this removal, the algorithm inserts $x$ into the heap $Q$ with key $\ell(x)$, given that $Q$ does not already contain $x$. 

\paragraph*{Running Time Analysis.}

We first concern ourselves with the number of cluster change per node in our decremental algorithm. For any node $v \in V$, we say that the clustering \emph{changes} for~$v$ due to an edge deletion if this deletion either increases the level $\ell(v)$ or forces a change in the cluster pointer $c(v)$. It is well-known that the ES-tree can handle a level increase for any node $v$ in time $O(\deg(v))$. As we will see next, we can also handle a cluster change for a node in the same level in $O(\deg(v) \log n )$ time. However, we need to ensure that the number of such cluster changes for any node and any fixed level is small, for our algorithm to be efficient. Below we argue that one can have a fairly good bound on the expected number of such changes, and this is due to the special tie-breaking scheme we use when assigning nodes to clusters.

Fix any node $v \in V$, and consider $v$ during the sequence of edge deletions. Note that since only deletions are allowed, the level $\ell(v)$ is non-decreasing. This induces a natural partitioning of the sequence of edge deletions into subsequences such that the $\ell(v)$ remains unaffected during each subsequence. Specifically, for every node $v \in V$ and every $0 \leq i \leq \Delta$, let $S(i)$ the be subsequence of edge deletions during which $\ell(v) = i$, where $\Delta \leq O(\log n / \beta)$. The following bound on the expected number of cluster changes of $v$ during $S(i)$ follows an argument by Baswana et al.~\cite{BaswanaKS12}.

\begin{lemma} \label{lem: nrClusterChanges}
For every node $ v \in V$ and every $0 \leq i \leq \Delta$, during the entire subsequence $S(i)$, the cluster $c(v)$ of $v$ changes at most $O(\log n)$ times, in expectation.
\end{lemma}
\begin{proof}
Let $N_{i-1}(v)$ be the neighbors of $v$ at level $(i-1)$, grouped according to the the clusters they belong to. This grouping naturally induces a family $\mathcal{P}$ of all potential parents sets $P$ of $v$ at level $(i-1)$, just before the beginning of subsequence $S(i)$.
%Let $\mathcal{P}$ be the family of potential parents sets $P$ of $v$ at level $(i-1)$, grouped according to the clusters they belong to, just before the beginning of subsequence $S(i)$. 
Let $C$ be the set of the corresponding clusters centers, i.e., for each $P \in \mathcal{P}$ add $c(P)$ to $C$, and note that $v$ can only join those centers during $S(i)$. Since we are considering only edge deletions, observe that when $v$ leaves a cluster centred at some node $c \in C$, it cannot join later the same cluster $c$ during $S(i)$.  

We next bound the number of cluster changes. For each $c \in C$, there must exist an edge in the subsequence $S(i)$ whose deletion increases $\dist(v,c)$, and thus $c$ is no longer a valid cluster center for $v$ at level $i$. The latter is also equivalent to some $P$ with $c(P) = c$ becoming empty after this edge deletion. Let $\langle c_1,\ldots,c_t \rangle$ be the sequence of nodes of $C$ \emph{ordered} according to the time when $v$ has no edge to a node in $P_j$, $1 \leq j \leq t$. We want to compute the probability that $v$ ever joins the cluster centred at $c_j$ during $S(i)$. Note that this event is a consequence of $v$ changing its current cluster center $c_{j'}$ due to all parents in $P(j')$ increasing their level. According to our tie-breaking scheme in $(\ref{eq: breakingTies})$, for this to happen, $c_j$ must be the first among all potential cluster centers $\{c_j,\ldots,c_t\}$ in the random permutation~$\pi$. 
%By definition of $\fraction()$, the probability that any two fractional values are equal is $0$. 
Since $\pi$ is a uniform random permutation, the probability that $c_j$ appears first is $1/(t-j+1)$. By linearity of expectation, the expected number of centers from $C$ whose clusters $v$ joins during $S(i)$ is $\sum_{j=1}^{t} \frac{1}{t-j+1} = O(\log t) = O(\log n)$. This also bounds the number of cluster changes of $v$ during $S(i)$. 
\end{proof}


We next bound the total update time of our decremental algorithm, and also give a bound on the total number of inter-cluster edges during its execution. 

\begin{theorem}\label{thm:decremental decomposition}
There is a decremental algorithm for maintaining a $ (\fract, O (\tfrac{\log{n}}{\fract})) $-decomposition with at most $ O (\fract n) $ clusters (in expectation) containing non-isolated nodes under a sequence of edge deletions in expected total update time $ O (m \log^3 n / \fract) $ such that, over all deletions, each edge becomes an inter-cluster edge at most $ O (\log^2 n) $ times in expectation.
\end{theorem}
\begin{proof}
In a preprocessing step, we first repeat the sampling of the shift values until the maximum shift value is $ \log n/\beta $.
This event happens with probability $1-1/n$ (compare Theorem~\ref{thm: Miller_LDD}) and thus, by the waiting time bound, we need to repeat the sampling only a constant number of times.
Therefore, this preprocessing takes time $ O (n) $, which is subsumed in our claimed bound on the total update time.

We first note that procedure $\Initialize()$ can be implemented in $O (m \log n)$ time. This is because (1) the data-structures $\ell(\cdot), p(\cdot)$ and $c(\cdot)$ are initialized using Algorithm~\ref{alg:ModDijkstra} whose running time is bounded by $O (m \log n)$, (2) for each $u \in V$, the set $P(u)$ can by computed in $O(\deg (u))$ time, which in turn gives that all such sets can be determined in $\sum_{u \in V} O(\deg(u)) = O(m)$ time.

We next analyze the total time over the sequence of all edge deletions. Consider procedure $\Delete(u,v)$ for deletion of an edge $(u,v)$. If edge $(u,v)$ does not lead to a change in the clustering of one of its endpoints, then it can be processed in $O(1)$ time. Otherwise, the end-point whose clustering has changed is inserted into heap $Q$, which can be implemented in $O(\log n)$ time. Now, observe that the computation time spent by procedure $\Delete(u,v)$ is bounded by the number of nodes processed by heap $Q$ after the deletion of edge $(u,v)$, during procedure $\UpdateLevels()$. By construction, the processed nodes are precisely those whose clustering has changed due to the deletion of $(u,v)$, and after the processing, their new clustering its computed. A node $y$ extracted from $Q$ is processed in $O(\deg(y) \log n)$ time, as we will shortly argue. Therefore, we conclude that over the entire sequence of edge deletions, a node $y$ will perform $O(\deg(y) \log n)$ amount of work, each time its clustering changes. By Lemma~\ref{lem: nrClusterChanges}, as long as the level of $y$ is not increased, the clustering of $y$ will change $O(\log n)$ times, in expectation. Since there are at most $\Delta = O(\log n / \beta)$ levels, the expected number of cluster changes for $y$ is bounded by $O((\log^{2} n) / \beta)$. As our analysis applies to any node $y \in V$, we conclude that the expected total update time of our decremental algorithm is
\begin{equation} \label{eqn: runningTime}
	\sum_{y \in V} O \left((\deg(y) \log^3 n) / \beta \right) = O\left((m \log^{3} n / \beta)\right) \, .
\end{equation}

To show our claim that each node $y$ extracted from $Q$ is processed in time $O(\deg(y) \log n)$, we need two observations. First, recall that $P(y)$ can be computed in $O(\deg(y))$ time, and thus the data-structures $\ell(\cdot), p(\cdot)$ and $c(\cdot)$ can be then updated in $O(1)$ time. Second, in the worst-case, $y$ affects the clustering of all its neighbors and inserts them into $Q$. This step can be implemented in $O(\deg(y) \log n)$ time.

We finally show that each edge becomes an inter-cluster edge at most $ O (\log^2 n) $ times in expectation.
Fix some arbitrary edge $ e = (x, y) $ and consider the graph $ G $ after an arbitrary number of the adversary's deletions.
We first formulate a necessary condition for $ e $ being an inter-cluster edge and give a bound on the probability of the corresponding event.
Let $ w $ denote the mid-point of $ e $, i.e., the imaginary node in the ``middle'' of edge $ e $ that is at distance $ \tfrac{1}{2} $ to both $ u $ and~$ v $.
Let $ m_{c(x)}(w) $ and $ m_{c(y)}(w) $ denote the shifted distance from $ w $ to $ c (x) $ and $ c (y) $ in $ G $, respectively.
We would like to argue that both $ m_{c(x)}(w) $ and $ m_{c(y)}(w) $ are close to the minimum shifted distance of the mid-point $ w $.
However, we cannot readily apply Lemma~\ref{lem:inter cluster edge implies mid-point condition} as our algorithm does not run on~$ G $; instead it runs on~$ G' $, in which the edge weights are rounded to integers.
However, we can apply Lemma~\ref{lem:inter cluster edge implies mid-point condition} on $ G' $ and get that $ \floor{m_{c(x)}(w)} $ and $ \floor{m_{c(y)}(w)} $ are within $ 1 $ of the minimum rounded shifted distance of the mid-point $ w $.
Thus, $ | \floor{m_{c(x)}(w)} - \floor{m_{c(y)}(w)} | \leq 1 $, which implies that $ | m_{c(x)}(w) - m_{c(y)}(w) | \leq 2 $.
This means that $ | m_{c(x)}(w) - m_{c(y)}(w) | \leq 2 $ is a necessary condition for $ e = (x, y) $ to be an inter-cluster edge.
As the adversary is oblivious to the random choices of our algorithm, we know by Lemma~\ref{lem:probability of mid-point condition} that $ \Pr [| m_{c(x)}(w) - m_{c(y)}(w) | \leq 2 ] \leq 2 \beta $ in each of the graphs created by the adversary's sequence of deletions.

Observe that for each of the endpoints ($ x $ and~$ y $) of $ e $ the level in our decremental algorithm is non-decreasing.
Let $ 0 \leq i \leq \Delta $, and let $ S (i) $, say of length~$ t $, be the (possibly empty) subsequence of edge deletions during which $ \ell (x) = i $.
We show below that the expected number of times that $ e $ becomes an inter-cluster edge during deletions in $ S (i) $ is $ O (\beta \log{n}) $.
It then follows that the total number times $ e $ becomes an inter-cluster edges is $ O (\log^2{n}) $ by linearity of expectation: sum up the number of times $ e $ becomes an inter-cluster edge in each subsequence $ S (i) $ for $ 0 \leq i \leq \Delta $ where $ \Delta \leq O (\log{n} / \beta) $, and repeat the argument for the other endpoint $ y $ of $ e $ as well.

For every $ 1 \leq j \leq t $ define the following events:
\begin{itemize}
\item $ A_j $ is the event that $ e $ becomes an inter-cluster edge after the $j$-th deletion in $ S (i) $, and was not an inter-cluster edge directly before this deletion.
\item $ B_j $ is the event that at least one of the endpoints of $ e $, $ x $ or $ y $, changes its cluster after the $j$-th deletion in $ S (i) $.
\item $ C_j $ is the event that $ e $ is an inter-cluster edge after the $j$-th deletion in $ S (i) $.
\item $ D_j $ is the event that $ | m_{c(x)}(w) - m_{c(y)}(w) | \leq 2 $ after the $j$-th deletion in $ S (i) $, where $ w $ is the mid-point of $ e $.
\end{itemize}

Note that $ e $ can only become an inter-cluster edge if at least one of its endpoints changes its cluster.
Thus, the event~$ A_j $ implies the event $ B_j \wedge C_j $ and therefore $ \Pr [A_j] \leq \Pr [B_j \wedge C_j] $.
Furthermore, by Lemma~\ref{lem:inter cluster edge implies mid-point condition}, the event $ C_j $ implies the event $ D_j $.
We thus have $ \Pr [B_j \wedge C_j] \leq \Pr [B_j \wedge D_j] $.
Observe that the event $ D_j $ only depends on the random choice of the shift values $ \delta $ and that, in the fixed subsequence of deletions $ S (i) $, the event $ B_j $ only depends on the random choice of the permutation~$ \pi $.
Thus, $ B_j $ and $ D_j $ are independent and therefore $ \Pr [B_j \wedge D_j] = \Pr [B_j] \cdot \Pr [D_j] $.
Finally, note that the expected number of indices $ j $ such that the event $ B_j $ happens is at most the expected number of cluster changes for both endpoints of $ e $, as bounded by Lemma~\ref{lem: nrClusterChanges}, and thus $ \sum_{1 \leq i \leq t} \Pr [B_j] = O (\log n) $ for the random permutation~$ \pi $.
It follows that the expected number of times edge $ e $ becomes an inter-cluster edge (i.e., the expected number of indices $ j $ such that event $ A_j $ happens) is
\begin{align*}
\sum_{1 \leq i \leq t} \Pr [A_j] & \leq \sum_{1 \leq i \leq t} \Pr [B_j \wedge C_j] \leq \sum_{1 \leq i \leq t} \Pr [B_j \wedge D_j] = \sum_{1 \leq i \leq t} \Pr [B_j] \cdot \Pr [D_j] \\ 
& \leq \sum_{1 \leq i \leq t} \Pr [B_j] \cdot 2 \beta = 2\beta \cdot \sum_{1 \leq i \leq t} \Pr [B_j] = O (\beta \log{n}) \, ,
\end{align*}
where the penultimate inequality follows from Lemma~\ref{lem:probability of mid-point condition}.
\end{proof}

Note that in this proof, to bound the number total number of inter-cluster edges, we exploited that our two sources of randomness, the random shifts~$ \delta $ and the random permutation~$ \pi $ have different purposes: $ \delta $ influences whether an edge $ e $ is an inter-cluster edge and $ \pi $ influences the number of cluster changes of the endpoints of $ e $.
We have deliberately set up the algorithm in such a way that the independence of the corresponding events can be exploited in the proof.
This is the reason why we explicitly introduced a new random permutation for tie-breaking instead of using the random shifts for this purpose as well.
\begin{remark} \label{remark: LDDrunningTime}
Note that Equation~(\ref{eqn: runningTime}) implies that the total expected update time of Theorem~\ref{thm:decremental decomposition} is $O(m \log^{3} n / \beta)$. For the sake of exposition, we have implemented the ES-tree using a heap, which introduces a $O(\log n)$ factor in the running time. \cite{King99} (Section~2.1.1) gives a faster implementation of the ES-tree that eliminates this extra $O(\log n)$ factor. Thus, using her technique, we can also bring down our running time to $O(m \log^{2} n / \beta)$. This improvement will be particularly useful when applying our dynamic low-diameter decomposition to the construction of dynamic spanners in Section~\ref{sec:spanner}.
\end{remark}


\begin{algorithm2e}[htb!]
\caption{Modified ES-tree}
\label{alg:ES_tree}

\tcp{\textrm{The modified ES-tree is formulated for weighted undirected graphs.}}
\BlankLine

\tcp{\textrm{Internal data structures:
\begin{itemize}
\item $ \pi $: random permutation on $V$
\item $ \delta_v $: random shift of $ v $
\item $ P (v) $: the set of potential parents in the tree
\item $ p (v) $: for every node $ v $ a pointer to its parent in the tree
\item $ c (v) $: for every node $ v $ a pointer to the cluster center
\item $ Q $: global heap whose intended use is to store nodes whose levels might need to be updated
\end{itemize}
}}
\vspace{-3ex}

\BlankLine

\Procedure{\Initialize{}}{
	Initialize using Algorithm~\ref{alg:ModDijkstra}\;
	Set $ \lev (v) $, $ P(v) $, $ p(v) $, $ c(v) $ for every node $ v $ accordingly\;
}

\Procedure{\Delete{$u$, $v$}}{
	\If{$ v \in P (u) $}{
		Remove $ v $ from $ P (u) $\;
		\If{$ P (u) = \emptyset$}{
			Insert $ u $ into heap $ Q $ with key $ \lev (u) $\;
			\UpdateLevels{}\;
		}
	}
}

\Procedure{\UpdateLevels{}}{
	\While{heap $ Q $ is not empty}{\label{line:while loop}
	    Take node $ y $ with minimum key $ \lev (y) $ from heap $ Q $ and remove it from $ Q $ \label{line: take y from Q}\;
		Compute $ P (y) $ as the set of neighbors $ z $ of $ y $ minimizing $ (\lev (z) + \ww (y, z), \pi(c(z))) $ lexicographically\;
		Set $ p (y) $ as one of the nodes in $ P (y) $\;
		Set $ \lev (y) = \lev (p(y)) + \ww' (y, p(y) $\;
		\eIf{$ p(y) = s $}{
			Set $ c (y) = y  $\;
		}{
			Set $ c (y) = c( p(y)) $\;
		}

		\ForEach{neighbor $ x $ of $ y $}{\label{line: update neighbors' heaps}
			\If{$ y \in P (x) $}{
				Remove $ y $ from $ P (x) $\;
				\If{$ P (x) = \emptyset$}{
					Insert $ x $ into heap $ Q $ with key $ \lev (x) $ if $ Q $ does not already contain $ x $\;
				}
			}
		}
	}
}
\end{algorithm2e}


\subsection{Fully Dynamic Low-Diameter Decomposition}\label{sec:fully dynamic LDD}

We finally show how to extend the decremental algorithm of Theorem~\ref{thm:decremental decomposition} to a fully dynamic algorithm, allowing also insertions of edges.
\begin{theorem}[Restatement of Theorem~\ref{thm:fully dynamic LDD}]
Given any unweighted, undirected multigraph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a $ (\fract, O (\tfrac{\log{n}}{\fract})) $-decomposition (with clusters of strong diameter $ O (\tfrac{\log{n}}{\fract}) $ and at most $ \beta m $ inter-cluster edges in expectation) that has expected amortized update time $ O (\log^2{n} / \fract^2) $.
A spanning tree of diameter $ O (\tfrac{\log{n}}{\fract}) $ for each cluster can be maintained in the same time bound.
The expected amortized number of edges to become inter-cluster edges after each update is $ O (\log^2{n} / \fract) $.
These guarantees hold against an oblivious adversary.
\end{theorem}

\begin{proof}
The fully dynamic algorithm proceeds in phases, starting from an empty graph.
For every $ i > 1 $, let $ m_i $ denote the number of edges in the graph at the beginning of phase $ i $.
After $ \fract m_i / 3 $ updates in the graph we end phase $ i $ and start phase $ i+1 $.
At the beginning of each phase we re-initialize the decremental algorithm of Theorem~\ref{thm:decremental decomposition} for maintaining a $ (\fract / 3, 3 \cdot O (\tfrac{\log{n}}{\fract})) $-decomposition.\footnote{Note that for the first constant number of updates this basically amounts to recomputation from scratch at each update.}
Whenever an edge is deleted from the graph, we pass the edge deletion on to the decremental algorithm.
Whenever an edge is inserted to the graph, we do nothing, i.e., we deal with insertions of edges in a completely \emph{lazy} manner.

We first analyze the ratio of inter-cluster edges at any time during phase $ i $.
First observe that the number of inter-cluster edges is at most $ 2 \fract m_i / 3 $ in expectation, where at most $ \fract m_i / 3 $ edges in expectation are contributed by the $ (\fract / 3, 3 \cdot O (\tfrac{\log{n}}{\fract})) $-decomposition of the decremental algorithm and at most $ \fract m_i / 3 $ edges are contributed from inserted edges.
Second, the number of edges in the graph is at least $ m_i - \fract m_i / 3 $, as $ m_i $ is the initial number of edges and at most $ \fract m_i / 3 $ edges have been deleted.
Thus, the ratio of inter-cluster edges is at most
\begin{equation*}
\frac{2 \fract m_i / 3}{m_i - \fract m_i/3} = \frac{2 \fract}{3 - \fract} \leq \frac{2 \fract}{2 + \fract - \fract} = \fract \, .
\end{equation*}
Our fully dynamic algorithm therefore correctly maintains a $ (\fract, O (\tfrac{\log{n}}{\fract})) $-decomposition.

We now analyze the amortized update time of the algorithm.
Start with an empty graph and consider a sequence of $ q $ updates.
Let $ k $ denote the number of the phase after the $ q $-th update.
Then $ q $ can be written as $ q = \sum_{1 \leq i < k} \fract m_i / 3 + t $, where $ t $ is the number of updates in phase $ k $.
For every phase $ i $ that has been started, we spend time $ O (m_i \log^2 n / \fract) $ by Theorem~\ref{thm:decremental decomposition} and Remark~\ref{remark: LDDrunningTime}. We know that $ t \leq \fract m_k / 3 $ and in particular we also have $ m_k \leq \sum_{1 \leq i \leq k-1} \fract m_i / 3 $ as every edge that is contained in the graph at the beginning of phase $ k $ has been inserted in one of the previous phases.
We can thus bound the amortized spent by the algorithm for $ q $ updates by
\begin{multline*}
\frac{\sum_{1 \leq i \leq k-1} O (m_i \log^2 n / \fract) + O (m_k \log^2 n / \fract)}{\sum_{1 \leq i \leq k-1} \fract m_i / 3} \\
 \leq \frac{\sum_{1 \leq i \leq k-1} O (m_i \log^2 n / \fract) + O (\sum_{1 \leq i \leq k-1} m_i \log^2 n)}{\sum_{1 \leq i \leq k-1} \fract m_i / 3} = O \left( \frac{\log^2 n}{\fract^2} \right) \, .
\end{multline*}

Finally, we analyze the amortized number of edges to become inter-cluster edges per update.
For every phase $ i $ that has been started, we have a total number of $ O (m_i \log^2 n) $ edges that become inter-cluster edges in the decremental algorithm by Theorem~\ref{thm:decremental decomposition}.
Additionally, at most $ \fract m_i / 3 = O (m_i) $ inserted edges could also become inter-cluster edges.
We can thus bound the amortized number of edges to become inter-cluster per update by
\begin{multline*}
\frac{\sum_{1 \leq i \leq k-1} O (m_i \log^2 n) + O (m_k \log^2 n)}{\sum_{1 \leq i \leq k-1} \fract m_i / 3} \\
 \leq \frac{\sum_{1 \leq i \leq k-1} O (m_i \log^2 n) + O (\sum_{1 \leq i \leq k-1} \fract m_i \log^2 n)}{\sum_{1 \leq i \leq k-1} \fract m_i / 3} = O \left( \frac{\log^2 n}{\fract} \right) \, .
\end{multline*}
\end{proof}


==> chapters/lowstretchtree/abstract.tex <==
Spanning trees of low average stretch on the non-tree edges, as introduced by Alon et al.~\cite{AlonKPW95}, are a natural graph-theoretic object. In recent years, they have found significant applications in solvers for symmetric diagonally dominant (SDD) linear systems. In this work, we provide the first dynamic algorithm for maintaining such trees under edge insertions and deletions to the input graph. Our algorithm has update time $ n^{1/2 + o(1)} $ and the average stretch of the maintained tree is $ n^{o(1)} $, which matches the stretch in the seminal result of Alon et al.

Similar to Alon et al., our dynamic low-stretch tree algorithm employs a dynamic hierarchy of low-diameter decompositions (LDDs).
As a major building block we use a dynamic LDD that we obtain by adapting the random-shift clustering of Miller et al.~\cite{MillerPX13} to the dynamic setting.
%To this end, we first develop a deletions-only algorithm that essentially is a variant of the Even-Shiloach algorithm~\citem[JACM 1981]{EvenS81}.
%This exploits the observation of Miller et al.\ that (statically) the clustering can be determined by a single-source shortest path computation.
%To avoid certain costly cluster changes in the algorithm, we enhance the clustering with a tie-breaking scheme proposed by Baswana et al.~\citem[TALG '12]{BaswanaKS12} in the context of dynamic spanners.
%We then extend our deletions-only algorithm to a fully dynamic one by a ``lazy'' update policy for insertions.
%
The major technical challenge in our approach is to control the propagation of updates within our hierarchy of LDDs: each update to one level of the hierarchy could potentially induce several insertions \emph{and} deletions to the next level of the hierarchy.
We achieve this goal by a sophisticated amortization approach.
In particular, we give a bound on the number of changes made to the LDD per update to the input graph that is significantly better than the trivial bound implied by the update time.

We believe that the dynamic random-shift clustering might be useful for independent applications.
One of these applications is the dynamic spanner problem.
By combining the random-shift clustering with the recent spanner construction of Elkin and Neiman~\cite{ElkinN17}.
We obtain a fully dynamic algorithm for maintaining a spanner of stretch $ 2k - 1 $ and size $ O (n^{1 + 1/k} \log{n}) $ with amortized update time $ O (k \log^2 n) $ for any integer $ 2 \leq k \leq \log n $.
Compared to the state-of-the art in this regime Baswana et al. \cite{BaswanaKS12}, we improve upon the size of the spanner and the update time by a factor of $ k $.


==> chapters/lowstretchtree/conclusion.tex <==
\section{Conclusion}


==> chapters/lowstretchtree/introduction.tex <==
\section{Introduction}

Graph compression is an important paradigm in modern algorithm design.
Given a graph $ G $ with $ n $ nodes, can we find a substantially smaller (read: sparser) subgraph $ H $ such that $ H $ preserves central properties of~$ G $?
Very often, this compression is ``lossy'' in the sense that the properties of interest are only preserved approximately.
A ubiquitous example of graph compression schemes are \emph{spanners}:
every graph $ G $ admits a spanner $ H $ with $ O (n^{1 + 1/k}) $ edges that has \emph{stretch}~$ 2 k - 1 $ (for any integer $ k \geq 2 $), meaning that for every edge $ e = (u, v) $ of~$ G $ not present in $ H $ there is a path from $ u $ to $ v $ in~$ H $ of length at most $ 2 k - 1 $.
Thus, when $ k = \log{n} $, very succinct compression with $ O (n) $ edges can be achieved at the price of stretch $ O (\log n) $.

The most succinct form of subgraph compression is achieved when $ H $ is a tree.
Spanning trees, for example, are a well-known tool for preserving the connectivity of a graph.
It is thus natural to ask whether, similar to spanners, one could also have spanning trees with low stretch for each edge.
This unfortunately is known to be false: in a ring of $ n $ nodes every tree will result in a stretch of $ n - 1 $ for the single edge not contained in the tree.
However, it turns out that a quite similar goal can be achieved by relaxing the concept of stretch:
every graph $ G $ admits a spanning tree $ T $ of \emph{average stretch} $ O (\log{n} \log \log n) $~\cite{AbrahamN12}, where the average stretch is the sum of the stretches of all edges divided by the total number of edges.
Such subgraphs are called \emph{low (average) stretch trees} and have found numerous applications in recent years, most notably in the design of fast solvers for symmetric diagonally dominant (SDD) linear systems~\cite{SpielmanT14,KoutisMP14,BlellochGKMPT14,KoutisMP11,KelnerOSZ13,CohenKMPPRX14}.
We believe that their fundamental graph-theoretic motivation and their powerful applications make low-stretch trees a very natural object to study as well in a dynamic setting, similar to spanners~\cite{AusielloFI06,Elkin11,BaswanaKS12,BodwinK16} and minimum spanning trees~\cite{Frederickson85,EppsteinGIN97,HenzingerK01,HolmLT01,Wulff-Nilsen17,NanongkaiSW17}.
Indeed, the design of a dynamic algorithm for maintaining a low-stretch tree was posed as an open problem by Baswana et al.~\cite{BaswanaKS12}, but despite extensive research on dynamic algorithms in recent years, no such algorithm has yet been found.

In this chapter, we give the first non-trivial algorithm for this problem in the \emph{dynamic} setting.
Specifically, we maintain a low-stretch tree $ T $ of a dynamic graph~$ G $ undergoing updates in the form of edge insertions and deletions in the sense that after each update to $ G $ we compute the set of necessary changes to $ T $.
The goal in this problem is to keep the time spent after each update small while still keeping the average stretch of $ T $ tolerable.
Our main result is a fully dynamic algorithm for maintaining a spanning tree of expected average stretch~$ n^{o(1)} $ with expected amortized update time~$ n^{1/2 + o(1)} $.
At a high level, we obtain this result by combining the classic low-stretch tree construction of Alon et al.~\cite{AlonKPW95} with a dynamic algorithm for maintaining low diameter decompositions (LDD) based on random-shift clustering~\cite{MillerPX13}.
Our LDD algorithm might be of independent interest, and we provide another application by using it to obtain a dynamic version of the recent spanner construction of Elkin and Neiman~\cite{ElkinN17}.
The resulting dynamic spanner algorithm improves upon one of the state-of-the-art algorithms by Baswana et al.~\cite{BaswanaKS12}.

Our overall approach towards the low-stretch tree algorithm -- \sloppy to use low-diameter decompositions based on random-shift clustering in the construction of Alon et al.~\cite{AlonKPW95} -- has been used before in parallel and distributed algorithms~\cite{BlellochGKMPT14,GhaffariKKLP15,HaeuplerL18}.
However, to make this approach work in the dynamic setting we need to circumvent some non-trivial challenges.
In particular, we cannot employ the following paradigm that often is very helpful in designing dynamic algorithms: design an algorithm that can only handle edge deletions and then extend it to the fully dynamic setting using a general reduction.
While we do follow this paradigm for our dynamic LDD algorithm, there are two obstacles that prevent us from doing so for the dynamic low-stretch tree:
First, many fully-dynamic-to-decremental reductions exploit some form of ``decomposability'', which does not hold for low-stretch trees, i.e., low-stretch trees of subgraphs of the input graph cannot be simply be combined to a single low-stretch tree of the full graph.
%First, there is no obvious candidate for such a fully-dynamic-to-decremental reduction.
Second, in our dynamic low-diameter decomposition edges might start and stop being inter-cluster edges, even if the input graph is only undergoing deletions.
In the hierarchy of Alon et al.\ this leads to both insertions and deletions at the next level of the hierarchy.
As opposed to other dynamic problems~\cite{HenzingerKN16,AbrahamDKKP16}, one algorithm cannot simply enforce some type of ``monotonicity'' by not passing on insertions to the next level of the hierarchy (to stay within a deletions-only setting) as there might be too many such edges to ignore them. 
%In particular, if an edge $ e $ appears as an inter-cluster edge and we do not make it available to the next level, $ e $ cannot be part of the low-stretch tree $ T $ maintained by the algorithm.
%We would then, in a separate step, continuously have to fix $ T $ to incorporate edges that have been left out.
%It is however not clear how to make such a fix while still keeping the average stretch of the tree low, in particular because there might be many such edges inserted over the course of the deletions-only algorithm.
Thus, it seems that we really have to deal with the fully dynamic setting in the first place.
We show that this can be done by a sophisticated amortization approach that explicitly analyzes the number of updates passed on to the next level.


\paragraph*{Related Work.}

Low average stretch trees have been introduced by Alon et al.~\cite{AlonKPW95} who obtained an average stretch of $ 2^{O (\sqrt{\log n \log \log n})} $ and also gave a lower bound of $ \Omega (\log n) $ on the average stretch.
The first construction with polylogarithmic average stretch was given by Elkin et al.~\cite{ElkinEST08}.
Further improvements~\cite{AbrahamBN08,KoutisMP11} culminated in the state-of-the-art construction of Abraham and Neiman~\cite{AbrahamN12} with average stretch $ O(\log n \log \log n) $.
All these trees with polylogarithmic average stretch can be computed in time $ \tilde O (m) $. To the best of our knowledge, all known algorithms in parallel and distributed models of computation~\cite{BlellochGKMPT14,GhaffariKKLP15,HaeuplerL18} are based on the scheme of Alon et al.\ and thus do not provide polylogarithmic stretch guarantees.

The main application of low-stretch trees has been in solving symmetric, diagonally dominant (SDD) systems of linear equations.
It has been observed that iterative methods for solving these systems can be made faster by preconditioning with a low-stretch tree~\cite{Vaidya91,BomanH03,SpielmanW09}.
Consequently, they have been an important ingredient in the breakthrough result of Spielman and Teng~\cite{SpielmanT14} for solving SDD systems in nearly linear time.
In this solver, low-stretch trees are utilized for constructing ultra-sparsifiers, which in turn are used as preconditioners.
Beyond this initial breakthrough, low-stretch trees have also been used in subsequent, faster solvers~\cite{KoutisMP14,BlellochGKMPT14,KoutisMP11,KelnerOSZ13,CohenKMPPRX14}.
%
Another prominent application of low-stretch trees~(concretely, the variant of random spanning trees with low expected stretch) is the remarkable cut-based graph decomposition of R\"acke~\Cite{Racke08,AndersenF09}, which embeds any general undirected graph into convex combination of spanning trees, while paying only a $\tilde{O}(\log n)$ congestion for the embedding. This decomposition tool, initially aimed at giving the best competitive ratio for oblivious routing, has found several applications ranging from approximation algorithms for cut-based problems~(e.g., minimum bisection~\cite{Racke08}) to graph compression~(e.g., vertex sparsifiers~\cite{Moitra09}). 
%
Other classic problems in the realm of approximation algorithms that utilize the properties of low-stretch trees include the $ k $-server problem~\cite{AlonKPW95} and the minimum communication cost spanning tree problem~\cite{Hu74,PelegR98}.

In terms of dynamic algorithms, we are not aware of any prior work for maintaining low-stretch trees.
The closest related works are arguably dynamic algorithms for maintaining distance oracles and spanners, as they also aim preserving pairwise distances, and dynamic algorithms for maintaining minimum spanning trees, as they also are spanning trees with an additional property.

%Regarding the motivation of solving SDD systems, the closest related result is possibly the algorithm of Abraham et al.~\cite{AbrahamDKKP16} for maintaining a spectral sparsifier with polylogarithmic update time.
%Apart from that, the problems of dynamically maintaining a spanner or a (minimum) spanning tree seem to be the most related ones.

A distance oracle is a data structure that can answer queries for the (approximate) distance between a pair of nodes.
The fully dynamic distance oracle of Abraham, Chechik, and Talwar~\cite{AbrahamCT14} for unweighted, undirected graphs has expected amortized update time $ \tilde O (\sqrt{m} n^{1/k}) $, query time $ O (k^2 \rho^2) $, and stretch $ 2^{O (k \rho)} $, where the parameter $ k \geq 2 $ is integer and $ \rho = 1 + \lceil \tfrac{\log n^{1 - 1/k}}{\log(m / n^{1 - 1/k})} \rceil $.
To the best of our knowledge, the recent decremental distance oracle of Chechik~\cite{Chechik18} can be used to extend this result to weighted graphs and to improve the stretch and the query time, while leaving the update time essentially unchanged.

For dynamic spanner algorithms, the main goal is to maintain, for any given integer $ k \geq 2 $, a spanner of stretch $ 2k - 1 $ with $ \tilde O (n^{1 + 1/k}) $ edges.
Spanners of stretch $ 2k - 1 $ and size $ O (n^{1 + 1/k}) $ exist for every undirected graph~\cite{Awerbuch85}, and this trade-off is presumably tight under Erd\H{o}s's girth conjecture.
The dynamic spanner problem has been introduced by Ausiello et al.~\cite{AusielloFI06}.
They showed how to maintain a $3$- or $5$-spanner with amortized update time proportional to the maximum degree of the graph.
Using techniques from the streaming literature, Elkin~\cite{Elkin11} provided an algorithm for maintaining a $ (2k - 1) $-spanner with $ \tilde O (m n^{-1/k}) $ expected update time.
Faster update times were achieved by Baswana et al.~\cite{BaswanaKS12}: their algorithms maintain $ (2k - 1) $-spanners either with expected amortized update time $ O(1)^k $ or with expected amortized update time $ O (k^2 \log^2 n) $.
%Recently, Bodwin and Krinninger~\cite{BodwinK16} complemented these results by giving algorithms with worst-case update times that are correct with high probability, namely update time $ O(n^{3/4}) $ for maintaining a $3$-spanner and update time $ O(n^{5/9}) $ for maintaining a $5$-spanner.
Later, Bodwin and Krinninger~\cite{BodwinK16} initiated the study of dynamic spanners with worst-case update times, and recently, Bernstein, Forster, and Henzinger~\cite{BernsteinFH19} presented a deamortization approach to maintain $ (2k - 1) $-spanners with high-probability worst-case update time $ O(1)^k \log^3 n $.
All of these algorithms exhibit the stretch/space trade-off mentioned above in unweighted graphs, up to polylogarithmic factors in the size of the spanner.
%All randomized dynamic spanner algorithms mentioned above need to assume an oblivious adversary whose chosen sequence of updates is independent of the random choices of the algorithm.
%Another class of dynamic graph sparsification algorithms has first been studied by Abraham et al.~\cite{AbrahamDKKP16} who show how to maintain cut and spectral sparsifiers with polylogarithmic update time.

The first non-trivial algorithm for dynamically maintaining a minimum spanning tree was developed by Frederickson~\cite{Frederickson85} and had a worst-case update time of $ O (\sqrt{m}) $.
Using a general sparsification technique, this bound was improved to $ O (\sqrt{n}) $ by Eppstein et al.~\cite{EppsteinGIN97}.
In terms of amortized bounds, Holm et al.~\cite{HolmLT01} were the first to improve this bound and obtained polylogarithmic amortized update time.
A recent breakthrough of Nanongkai, Saranurak, and Wulff-Nilsen~\cite{Wulff-Nilsen17,NanongkaiS17,NanongkaiSW17}, who finally achieved a \emph{worst-case} update time of $ n^{o(1)} $.

%The first non-trivial algorithm for dynamically maintaining a spanning tree (and also an MST, a minimum spanning tree) was developed by Frederickson~\cite{Frederickson85} and had a worst-case update time of $ O (\sqrt{m}) $.
%Using a general sparsification technique, this bound was improved to $ O (\sqrt{n}) $ by Eppstein et al.~\cite{EppsteinGIN97}.
%For the dynamic spanning tree problem, this barrier has first been broken by Henzinger and King~\cite{HenzingerK99} who gave a randomized algorithm with polylogarithmic \emph{amortized} update time.
%Holm et al.~\cite{HolmLT01} later showed that polylogarithmic amortized update time can be obtained deterministically, also for the dynamic MST problem.
%In terms of worst-case guarantees, Kapron et al.~\cite{KapronKM13} were the first to present an approach for polylogarithmic worst-case update time.
%The main goal of Kapron et al. was to solve the dynamic connectivity problem, but their algorithm can also only maintain a spanning tree against an oblivious adversary.
%Although there has been a significant amount of follow-up work in this area~\cite{HenzingerK01,HenzingerT97,Thorup00,Wulff-Nilsen13,GibbKKT15,HuangHKP17,Kejlberg-Rasmussen16}, the worst-case update time for the MST problem stayed at $ O (\sqrt{n}) $.
%This changed with a recent breakthrough of Nanongkai et al.~\cite{Wulff-Nilsen17,NanongkaiS17,NanongkaiSW17}, who finally achieved a worst-case update time of $ n^{o(1)} $ for maintaining an MST.
%Note that for MSTs a simple reweighting can enforce a unique solution and thus dynamic MST algorithms do not require the oblivious adversary assumption; they immediately work against an adaptive online adversary who may choose the next update after observing the output of the algorithm.


\paragraph*{Our Results.}

Our main result is a dynamic algorithm for maintaining a low average stretch tree of an unweighted, undirected graph.

\begin{theorem}\label{thm:fully dynamic low stretch tree}
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanning forest of expected average stretch $ n^{o(1)} $ that has expected amortized update time $ m^{1/2 + o(1)} $.
These guarantees hold against an oblivious adversary.
\end{theorem}

This is the first non-trivial algorithm for this fundamental problem.
Our stretch matches the seminal construction of Alon et al.~\cite{AlonKPW95}, which is still the state of the art in parallel and distributed settings~\cite{BlellochGKMPT14,GhaffariKKLP15,HaeuplerL18}.
%In terms of the adversarial model, we must assume that the adversary is oblivious, which means that its choices are independent of the random choices of our algorithm.
%There are some situations where this assumption is not justified~\cite{Madry10}, but the oblivious adversary is one of the standard models studied in this field.
%For example, all randomized dynamic spanner algorithms known so far~\cite{Elkin11,BaswanaKS12,BodwinK16} need to assume an oblivious adversary.

Similar to the approach of~\cite{KoutisLP16} in the \emph{static} setting, we can apply Theorem~\ref{thm:fully dynamic low stretch tree} to a cut sparsifier of the input graph, which has only $ \tilde O (n) $ edges, to improve the running time for dense graphs.
Such a cut sparsifier can be maintained with the dynamic algorithm of Abraham et al.~\cite{AbrahamDKKP16} that has polylogarithmic update time.

\begin{corollary}\label{cor:fully dynamic low stretch tree}
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanning forest of expected average stretch $ n^{o(1)} $ that has expected amortized update time $ n^{1/2 + o(1)} $.
These guarantees hold against an oblivious adversary.
\end{corollary}

Obtaining this improvement is non-trivial because cut sparsifiers are weighted graphs, even when the input graph is unweighted, and the algorithm of Theorem~\ref{thm:fully dynamic low stretch tree} only accepts unweighted graphs.
To deal with this issue, we deviate from the approach of~\cite{KoutisLP16} by interpreting the edge weights of the sparsifier as edge multiplicities in an unweighted graph.
A fine-grained analysis of the amount of change to edge the multiplicities per update to the input graph then allows us to get the desired benefits of combining both algorithms.

%We then show that the algorithm of Theorem~\ref{thm:fully dynamic low stretch tree} can also handle such graphs for updates that increment or decrement one edge multiplicity by $ 1 $.
%A fine-grained analysis of the total multiplicity of edges of the sparsifier and its expected amount of change per update to the input graph then gives the desired result.

We additionally show that $ \sqrt{n} $ is not an inherent barrier to the update time, at least if very large stretch is tolerated.
A modification of our algorithm gives average stretch $ O(t) $ and update time $ \tfrac{n^{1 + o(1)}}{t} $ for $ t \geq \sqrt{n} $.

One of the main building blocks of our dynamic low-stretch tree algorithm is a dynamic algorithm for maintaining a low-diameter decomposition (LDD). Roughly speaking, for $\beta \in (0,1)$ and $\diam > 0$,  a $(\beta, \diam)$-decomposition of a graph is a partitioning of its nodes into node-disjoint clusters such that (1) any pair of nodes belonging to the same cluster are at distance at most $\diam$, and (2) the number of edges whose endpoints belong to different clusters is bounded by $\beta m$. The following theorem gives a dynamic variant of such decompositions.
 
\begin{theorem}\label{thm:fully dynamic LDD}
Given any unweighted, undirected multigraph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a $ (\fract, O (\tfrac{\log{n}}{\fract})) $-decomposition (with clusters of strong diameter $ O (\tfrac{\log{n}}{\fract}) $ and at most $ \beta m $ inter-cluster edges in expectation) that has expected amortized update time $ O (\log^2{n} / \fract^2) $.
A spanning tree of diameter $ O (\tfrac{\log{n}}{\fract}) $ for each cluster can be maintained in the same time bound.
The expected amortized number of edges to become inter-cluster edges after each update is $ O (\log^2{n} / \fract) $.
These guarantees hold against an oblivious adversary.
\end{theorem}
Our algorithm is based on the random-shift clustering of Miller at al.~\cite{MillerPX13}, with many tweaks to make it work in a dynamic setting.
In our analysis of the algorithm, we bound the amortized number of changes to the clustering per update by $ \tilde O (1 / \fract) $, which is significantly smaller than the naive bound of $ \tilde O (1 / \fract^2) $ implied by the update time.
This is particularly important for hierarchical approaches, such as in our dynamic low-stretch tree algorithm, because a small bound on the number of amortized changes helps in controlling the number of induced updates to be processed within the hierarchy.
Independently, Saranurak and Wang~\cite{SaranurakW19} obtained a fully dynamic LLD algorithm with nearly the same guarantees (up to polylogarithmic factors).\footnote{The low-diameter decomposition of Saranurak and Wang can be maintained against an adaptive online adversary. However, the low-diameter spanning trees of their clustering can only be maintained against an oblivious adversary. Therefore, plugging in their dynamic LDD algorithm into our dynamic low-stretch tree construction does not yield any improvement over our guarantees.}
%We remark that, in the decremental setting, the expander decomposition and pruning techniques of Nanongkai et al.~\cite{NanongkaiSW17} will yield a result similar to Theorem~\ref{thm:fully dynamic LDD}, but with overheads of $ n^{o(1)} $~\cite{Saranurak18}.\footnote{Note that the decremental algorithm of Nanongkai et al.\ will have a stronger worst-case update time guarantee. However, this guarantee will not carry over the fully dynamic setting, at least not by using our reduction in Section~\ref{sec:fully dynamic LDD}, which to the best of our understanding cannot be de-amortized with standard techniques.}
We believe that our solution is arguably simpler than their expander pruning approach.

The dynamic random-shift clustering underlying our dynamic LDD is of independent interest.
A direct consequence demonstrating the usefulness of our dynamic random-shift clustering algorithm is the following new result for the dynamic spanner problem.
\begin{theorem}\label{thm:fully dynamic spanner}
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanner of stretch $ 2k - 1 $ and expected size $ O (n^{1 + 1/k} \log{n}) $ that has expected amortized update time $ O (k \log^2{n}) $.
These guarantees hold against an oblivious adversary.
\end{theorem}
Recall that the fully dynamic algorithm of Baswana et al.~\cite{BaswanaKS12} maintains a spanner of stretch $ 2k - 1 $ and expected size $ O (k n^{1 + 1/k} \log n) $ with expected amortized update time $ O (k^2 \log^2{n}) $.
Our new algorithm thus improves both the size and the update time by a factor of~$ k $.
This is particularly relevant because the stretch/size trade-off of $ 2k - 1 $ vs.\ $ O (n^{1 + 1/k}) $ is tight under the girth conjecture.
We thus exceed the conjectured optimal size by a factor of only $ \log{n} $ compared to the prior $ k \log{n} $, where $ k $ might be as large as $ \log n $.
When we restrict ourselves to the decremental setting, we do achieve size $ O (n^{1 + 1/k}) $ with expected amortized update time $ O (k \log{n}) $.
Again, this saves a factor of~$ k $ compared to Baswana et al.~\cite{BaswanaKS12}.
To obtain Theorem~\ref{thm:fully dynamic spanner}, we employ our dynamic random-shift clustering algorithm in the spanner construction of Elkin and Neiman~\cite{ElkinN17} and combine it with the dynamic spanner framework of Baswana et al.~\cite{BaswanaKS12}.
%We believe that this application is another demonstration of the usefulness of our dynamic random-shift clustering algorithm.


\paragraph*{Structure of this Chapter.}

The remainder of this chapter is structured as follows.
We first settle the notation and terminology in Section~\ref{sec:prelim}.
We then give a high-level overview of our results and techniques in Section~\ref{sec:overview}.
Finally, we provide all necessary details for our dynamic low-stretch tree (Section~\ref{sec:low_stretch_tree}), our dynamic low-diameter decomposition (Section~\ref{sec:LDD}), and our dynamic spanner algorithm (Section~\ref{sec:spanner}).


==> chapters/lowstretchtree/low_stretch_tree.tex <==
\section{Dynamic Low Average Stretch Forest}\label{sec:low_stretch_tree}

Our dynamic algorithms for maintaining a low average stretch forest will use a hierarchy of low-diameter decompositions.
We first analyze very generally the update time for maintaining such a decomposition and explain how to obtain a spanning forest from this hierarchy in a natural way, similar to the construction of Alon et al.~\cite{AlonKPW95}.
We then analyze two different approaches for maintaining the tree, which will give us two complementary points in the design space of dynamic low-stretch tree algorithms.
Finally, we explain how to exploit input graph sparsification to improve the update time of our first algorithm.


\subsection{Generic Dynamic LDD Hierarchy}

Consider some integer parameter $ k \geq 1 $ and parameters $ \fract_0, \ldots, \fract_{k-1} \in (0, 1) $.
For each $ 0 \leq i \leq k-1 $, let $ \mathcal{D}_i $ be the fully dynamic algorithm for maintaining a $ (\fract_i, O (\tfrac{\log{n}}{\fract_i})) $-decomposition as given by Theorem~\ref{thm:fully dynamic LDD}.
Our \emph{LDD-hierarchy} consists of $ k+1 $ multigraphs $ G_0 = (V, E_0), \ldots, G_k = (V, E_k) $ where $ G_0 $ is the input graph $ G $ and, for each $ 0 \leq i \leq k-1 $, the graph $ G_{i+1} $ is obtained from contracting $ G_i $ according to a $ (\beta_i, O (\tfrac{\log{n}}{\fract_i}))$-decomposition of $ G_i $ as follows:
For every node $ v \in V $, let $ c_i (v) $ denote the center of the cluster to which $ v $ is assigned in the $ (\beta_i, O (\tfrac{\log{n}}{\fract_i}))$-decomposition of $ G_i $.
Now define $ E_{i+1} $ as the multiset of edges containing for every edge $ (u, v) \in E_i $ such that $ c_i (u) \neq c_i (v) $ one edge $ (c_i (u), c_i (v)) $, i.e., $ E_{i+1} = \{ (c_i (u), c_i (v)) : (u, v) \in E_i \text{ and } c_i (u) \neq c_i (v) \} $, where the multiplicity of each edge is equal to the number of edges between the corresponding clusters in~$ G_i $.
Remember that all graphs~$ G_i $ have the same set of nodes, but nodes that do not serve as cluster centers in $ G_{i-1} $ will be isolated in $ G_i $.
It might seem counter-intuitive at first that these isolated nodes are not removed from the graph, but observe that in our dynamic algorithm nodes might start or stop being cluster centers over time.
By keeping all nodes in all subgraphs, we avoid having to explicitly deal with insertions or deletions of nodes.\footnote{Note that it is easy to explicitly maintain the sets of isolated and non-isolated nodes by observing the degrees.}

Note that the $ (\fract_i, O (\tfrac{\log{n}}{\fract_i})) $-decomposition of $ G_i $ guarantees that $ | E_{i+1} | \leq \beta_i \cdot | E_i | $ in expectation, which implies the following bound.

\begin{observation}\label{obs:number of nodes and edges}
For every $ 0 \leq i \leq k $, $ |E_i| \leq m \cdot \prod_{0 \leq j \leq i - 1} \beta_j $ in expectation.\footnote{Note that for $ i = 0 $ the product $ \prod_{0 \leq j \leq i-1} \fract_j $ is empty and thus equal to $ 1 $.}
\end{observation}

We now analyze the update time for maintaining this LDD-hierarchy under insertions and deletions to the input graph~$ G $.
Note that for each level~$ i \leq k - 1 $ of the hierarchy, changes made to the graph $ G_i $ might result in the dynamic algorithm~$ \mathcal{D}_i $ making changes to the $ (\fract_i, O (\tfrac{\log{n}}{\fract_i})) $-decomposition of $ G_i $.
In particular, edges of $ G_i $ could start or stop being inter-cluster edges in the decomposition, which in turn leads to edges being added to or removed from~$ G_{i + 1} $.
Thus, a single update to the input graph~$ G $ might result in a blow-up of induced updates to be processed by the algorithms $ \mathcal{D}_1, \ldots, \mathcal{D}_{k -1} $.
To limit this blow-up, we use an additional property of our LDD-decomposition given in Theorem~\ref{thm:fully dynamic LDD}, namely the non-trivial bound on the number of edges to become inter-cluster edges after each update.

\begin{lemma}\label{lem:update time hierarchy}
The LDD-hierarchy can be maintained with an expected amortized update time of
\begin{equation*}
\tilde O \left( \sum_{0 \leq j \leq k-1} \frac{ O (\log n)^{2 (k-1)} }{\fract_j \prod_{0 \leq j' \leq j} \fract_{j'}} \right) \, .
\end{equation*}
\end{lemma}

\begin{proof}
For every $ 0 \leq i \leq k - 1 $ and every $ q \geq 1 $ define the following random variables:
\begin{itemize}
\item $ X_i (q) $: The total time spent by algorithm $ \mathcal{D}_i $ for processing any sequence of $ q $~updates to~$ G_i $.
\item $ Y_i (q) $: The total number of changes performed to $ G_{i+1} $ by $ \mathcal{D}_i $ while processing any sequence of $ q $~updates to~$ G_i $.
\item $ Z_i (q) $: The total time spent by algorithms $ \mathcal{D}_i, \ldots, \mathcal{D}_{k-1} $ for processing any sequence of $ q $~updates to~$ G_i $.
\end{itemize}
Note that the expected values of $ X_i (q) $ and $ Y_i (q) $ are bounded by Theorem~\ref{thm:fully dynamic LDD}~(the latter holds since only changes involving inter-cluster edges are propagated as updates to the next level).
We will show by induction on $ i $ that $ E [Z_i (q)] = \tilde O (q \cdot \sum_{i \leq j \leq k-1} \tfrac{ O (\log n)^{2(k-i-1)} }{\fract_j \prod_{i \leq j' \leq j} \fract_{j'}}) $, which with $ i = 0 $ implies the claim we want to prove.

Before showing the proof, observe that our LDD-hierarchy uses multiple instances of the dynamic low-diameter decomposition. We can order these instances in a hierarchical manner such that changes in the instance $i$ only affect instances $i+1$ and above (this is possible because all changes propagate one way through the hierarchy). Since the random bits among levels are independent, we can think of the random bits in the previous level being fixed in advance, and hence the updates to the instance $i$ are fixed as well. The latter implies that each instance $i$ in the LDD-hierarchy is running in the oblivious adversary setting, as required by Theorem~\ref{thm:fully dynamic LDD}.

We next prove the claimed bound on $E [Z_i (q)]$. In the base case $ i = k - 1 $, we know by Theorem~\ref{thm:fully dynamic LDD} that algorithm $ \mathcal{D}_{k-1} $ maintaining the $ (\fract_{k - 1}, O (\tfrac{\log{n}}{\fract_{k - 1}})) $-decomposition of $ G_{k-1} $ spends expected amortized time $ \tilde O (\frac{1}{\fract_{k-1}^2}) $ per update to $ G_{k-1} $, i.e., $ E [Z_{k - 1} (q)] = E [X_{k - 1} (q)] = \tilde O (q \cdot \frac{1}{\fract_{k-1}^2}) $ for any $ q \geq 1 $.
For the inductive step, consider some $ 0 \leq i < k - 1 $ and any $ q \geq 1 $.
Any sequence of $ q $ updates to $ G_i $ induces at most $ Y_i (q) $ updates to $ G_{i + 1} $.
Each of those updates has to be processed by the algorithms $ \mathcal{D}_{i+1}, \ldots, \mathcal{D}_{k-1} $.
We thus have $ Z_i (q) = X_i (q) + Z_{i+1} (Y_i (q)) $.

To bound $ E [Z_i (q)] $, recall first the expectations of the involved random variables.
As by Theorem~\ref{thm:fully dynamic LDD} the algorithm~$ \mathcal{D}_i $ maintaining the $ (\fract_i, O (\tfrac{\log{n}}{\fract_i})) $-decomposition of $ G_i $ has expected amortized update time $ \tilde O (\tfrac{1}{\fract_i^2}) $, it spends an expected total time of $ E [X_i (q)] = \tilde O (q \cdot \tfrac{1}{\fract_i^2}) $ for any sequence of $ q $ updates to $ G_i $.
Furthermore, over the whole sequence of $ q $~updates, the expected number of edges to ever become inter-cluster edges in the $ (\fract_i, O (\tfrac{\log{n}}{\fract_i})) $-decomposition of $ G_i $ is $ O (q \cdot \tfrac{ \log^2 n }{\fract_i}) $.
This induces at most $ O (q \cdot \tfrac{ \log^2 n }{\fract_i}) $ updates (insertions or deletions) to the graph $ G_{i+1} $, i.e., $ E [Y_i (q)] = O (q \cdot \tfrac{ \log^2 n }{\fract_i}) $.
By the induction hypothesis, the expected amortized update time spent by $ \mathcal{D}_{i+1}, \ldots, \mathcal{D}_{k-1} $ for any sequence of $ q' $ updates to $ G_{i+1} $ is $ E [Z_{i+1} (q')] = \tilde O (q' \cdot \sum_{i + 1 \leq j \leq k-1} \tfrac{ O (\log n)^{2(k-i-2)} }{\fract_j \prod_{i + 1 \leq j' \leq j} \fract_{j'}}) $.

Now by linearity of expectation we get
\begin{equation*}
E [Z_i (q)] = E \left[ X_i (q) + Z_{i+1} (Y_i (q)) \right] = E \left[ X_i (q) \right] + E \left[ Z_{i+1} (Y_i (q)) \right]
\end{equation*}
and by the law of total expectation we can bound $ E \left[ Z_{i+1} (Y_i (q)) \right] $ as follows:
\begin{align*}
E \left[ Z_{i+1} (Y_i (q)) \right] &= \sum_y E \left[ Z_{i+1} (Y_i (q)) \mid Y_i (q) = y \right] \cdot \Pr [Y_i (q) = y] \\
 &= \sum_y E \left[ Z_{i+1} (y) \right] \cdot \Pr [Y_i (q) = y] \\
 &= \sum_y \tilde O \left( y \cdot \sum_{i + 1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-2)} }{\fract_j \prod_{i + 1 \leq j' \leq j} \fract_{j'}} \right) \cdot \Pr [Y_i (q) = y] \\
 &= \tilde O \left( \sum_{i + 1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-2)} }{\fract_j \prod_{i + 1 \leq j' \leq j} \fract_{j'}} \right) \cdot \sum_y y \cdot \Pr [Y_i (q) = y] \\
 &= \tilde O \left( \sum_{i + 1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-2)} }{\fract_j \prod_{i + 1 \leq j' \leq j} \fract_{j'}} \right) \cdot E [Y_i (q)] \\
 &= \tilde O \left( \sum_{i + 1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-2)} }{\fract_j \prod_{i + 1 \leq j' \leq j} \fract_{j'}} \right) \cdot O \left( q \cdot \frac{ \log^2 n }{\fract_i} \right) \\
 &= \tilde O \left( q \cdot \sum_{i+1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-1)} }{\fract_j \prod_{i \leq j' \leq j} \fract_{j'}} \right)
\end{align*}
We thus get
\begin{align*}
E [Z_i (q)] & = \tilde O (q \cdot \tfrac{1}{\fract_i^2}) + \tilde O \left( q \cdot \sum_{i+1 \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-1)} }{\fract_j \prod_{i \leq j' \leq j} \fract_{j'}} \right) \\ 
            & = \tilde O \left( q \cdot \sum_{i \leq j \leq k-1} \frac{ O (\log n)^{2(k-i-1)} }{\fract_j \prod_{i \leq j' \leq j} \fract_{j'}} \right)
\end{align*}
as desired.
\end{proof}

Given any spanning forest $ T' $ of $ G_k $, there is a natural way of defining a spanning forest~$ T $ of~$ G $ from the LDD-hierarchy.
To this end, we first formally define the contraction of a node $ v $ of $ G $ to a cluster center $ v' $ of $ G_i $ (for $ 0 \leq i \leq k) $ as follows:
Every node $ v $ of $ G $ is contracted to itself in $ G_0 $, and, for every $ 1 \leq i \leq k $, a node $ v $ of $ G $ is contracted to $ v' $ in $ G_i $ if $ v $ is contracted to $ u' $ in $ G_{i-1} $ and $ c_{i-1} (u') = v' $.
Similarly, for every $ 0 \leq i \leq k $, an edge $ e = (u, v) $ of $ G $ is contracted to an edge $ e' = (u', v') $ of $ G_i $ if $ u $ is contracted to $ u' $ and $ v $ is contracted to $ v' $.
Now define $ T $ inductively as follows:
We let $ T_0 $ be the forest consisting of the spanning trees of diamteter $ O (\tfrac{\log{n}}{\fract_0}) $ of the clusters in the $ (\fract_0, O (\tfrac{\log{n}}{\fract_0}))$-decomposition of $ G_0 $.
For every $ 1 \leq i \leq k $, we obtain $ T_i $ from $ T_{i-1} $ and a $ (\fract_i, O(\tfrac{\log{n}}{\fract_i})) $-decomposition of $ G_i $ as follows: for every edge $ e' $ in a shortest path tree in one of the clusters, we include in $ T_i $ \emph{exactly one} edge $e$ of $G$ among the edges that are contracted to $ e' $ in $ G_i $.
Finally, $ T $ is obtained from $ T_k $ as follows: for every edge~$ e' $ in the spanning forest~$ T' $ of~$ G_k $, we include in~$ T $ the edge~$ e $ of~$ G $ contracted to~$ e' $ in~$ G_k $.
As the clusters in each decomposition are non-overlapping, we are guaranteed that $ T $ is indeed a forest.
Note that, apart from the time needed to maintain $ T' $, we can maintain $ T $ in the same asymptotic update time as the LDD-hierarchy (up to logarithmic factors).

We now partially analyze the stretch of $ T $ with respect to $ G $.

\begin{lemma}\label{lem:path length for nodes in same cluster}
For every $ 1 \leq i \leq k $, and for every pair of nodes $ u $ and~$ v $ that are contracted to the same cluster center in $ G_i $, there is a path from $ u $ to $ v $ in $ T $ of length at most $ \tfrac{O(\log{n})^i}{\prod_{0 \leq j \leq i-1} \fract_j} $.
\end{lemma}

\begin{proof}
The proof is by induction on~$ i $.
The induction base $ i = 1 $ is straightforward:
For $ u $ and $ v $ to be contracted to the same cluster center in $ G_1 $, they must be contained in the same cluster~$ C $ of the $ (\fract_0, O (\tfrac{\log{n}}{\fract_0})) $-decomposition of $ G_0 $ maintained by $ \mathcal{D}_0 $.
Remember that $ C $ has strong diameter at most $ O (\tfrac{\log{n}}{\fract_0}) $.
Thus, in the shortest path tree of $ C $ there is a path of length at most $ O (\tfrac{\log{n}}{\fract_0}) $ from $ u $ to $ v $ using edges of $ G_0 = G $.
By the definition of $ T $, this path is also present in $ T $.

For the inductive step, let $ 2 \leq i \leq k $ and let $ u' $ and $ v' $ denote the cluster centers to which $ u $ and $ v $ are contracted in $ G_{i - 1} $, respectively.
For $ u $ and $ v $ to be contracted to the same cluster center in $ G_i $, $ u' $ and $ v ' $ must be contained in the same cluster~$ C $ of the $ (\fract_{i - 1}, O (\tfrac{\log{n}}{\fract_{i - 1}})) $-decomposition of $ G_{i - 1} $ maintained by $ \mathcal{D}_{i - 1} $.
As $ C $ has strong diameter at most $ O (\tfrac{\log{n}}{\fract_{i - 1}}) $, there is a path $ \pi $ from $ u' $ to $ v' $ of length at most $ O (\tfrac{\log{n}}{\fract_{i - 1}}) $ in the shortest path tree of $ C $.
Let $ x_1, \ldots, x_t $ denote the nodes on $ \pi $, where $ x_1 = u' $ and $ x_t = v' $.
By the definition of our tree $T$ with respect to $ G $, there must exist edges $ (a_1, b_1), \ldots, (a_t, b_t) $ of~$ G $ such that
\begin{itemize}
\item $ (a_\ell, b_\ell) $ is contained in $ T $ for all $ 1 \leq \ell \leq t $,
\item $ u $ and $ a_1 $ are contracted to the same cluster center in $ G_{i-1} $,
\item $ b_t $ and $ v $ are contracted to the same cluster center in $ G_{i-1} $, and
\item $ b_\ell $ and $ a_{\ell+1} $ are contracted to the same cluster center in $ G_{i-1} $ for all $ 1 \leq \ell \leq t - 1 $.
\end{itemize}
By the induction hypothesis we know that for every $ 1 \leq \ell \leq t-1 $ there is a path of length at most $ \tfrac{O (\log{n})^{i - 1}}{\prod_{0 \leq j \leq i-2} \fract_j} $ from $ b_\ell $ to $ a_{\ell+1} $ in $ T $.
Paths of the same maximum length also exist from $ u $ to $ a_1 $ and from $ b_t $ to $ v $.
It follows that there is a path from $ u $ to $ v $ in $ T $ of length at most
\begin{align*}
(t + 1) \cdot \frac{O (\log{n})^{i - 1}}{\prod_{0 \leq j \leq i-2} \fract_j} + t & \leq 3 t \cdot \frac{O (\log{n})^{i - 1}}{\prod_{0 \leq j \leq i-2} \fract_j} \\
 & = O \left( \frac{\log{n}}{\fract_i} \right) \cdot \frac{O (\log{n})^{i - 1}}{\prod_{0 \leq j \leq i-2} \fract_j}
 = \frac{O (\log{n})^i}{\prod_{0 \leq j \leq i-1} \fract_j}
\end{align*}
as desired.
\end{proof}

To analyze the stretch of $ T $, we will use the following terminology:
we let the \emph{level} of an edge $ e $ of $ G $ be the largest $ i $ such that edge $ e $ is contracted to some edge~$ e' $ in $ G_i $.
Remember that $ E_i $ is a multiset of edges containing as many edges $ (u', v') $ as there are edges $ (u, v) \in E $ with $ u $ and $ v $ being contracted to different cluster centers $ u' $ and $ v' $ in $ G_i $, respectively.
Thus, the expected number of edges at level $ i $ is at most $ | E_i | $.
Note that for an edge $ e = (u, v) $ to be at level~$ i $, $ u $ and $ v $ must be contracted to the same cluster center in $ G_{i + 1} $.
Therefore, by \Cref{lem:path length for nodes in same cluster}, the stretch of edges at level~$ i $ in $ T $ with respect to $ G $ is at most $ \frac{O(\log{n})^{i+1}}{\prod_{0 \leq j \leq i} \fract_j} $.
The expected contribution to the total stretch of $ T $ by edges at level $ i \leq k - 1 $ is thus at most
\begin{equation}\label{eq:stretch of level i edges}
| E_i | \cdot \frac{O(\log{n})^{i+1}}{\prod_{0 \leq j \leq i} \fract_j} \leq \frac{m}{\beta_i} \cdot O (\log{n})^{i+1} \, .
\end{equation}


\subsection{Dynamic Low-Stretch Tree Algorithms}

To now obtain a fully dynamic algorithm for maintaining a low-stretch forest, it remains to plug in a concrete algorithm for maintaining $ T' $ together with suitable choices of the parameters.
We analyze two choices for dynamically maintaining $ T' $.
The first is the ``lazy'' approach of recomputing a low-stretch forest from scratch after each update to the input graph.
The second is a fully dynamic spanning forest algorithm with only trivial stretch guarantees.

\begin{theorem}[Restatement of Theorem~\ref{thm:fully dynamic low stretch tree}]
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanning forest of expected average stretch $ n^{o(1)} $ that has expected amortized update time $ m^{1/2 + o(1)} $.
These guarantees hold against an oblivious adversary.
\end{theorem}

\begin{proof}
%As stated in the theorem, we next give an algorithm with $ m^{1/2 + o(1)} $ update time. To bring the running time down to $ n^{1/2 + o(1)} $ (i.e., prove Corollary~\ref{cor:fully dynamic low stretch tree}), we can run this algorithm on a cut sparsifier of size $ \tilde O (n) $ that is maintained by a dynamic algorithm with polylogarithmic update time.
%We provide the details of this approach in Appendix~\ref{apx:sparsifier}.

We set $ k = \lceil \sqrt{\log{n}} \rceil $ and $ \fract_i = \fract = \tfrac{1}{m^{1 / (2k + 1)}} $ for all $ 0 \leq i \leq k-1 $ and maintain an LDD-hierarchy with these parameters.
Additionally, we maintain the graph $ G' $ induced by all non-isolated nodes of $ G_k $, which can easily be done by maintaining the degrees of nodes in $ G_k $.
After each update to $ G $, we compute a low-average stretch forest of $ T' $ of $ G' $.
Note that this recomputation is performed \emph{after} having updated all graphs in the hierarchy; we use the state-of-the-art static algorithm for computing a spanning forest of the multigraph $ G' $ with total stretch $ \tilde O (| E_k |) $ in time $ \tilde O (| E_k |) $.

By Equation~\eqref{eq:stretch of level i edges}, the contribution to the total stretch of $ T $ by edges at level $ i \leq k - 1 $ is at most $ m \cdot \tfrac{O (\log{n})^{i+1}}{\beta_i} $.
To bound the contribution of edges at level~$ k $, consider some edge $ e = (u, v) $ at level~$ k $ and let $ u' $ and $ v' $ denote the cluster centers to which $ u' $ and $ v' $ are contracted in $ G_k $, respectively.
Let $ \pi $ denote the path from $ u' $ to $ v' $ in $ T' $.
Using similar arguments as in the proof of Lemma~\ref{lem:path length for nodes in same cluster}, the contracted nodes and edges of $ \pi $ can be expanded to a path from $ u $ to~$ v $ in~$ T $ of length at most $ \tfrac{O (\log{n})^k}{\prod_{0 \leq i \leq k - 1} \fract_i} \cdot | \pi | $.
Thus, the contribution of edges at level~$ k $ is at most $ \tilde O (| E_k |) \cdot \tfrac{O (\log{n})^k}{\prod_{0 \leq i \leq k - 1} \fract_i} = \tilde O (m \cdot O (\log{n})^k) $ and the total stretch of~$ T $ with respect to~$ G $ is
\begin{align*}
\sum_{0 \leq i \leq k - 1} m \cdot \frac{O (\log{n})^{i+1}}{\beta} &  + \tilde O (m \cdot O (\log{n})^k) \\
 & = \tilde O \left( m \cdot \left( \frac{1}{\fract} \cdot \sum_{0 \leq i \leq k - 1} O (\log{n})^{i+1} + O (\log{n})^k \right) \right) \\
 &= \tilde O \left( m \cdot \frac{O (\log{n})^k}{\fract} \right) \\
 &= \tilde O \left( m m^{1 / (2k + 1)} \cdot O (\log{n})^k \right) \\
 &= m^{1 + o(1)} \, ,
\end{align*}
which gives an average stretch of $ m^{o(1)} = n^{o(1)} $.

By Observation~\ref{obs:number of nodes and edges}, $ G_k $ has at most $ m \beta^k $ edges in expectation and thus $ G' $ has at most $ m \beta^k $ nodes and edges in expectation.
Using the bound of Lemma~\ref{lem:update time hierarchy} for the update time of the LDD-hierarchy and the bound of $ \tilde O (m \beta^k ) $ for recomputing the low-stretch tree $ T' $ on $ G' $ from scratch, the expected amortized update time for maintaining $ T $ is
\begin{align*}
\tilde O \left( \sum_{0 \leq j \leq k-1} \frac{O (\log n)^{2 k}}{\fract_j \prod_{0 \leq j' \leq j} \fract_{j'}} + | E_k | \right) &= \tilde O \left( \sum_{0 \leq j \leq k-1} \frac{O (\log n)^{2 k}}{\fract^{j + 2}} + m \beta^k \right) \\
 &= \tilde O \left( \frac{O (\log n)^{2 k}}{\fract^{k + 1}} + m \beta^k \right) \\
 &= \tilde O (m^{(k + 1) / (2k + 1)} \cdot O (\log n)^{2 k}) \\
 &= \tilde O (m^{1/2 + 1 / (4k + 2)} \cdot O (\log n)^{2 k})  \\
 &= m^{1/2 + o(1)} \, . \qedhere
\end{align*}
\end{proof}


\begin{theorem}\label{thm:LST trade-off}
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanning forest of expected average stretch $ O (t + n^{1/3 + o(1)}) $ that has expected amortized update time $ \tfrac{n^{1 + o(1)}}{t} $ for every $ 1 \leq t \leq n $.
These guarantees hold against an oblivious adversary.
\end{theorem}

\begin{proof}
We set $ k = \lceil \log{\log{n}} \rceil $, $ \fract_0 = \sqrt{t/n} $ and $ \fract_i = \sqrt{\fract_{i-1}} $ for all $ 1 \leq i \leq k-1 $ and maintain an LDD-hierarchy with these parameters.
The spanning forest $ T' $ is obtained by fully dynamically maintaining a spanning forest of $ G_k $ using any algorithm with polylogarithmic update time. %~\cite{HenzingerK99,HolmLT01}.

By Equation~\eqref{eq:stretch of level i edges}, the contribution to the total stretch of $ T $ by edges at level $ i \leq k - 1 $ is at most $ \frac{m}{\beta_i} \cdot O (\log{n})^{i+1} $.
For every edge $ e = (u, v) $ at level~$ k $ with $ u $ contracted to $ u' $ and $ v $ contracted to $ v' $ in $ G_k $, there is a path from $ u' $ to $ v' $ in $ T' $ that by undoing the contractions can be expanded to a path from $ u $ to $ v $ in $ T $, which trivially has length at most $ n - 1 $.
Thus, the contribution by each edge at level $ k $ is at most $ n - 1 $.
As for every $ 0 \leq i \leq k $ there are at most $ | E_i | = m \cdot \prod_{0 \leq j \leq i - 1} \beta_j $ edges at level $ i $ in expectation, we can bound the expected total stretch of $ T $ with respect to $ G $ as follows:
\begin{align*}
\sum_{0 \leq i \leq k-1}  | E_i | \cdot \frac{O(\log{n})^{i+1}}{\prod_{0 \leq j \leq i} \fract_j} & + | E_k | \cdot n  \\ & =
\sum_{0 \leq i \leq k-1} \frac{m \cdot O (\log{n})^{i+1}}{\fract_i} + m \cdot \prod_{0 \leq i \leq k-1} \fract_i \cdot n \\
 &= m \cdot \left( \sum_{0 \leq i \leq k-1} \frac{O (\log{n})^{i+1}}{\fract_i} + \prod_{0 \leq i \leq k-1} \fract_i \cdot n \right)
\end{align*}
This gives an average stretch of $ \sum_{0 \leq i \leq k-1} \tfrac{O (\log{n})^{i+1}}{\fract_i} + \prod_{0 \leq i \leq k-1} \fract_i \cdot n $.
We now simplify these two terms.
Exploiting that $ \fract_i \geq \fract_0 $ for all $ 1 \leq i \leq k-1 $, we get
\begin{align*}
\sum_{0 \leq i \leq k-1} \frac{O (\log{n})^{i+1}}{\fract_i} & \leq \sum_{0 \leq i \leq k-1} \frac{O (\log{n})^{i+1}}{\fract_0} = \frac{O (\log{n})^k}{\fract_0} \\ & = \frac{O (\log n)^k}{\sqrt{t/n}} = \sqrt{\frac{n^{1+o(1)}}{t}} \, .
\end{align*}
Furthermore, the geometric progression of the $ \fract_i $'s gives
\begin{align*}
\prod_{0 \leq i \leq k-1} \fract_i \cdot n & = \prod_{0 \leq i \leq k-1} \fract_0^{1/2^i} \cdot n = \fract_0^{\sum_{0 \leq i \leq k-1} 1/2^i} \cdot n = \fract_0^{2 - 1/2^{k-1}} \cdot n \\ 
& = \frac{t^{1 - 1/2^k}}{n^{1 - 1/2^k}} \cdot n \leq t \cdot n^{1/2^k} = O (t) \, .
\end{align*}
The average stretch of the forest maintained by our algorithm is thus at most $ O ( t + \sqrt{\tfrac{n^{1+o(1)}}{t}} ) $, which, after balancing the two terms, can be rewritten as $ O (t + n^{1/3 + o(1)}) $.

It remains to bound the update time of the algorithm.
By Lemma~\ref{lem:update time hierarchy}, the hierarchy can be maintained with an amortized update time of
\begin{align*}
\tilde O \left( \sum_{0 \leq j \leq k-1} \frac{O (\log n)^{2 k}}{\fract_j \cdot \prod_{0 \leq j' \leq j} \fract_{j'}} \right) & = \tilde O \left( \sum_{0 \leq j \leq k-1} \frac{O (\log n)^{2 k}}{\fract_0^{1 / 2^j} \cdot \fract_0^{2 - 1 / 2^j}} \right) \\
&  = \tilde O \left( \sum_{0 \leq j \leq k-1} \frac{O (\log n)^{2 k}}{\fract_0^2} \right)  \\ 
& = \frac{n \cdot O (\log n)^{2 k}}{t} = \frac{n^{1 + o(1)}}{t} \, .
\end{align*}
Since the amortized number of changes to $ G_k $ per update to $ G $ is trivially bounded by $ \tfrac{n^{1 + o(1)}}{t} $ as well and since $ T' $ can be maintained with polylogarithmic amortized time per update to $ G_k $, we can maintain $ T $ with amortized update time $ \tfrac{n^{1 + o(1)}}{t} $.
\end{proof}

Note that the algorithm of Theorem~\ref{thm:fully dynamic low stretch tree} is superior to the algorithm of Theorem~\ref{thm:LST trade-off} as long as $ t \leq \sqrt{n} $.
If $ t \geq \sqrt{n} $, then the algorithm of Theorem~\ref{thm:LST trade-off} provides stretch $ O (t) $ and update time $ \tfrac{n^{1 + o(1)}}{t} $.

\subsection{Input Graph Sparsification}\label{apx:sparsifier}

In the following, we explain how input graph sparsification can be performed to the algorithm of Theorem~\ref{thm:fully dynamic low stretch tree} by running the algorithm on a cut sparsifier, similar to the approach of Koutis et al.~\cite{KoutisLP16} in the \emph{static} setting.

\begin{corollary} [Restatement of Corollary~\ref{cor:fully dynamic low stretch tree}] \label{corApp:fully dynamic low stretch tree}
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanning forest of expected average stretch $ n^{o(1)} $ that has expected amortized update time $ n^{1/2 + o(1)} $.
These guarantees hold against an oblivious adversary.
\end{corollary}

To make the analysis rigorous, we introduce some additional notation for multigraphs.


\paragraph{Succinct Representation of Multigraphs.}
A multigraph $ G = (V, E) $ consists of a set of nodes~$ V $ and a multiset of edges~$ E $.
We denote by $ \bar{E} = \{ (u, v) \in \binom{V}{2} \mid (u, v) \in E \} $ the support of the multiset~$ E $.
This allows a multigraph $ G = (V, E) $ to be succinctly represented as its \emph{skeleton} $ \bar{G} = (V, \bar{E}, \mu_G) $ where $ \mu_G $ is a multiplicity function $ \mu_G : \bar{E} \rightarrow \mathbb{Z}^+ $ that assigns to each edge $ e $ its (positive integer) multiplicity $ \mu_G (e) $.
We denote by $ m \coloneqq | E | $ the number of multi-edges (considering multiplicities), and by $ \bar{m} \coloneqq | \bar{E} | $ the size of the support of $ E $ (disregarding multiplicities).
For simplicity, we assume that $ m $ is polynomial in~$ n $.
The total stretch of a spanning forest~$ T $ is defined with respect to~$ E $, i.e.,
\begin{equation}
\str_T (G) = \sum_{e = (u, v) \in E(G)} \dist_T (u, v) = \sum_{e = (u, v) \in \bar{E}(G)} \mu_G (e) \cdot \dist_T (u, v) \, . \label{eq:definition of total stretch}
\end{equation}

Our dynamic algorithm will exploit that, given the skeleton of a multigraph, a low-stretch forest of can be computed without (significant) dependence on the multiplicities.
\begin{lemma}\label{lem:multiplicity oblivious running time}
Given the skeleton $ \bar{G} $ of a multigraph $ G $, a spanning forest of $ G $ of total stretch $ m^{1 + o(1)} $ can be computed in time $ \tilde O (\bar{m}) $.
\end{lemma}
Such a guarantee can be achieved with a \emph{static} version of our algorithm, i.e., by combining the scheme of Alon et al.~\cite{AlonKPW95} with the LDD of Miller et al.~\cite{MillerPX13}.
Although we are not aware of any statement of such a ``multiplicity-oblivious'' running time in the literature, it seems plausible that the state-of-the art algorithms (achieving a total stretch of $ \tilde O (m) $) also have this property.
Note however that a stretch of $ m^{1 + o(1)} $ is anyway good enough for our purpose.


\paragraph{Refined Analysis of Dynamic Low-Stretch Tree Algorithm.}

We now restate the guarantees of our fully dynamic low-stretch forest algorithm when the input is a multigraph undergoing insertions and deletions of multi-edges (i.e., each update increases or decreases the multiplicity of some edge by~$ 1 $).
Our fully dynamic LDD algorithm maintains a clustering such that every edge is an inter-cluster edge with probability $ \beta $.
This implies that at most a $ \beta $-fraction of the edges are inter-cluster edges in expectation -- regardless of whether we consider multiplicities.
More precisely, contracting the clusters to single nodes yields a multigraph $ G' = (V', E') $ with $ | E' | \leq \beta | E | $ and $ | \bar{E}' | \leq \beta | \bar{E} | $.
Now, in particular the LDD hierarchy in the proof of Theorem~\ref{thm:fully dynamic low stretch tree} results in a multigraph $ G' = (V', E') $ with $ | E' | \leq \beta^k m $ and $ | \bar{E}' | \leq \beta^k \bar{m} $ (after $k$ levels).
For such a graph, if its skeleton is given explicitly, one can compute a spanning forest of total stretch $ O (|E'|^{1 + o(1)}) $ in time $ \tilde O (|\bar{E}'|) $ by Lemma~\ref{lem:multiplicity oblivious running time}.
Note that our dynamic algorithm can explicitly maintain the skeleton of $ G' $ with neglegible overheads in the update time.
It follows that our algorithm maintains a spanning forest of total stretch $ O (m^{1 + o(1)}) $ and has an update time of $ \tilde O (\bar{m}^{1/2 + o(1)}) $.


\paragraph{Cut Sparsifiers.}
For the definition of cut sparsifiers, we consider cuts of the form $ (U, V \setminus U) $ induced by a subset of nodes $ U \subset V $.
The capacity of such a cut $ (U, V \setminus U) $ in a graph $ G $ is defined as the total multiplicity of edges crossing the cut, i.e.,
\begin{equation*}
\capacity_G (U, V \setminus U) = \sum_{\substack{e = (u, v) \in \bar{E} \\ u \in U, v \in V \setminus U}} \mu_G (e)
\end{equation*}
A $ (1 \pm \epsilon) $-\emph{cut sparsifier}~\cite{BenczurK15} (with $ 0 \leq \epsilon \leq 1/2 $) of a multigraph $ G = (V, E) $ is a ``subgraph'' $ H = (V, F) $ with $ \bar{F} \subseteq \bar{E} $ such that for every $ U \subset V $ we have
\begin{equation*}
(1 - \epsilon) \capacity_G (U, V \setminus U) \leq \capacity_H (U, V \setminus U) \leq (1 + \epsilon) \capacity_G (U, V \setminus U) \, ,
\end{equation*}
i.e., $ H $ approximately preserves all cuts of $ G $.
Now let $ H $ be a $ (1 \pm \epsilon) $-\emph{cut sparsifier} of a multigraph $ G = (V, E) $ and let $ T = (V, E(T))$ be a (simple) spanning forest of $ H $.
For every edge $ e $ of the forest~$ T $, the nodes are naturally partitioned into two connected subsets upon removal of~$ e $.
Let these two subsets be denoted by $ V_e $ and $ V \setminus V_e $.
Emek~\cite{Emek11} and Koutis et al.~\cite{KoutisLP16}, observed that by rearranging the sum in~\eqref{eq:definition of total stretch}, one obtains the following cut-based characterization of the stretch:
\begin{equation*}
\str_T (G) = \sum_{e \in E(T)} \capacity_G (V_e, V \setminus V_e) \, .
\end{equation*}
Observe that the cut $ (V_e, V \setminus V_e) $ is approximately preserved in $ H $ and thus $ \capacity_G (V_e, V \setminus V_e) \leq \tfrac{1}{1 - \epsilon} \capacity_H (V_e, V \setminus V_e) \leq (1 + 2 \epsilon) \capacity_H (V_e, V \setminus V_e) $.
The stretch of $ G $ with respect to~$ T $ can now be bounded by
\begin{align*}
\str_T (G) &= \sum_{e \in E(T)} \capacity_G (V_e, V \setminus V_e) \\
&\leq (1 + 2 \epsilon) \sum_{e \in E(T)} \capacity_H (V_e, V \setminus V_e) \\
&= (1 + 2 \epsilon) \str_T (H) \, .
\end{align*}
Thus, computing the low-stretch forest on the sparsifier $ H $ instead of the original graph $ G $ only increases the total stretch by a constant factor if the number of multi-edges in $ H $ is proportional to the number of edges in $ G $.


\paragraph{Dynamic Cut Sparsifiers.}
The fully dynamic algorithm of Abraham et al.~\cite{AbrahamDKKP16} maintains, with high probability, a $ (1 \pm \epsilon) $-cut sparsifier~$ H = (V, F) $ of a simple graph~$ G = (V, E) $ such that $ | \bar{F} | = \tilde O (n / \epsilon^2) $ with update time $ \poly (\log n, \epsilon) $.
For each node $ v $, the degree in $ H $ exceeds the degree in $ G $ by at most a factor of $ (1 \pm \epsilon) $ because the cut $ (\{ v \}, V \setminus \{ v \}) $ is approximately preserved in $ H $.
We can thus bound the number of multi-edges in $ H $ (i.e., the sum of all edge multiplicities) by $ | F | = O ((1 + \epsilon) |E|) $.
The algorithm maintains a hierarchy of the edges with $ O (\log n) $ layers, where edges at level~$ i $ have multiplicity $ 4^i $ and each edge is at level~$ i $ with probability at most $ 1/4^i $.
After an update to the input graph, the dynamic algorithm adds or removes at most $ \poly(\log n, \epsilon) $ edges in each level.
%Using rough estimates, we can therefore additionally bound the expected number of multi-edges in $ H $ (i.e., the sum of all edge multiplicities) by $ | F | = \tilde O (|E|) $.
Thus, we can bound the amount of change to $ H $ per update to $ G $ as follows: for every update to $ G $, the expected sum of the changes to the edge multiplicities of~$ H $ is at most $ \poly(\log n, \epsilon) $.


\paragraph{Putting Everything Together~(Proof of Corollary~\ref{corApp:fully dynamic low stretch tree}).}
We now first use the fully dynamic algorithm of Abraham et al. to maintain a cut sparsifier $ H = (V, F) $ of the input graph $ G = (V, E) $ (with $ \epsilon = 1/2 $) and second run our fully dynamic low-stretch tree algorithm on top of $ H $.
Here, $ G $ is a simple graph with $ m = | E | $ edges and $ H $ is a multigraph with $ |F| = O (m) $ and $ |\bar{F}| = \tilde O (n) $.
The spanning forest $ T $ maintained in this way gives expected total stretch at most $ |F|^{1 + o(1)} $ with respect to $ H $.
As argued above, this implies an expected total stretch of at most $ O ((1 + 2 \epsilon) |F|^{1 + o(1)}) = O (m^{1 + o(1)}) $ with respect to $ G $, i.e., an average stretch of $ m^{o(1)} = n^{o(1)} $.
Each update to the input graph results in $ \polylog{n} $ changes to the sparsifier in expectation, which are then processed as ``induced'' updates by our dynamic low-stretch tree algorithm.
Thus, we overall arrive at an expected amortized update time of $ \tilde O (|\bar{F}|^{1/2 + o(1)}) = O (n^{1/2 + o(1)}) $.


==> chapters/lowstretchtree/overview.tex <==
\section{Technical Overview}\label{sec:overview}

In the following, we provide some intuition for our approach and highlight the main ideas of this chapter.

\paragraph*{Low Average Stretch Tree.}
%Before we give an overview of our new approach, we review the straightforward algorithm for an update time of $ \tilde O (n) $.
%The idea is to maintain a cut sparsifier~\cite{BenczurK15} of the underlying graph and to do a recomputation from scratch on the cut sparsifier after each update.
%The state-of-the-art static algorithm of Abraham and Neiman~\cite{AbrahamN12} computes a spanning tree of average stretch $ O (\log{n} \log{\log{n}}) $ in time $ \tilde O (m) $ on an input graph with $ m $ edges.
%The fully dynamic algorithm of Abraham et al.~\cite{AbrahamDKKP16} maintains a $ (1 \pm \epsilon) $-cut sparsifier with $ \tilde O (n / \epsilon^2) $ edges in polylogarithmic update time with high probability.
%An argument of Koutis, Levin, and Peng~\cite{KoutisLP16} shows that a spanning tree of total stretch~$ t $ with respect to a $ (1 \pm \epsilon) $-cut sparsifier of $ G $ has stretch $ (1 \pm 2 \epsilon) t $ with respect to~$ G $.
%Thus, by combining these two algorithms (and setting $ \epsilon = 1/2 $) we can maintain a spanning tree of average stretch $ O (\log^2 n \log \log n) $ with update time $ \tilde O (n) $ with high probability.
A first idea is to employ the dynamic low-diameter decomposition of Theorem~\ref{thm:fully dynamic LDD}.
This algorithm can maintain a \sloppy $ (\fract, O(\tfrac{\log{n}}{\fract})) $-decomposition, i.e., a partitioning of the graph into clusters such that there are at most $ \fract m $ inter-cluster edges and the (strong) diameter of each cluster is at most $ O (\tfrac{\log{n}}{\fract}) $.
In particular, each cluster has a designated center and the algorithm maintains a spanning tree of each cluster in which every node is at distance at most $ O (\tfrac{\log{n}}{\fract}) $ from the center.
Now consider the following simple dynamic algorithm:
\begin{enumerate}
\item Maintain a $ (\fract, O(\tfrac{\log{n}}{\fract})) $-decomposition of the input graph~$ G $.
\item Contract the clusters in the decomposition to single nodes and maintain a multigraph $ G' $ containing one node for each cluster and all inter-cluster edges.
\item Compute a low-stretch tree $ T' $ of $ G' $ after each update to~$ G $ using a static algorithm providing polylogarithmic average stretch.
\item Maintain $ T $ as the ``expansion'' of $ T' $ in which every node in $ T' $ is replaced by the spanning tree of diameter $ O (\tfrac{\log{n}}{\fract}) $ of the cluster representing the node.
\end{enumerate}
As the clusters are non-overlapping it is immediate that $ T $ is indeed a tree.
To analyze the average stretch of~$ T $, we distinguish between inter-cluster edges (with endpoints in different clusters) and intra-cluster edges (with endpoints in the same cluster).
Each intra-cluster edge has stretch at most $ O (\tfrac{\log{n}}{\fract}) $ as the spanning tree of the cluster containing both endpoints of such an edge is a subtree of $ T $.
Each inter-cluster edge has polylogarithmic average stretch in $ T' $ with respect to $ G' $.
By expanding the clusters, the length of each path in $ T' $ increases by a factor of at most $ O (\tfrac{\log{n}}{\fract}) $.
Thus, inter-cluster edges have an average stretch of $ O (\tfrac{\log{n}}{\fract} \polylog{n}) $ in $ T $.
As there are at most $ m $ intra-cluster edges and at most $ \fract m $ inter-cluster edges, the total stretch over all edges is at most $ O (m \cdot \tfrac{\log{n}}{\fract} + \fract m \cdot \tfrac{\log{n}}{\fract} \polylog{n}) = \tilde O (m \cdot \tfrac{1}{\fract}) $, which gives an average stretch of $ \tilde O (\tfrac{1}{\fract}) $.

To bound the update time, first observe that the number of inter-cluster edges is at most $ \fract m $.
Thus, $ G' $ has at most $ \fract m $ edges and therefore the static algorithm for computing $ T' $ takes time $ \tilde O (\fract m) $ per update.
Together with the update time of the dynamic LDD, we obtain an update time of $ \tilde O (\tfrac{1}{\fract^2} + \fract m) $.
By setting $ \fract = m^{1/3} $, we would already obtain an algorithm for maintaining a tree of average stretch $ \tilde O (m^{1/3}) $ with update time $ \tilde O (m^{2/3}) $.

We can improve the stretch and still keep the update time sublinear by a hierarchical approach in which the scheme of clustering and contracting is repeated $ k $ times.
Observe that the $i$-th contracted graph will contain at most $ \fract^i m $ many edges and, in the final tree $ T $, the stretch of each edge disappearing with the $(i + 1)$-th contraction is $ O (\tfrac{\log{n}}{\fract})^{i + 1} $, which can be obtained by expanding the contracted low-diameter clusters. 
After $ k $~contractions, there are at most $ \fract^k m $ edges remaining and they have polylogarithmic average stretch in~$ T' $ with respect to~$ G' $, which, again by expanding clusters, implies an average stretch of at most $ O (\tfrac{\log{n}}{\fract})^k \cdot \polylog{n} $ in~$ T $ with respect to~$ G $.
This leads to a total stretch of $ O (\sum_{0 \leq i \leq k - 1} \fract^i m \cdot O(\tfrac{\log{n}}{\fract})^{i + 1} + \fract^k m \cdot O (\tfrac{\log{n}}{\fract})^k \polylog{n}) = \tilde O (m \cdot \tfrac{O (\log n)^k}{\fract}) $, which gives an average stretch of $ \tilde O (\tfrac{O (\log n)^k}{\fract}) $.
To bound the update time, observe that updates propagate within the hierarchy as each change to inter-cluster edges of one layer will appear as an update in the next layer.
Each operation in the dynamic LDD algorithm will perform at most one change to the clustering, i.e., the number of changes propagated to the next layer of the hierarchy is at most $ \tilde O(\tfrac{1}{\fract^2}) $ per update to the current layer.
This will result in an update time of $ \tilde O ((\tfrac{\polylog{n}}{\fract})^{2(i - 1)} \cdot \frac{1}{\fract^2}) $ in the $i$-th contracted graph per update to the input graph.
The update time for maintaining the tree~$ T $ will then be $ \tilde O (\tfrac{1}{\fract^{2 k}} + \fract^k m) $, which is $ m^{2/3} $ at best, i.e., no better than the simpler approach above.
A tighter analysis can improve this update time significantly:
The second part of Theorem~\ref{thm:fully dynamic LDD} bounds the amortized number of edges to become inter-cluster edges by $ \tilde O (\tfrac{1}{\fract}) $.
This results in an update time of $ \tilde O ((\tfrac{\polylog{n}}{\fract})^{k + 1} + \fract^k m) $.
By setting $ k = \sqrt{\log{n}} $ and $ \fract = \tfrac{1}{m^{1 / (2k + 1)}} $ we can roughly balance these two terms in the update time and thus arrive at an update time of $ m^{1/2 + o(1)} $ while the average stretch is $ n^{o(1)} $.
The crux of our approach is thus an ``early stopping'' of the Alon et al.\ LDD hierarchy such that it does not ``exhaust'' the graph.
We crucially exploit that, for an unweighted input graph, the size of the contracted graph decreases geometrically, which allows us to partially compensate for the blow-up of propagated updates in the hierarchy.

We can use the following sparsification approach to further reduce the update time to $ n^{1/2 + o(1)} $:
The main idea is to maintain a cut sparsifier with $ \tilde O (n) $ edges and then run the algorithm on the cut sparsifier instead of the input graph to reduce the update time from $ m^{1/2 + o(1)} $ to $ n^{1/2 + o(1)} $.
The dynamic algorithm of Abraham et al.~\cite{AbrahamDKKP16} can maintain such a cut sparsifier with polylogarithmic update time.
Using a different cut sparsifier construction, Koutis, Levin, and Peng~\cite{KoutisLP16} showed in the static setting that a low-stretch tree of their cut sparsifier is also a low-stretch tree of the input graph (where the average stretch only increases multiplicatively by the approximation guarantee of the cut sparsifier).
However, we cannot use exactly the same approach because the cut sparsifier of Abraham et al.\ has edge weights, even though the input graph is unweighted.
We show that the main argument in~\cite{KoutisLP16} still goes through if we interpret the edge weights of the sparsifier as edge multiplicities in an unweighted graph.
We then show that the algorithm of Theorem~\ref{thm:fully dynamic low stretch tree} can also handle such graphs for updates that increment or decrement the multiplicity of some edge by $ 1 $.
A fine-grained analysis of the total multiplicity of edges of the sparsifier and its expected amount of change per update to the input graph then gives the desired result.

In Section~\ref{sec:low_stretch_tree}, where we present the details of our approach, we consider two slight generalizations:
First, we implicitly handle the case that the input graph could become disconnected by maintaining a low-stretch \emph{forest}.
Second, we give a parameterized analysis that also allows for a trade-off between stretch and update time.


\paragraph*{Low Diameter Decomposition.}

To obtain a suitable algorithm for dynamically maintaining a low-diameter decomposition, we follow the widespread paradigm of first designing a decremental -- i.e., deletions-only -- algorithm and then extending it to a fully dynamic one.
We can show that, for any sequence of at most $ m $ edge deletions (where $ m $ is the initial number of edges in the graph), a $ (\fract, O(\tfrac{\log{n}}{\fract})) $-decomposition can be maintained with expected total update time $ \tilde O (m / \fract) $.
Here, we build upon the work of Miller et al.~\cite{MillerPX13} who showed that \emph{exponential random-shift clustering} produces clusters of radius $ O (\log{n} / \fract) $ such that each edge has a probability of at most $ \fract $ to go between clusters.
This clustering is obtained by first having each node sample a random \emph{shift value} from the exponential distribution and then determining the cluster center of each node as the node to which it minimizes the difference between distance and (other node's) shift value.

In the parallel algorithm of~\cite{MillerPX13}, the clustering is obtained by essentially computing one single-source shortest path tree of maximum depth $ O (\log{n} / \fract) $.
To make this computation efficient\footnote{For their parallel algorithm, efficiency in particular means low depth of the computation tree.}, the shift values are rounded to integer values and the fractional values are only considered for tie-breaking.
We observe that one can maintain this bounded-depth shortest path tree with a simple modification of the well-known Even-Shiloach algorithm that spends time $ O ( \degree (v)) $ every time a node $ v $ increases its level (distance from the source) in the tree.
By rounding to integer edge weights, similar to~\cite{MillerPX13}, we can make sure that the number of level increases to consider is at most $ O (\log{n} / \fract) $ for each node.
Note however that this standard argument charging each node only when it increases its level is not enough for our purpose: the assignment of nodes to clusters follows the fractional values for tie-breaking, which might result in some node $ v $ changing its cluster -- and in this way also spend time $ O (\degree (v)) $ -- without increasing its level~(note that here the difficulty is not on maintaining the cluster that $v$ belongs to, but rather on bounding the number of cluster changes for $v$).
As has been observed in~\cite{MillerPX13}, the fractional values of the shift values effectively induce a random permutation on the nodes.
Using a similar argument as in the analysis of the dynamic spanner algorithm of Baswana et al.~\cite{BaswanaKS12}, we can thus show that in expectation each node changes its cluster at most $ O (\log{n}) $ times while staying at a particular level.
This results in a total update time of $ \tilde O (m / \fract) $.
Trivially, this also bounds the total number of times that edges become inter-cluster edges during the whole decremental algorithm by $ \tilde O (m / \fract) $.
Using a more sophisticated analysis we can obtain the stronger bound of $ \tilde O (m) $ on the latter quantity:
Intuitively, each endpoint of an edge changes its cluster at most $ \tilde O (\tfrac{1}{\fract}) $ times and after each cluster change the edge is an inter-cluster edge with probability at most $ \beta $, yielding a total of $ \tilde O ( m \cdot \tfrac{1}{\fract} \cdot \beta ) $ times that edges become inter-cluster edges.
The rigorous argument is however more complicated because we cannot guarantee that the event of being an inter-cluster edge might not be independent of the event of the endpoint changing its cluster.

To obtain a fully dynamic algorithm, we observe that any LDD can tolerate a certain number of insertions to the graph.
A $ (\fract, O(\tfrac{\log{n}}{\fract})) $-decomposition allows at most $ \fract m $ inter-cluster edges and thus, if we insert $ O (\fract m) $ edges to the graph without changing the decomposition, we still have an $ (O(\fract), O(\tfrac{\log{n}}{\fract})) $-decomposition.
We can exploit this observation by simply running a decremental algorithm, that is restarted from scratch after each phase of $ \Theta (\fract m) $ updates to the graph.
We then deal with edge deletions by delegating them to the decremental algorithm and we deal with edge insertions in a lazy way by doing nothing.
This results in a total time of $ \tilde O (m / \fract) $ that is amortized over $ \Theta (\fract m) $ updates to the graph, i.e., amortized update time $ \tilde O (1/\beta^2) $.
Similarly, the amortized number of edges to become inter-cluster edges after an update is $ \tilde O (1/\beta) $.

In our detailed description and analysis in Section~\ref{sec:LDD}, we first review the construction of Miller et al., and then present our decremental and fully dynamic algorithms.


==> chapters/lowstretchtree/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

\paragraph*{Graphs.}

Let $G=(V,E,\ww_G)$ be an undirected weighted graph, where $n = |V|$, $m = |E|$ and $\ww_G: E \rightarrow \mathbb{R}_+$. If $\ww_G(e) = 1$ for all $e \in E$, then we say $G$ is an undirected unweighted graph.
If $ E $ is a multiset, i.e., every element of $E$ may have integer multiplicity greater than $ 1 $, then we call $ G $ a multigraph.
For a subset $C \subseteq V$ let $G[C]$ denote the subgraph of $G$ induced by  $C$. Throughout the chapter we call $C \subset V$ a \emph{cluster}. For any positive integer $k$, a \emph{clustering} of $G$ is a partition of $V$ into disjoint subsets $C_1, C_2, \ldots, C_k$. We say that an edge is an \emph{intra-cluster} edges if both its endpoints belong to the same cluster $C_i$ for some $i$; otherwise, we say that an edge is an \emph{inter-cluster} edge.

For any $u,v \in V$ let $\dist_G(u,v)$ denote the length of a shortest path between $u$ and $v$ induced by the edge weights $\ww_G$ of the graph $G$. When $G$ is clear from the context, we will omit the subscript. The \emph{strong diameter} of a cluster $C \subset V$ is the maximum length of the shortest path between two nodes in $G[C]$, i.e., $\max \set{\dist_{G[C]}(u,v)}{u,v \in C}$. In the following we define a low-diameter clustering of $G$. 

\begin{definition} Let $k$ be any positive integer, $\beta \in (0,1)$ and $\diam > 0$. Given an undirected, unweighted graph $G=(V,E)$, a $(\fract,\diam)$-decomposition of $G$ is a partition of $V$ into disjoint subsets $C_1, C_2, \ldots,C_k$ such that:
\begin{enumerate}
\item The strong diameter of each $C_i$ is at most $\diam$.
\item The number of edges with endpoints belonging to different subsets is at most $\fract m$.
\end{enumerate}
\end{definition}
In the $(\fract,\diam)$-decompositions of the randomized dynamic algorithms in this chapter, the bound in Condition~2 is in expectation.

Let $H = (V, F) $ be a subgraph of $G = (V, E, \ww_G)$. For any pair of nodes $u,v \in V$, we let $\dist_H(u,v)$ denote the length of a shortest path between $u$ and $v$ in $H$. We define the \emph{stretch} of an edge $(u,v) \in E$ with respect to $H$ to be 
\begin{equation*}
	\str_H(u,v) \coloneqq  \frac{\dist_H(u,v)}{\ww_G(u,v)} \, .
\end{equation*}
%and the total stretch of $ G $ with respect to $ H $ to be
%\begin{equation*}
%	\str_H (G) \coloneqq  \sum_{(u,v) \in E} \str_T(u,v) \, .
%\end{equation*}
The stretch of $ H $ is defined as the maximum stretch of any of edge $(u,v) \in E$.
The \emph{average stretch} over all edges of $G$ with respect to $H$ is given by
\[
	\avestr_H(G) \coloneqq \frac{1}{|E|} \sum_{(u,v) \in E} \str_H(u,v).
\]

\begin{comment}
To leverage the full power of our algorithms, we will employ cut sparsifiers, which approximately preserve all cuts of a graph.
In the following, we consider cuts of the form $ (U, V \setminus U) $ induced by a subset of nodes $ U \subset V $.
The \emph{capacity} of such a cut $ (U, V \setminus U) $ in a graph $ G $ is defined as the total weight of edges crossing the cut., i.e.,
\begin{equation*}
\capacity_G (U, V \setminus U) = \sum_{\substack{e = (u, v) \in E \\ u \in U, v \in V \setminus U}} w_G (e) \, .
\end{equation*}
If $ G $ is an unweighted multigraph, the capacity of a cut $ (U, V \setminus U) $ is simply the total multiplicity of edges crossing the cut.
\begin{definition}[\cite{BenczurK15}]
A $ (1 \pm \epsilon) $-\emph{cut sparsifier} of a multigraph $ G = (V, E) $ is a subgraph $ H = (V, F) $ with $ F \subseteq E $ such that for every $ U \subset V $ we have % TODO allow different edge weights
\begin{equation*}
(1 - \epsilon) \capacity_G (U, V \setminus U) \leq \capacity_H (U, V \setminus U) \leq (1 + \epsilon) \capacity_G (U, V \setminus U) \, ,
\end{equation*}
\end{definition}

\begin{lemma}[Implicit in~\cite{KoutisLP16}]\label{lem:low stretch tree on cut sparsifier}
Let $ H $ be a $ (1 + \epsilon) $-cut sparsifier of a multigraph $ G $ (with $ 0 < \epsilon \leq \tfrac{1}{2} $) and let $ T $ be a spanning forest of $ H $.
Then $ T $ is a spanning forest of $ G $ of total stretch $ \str_T (G) \leq (1 + 2 \epsilon) \str_T (H) $.
\end{lemma}

\begin{proof}
Observe first that approximate cut preservation implies that each connected component of $ G $ is also a connected component of $ H $.
Thus, any spanning forest of $ H $ is also a spanning forest of $ G $.

For every edge $ e $ in a tree of the forest~$ T $, the nodes are naturally partitioned into two connected subsets upon removal of~$ e $.
Let these two subsets be denoted by $ V_e $ and $ V \setminus V_e $.
Emek~\cite{Emek11} and Koutis et al.~\cite{KoutisLP16}, observed that by rearranging the sum in~\eqref{eq:definition of total stretch}, one obtains the following cut-based characterization of the stretch:
\begin{equation*}
\str_T (G) = \sum_{e \in E(T)} \capacity_G (V_e, V \setminus V_e) \, .
\end{equation*}
Observe that the cut $ (V_e, V \setminus V_e) $ is approximately preserved in $ H $ and thus $ \capacity_G (V_e, V \setminus V_e) \leq \tfrac{1}{1 - \epsilon} \capacity_H (V_e, V \setminus V_e) \leq (1 + 2 \epsilon) \capacity_H (V_e, V \setminus V_e) $.
The stretch of $ G $ with respect to~$ T $ can now be bounded by
\begin{align*}
\str_T (G) &= \sum_{e \in E(T)} \capacity_G (V_e, V \setminus V_e) \\
&\leq (1 + 2 \epsilon) \sum_{e \in E(T)} \capacity_H (V_e, V \setminus V_e) \\
&= (1 + 2 \epsilon) \str_T (H) \, .
\end{align*}
Thus, computing the low-stretch spanning forest on the sparsifier $ H $ instead of the original graph $ G $ only increases the total stretch by a constant factor if the number of multi-edges in $ H $ is proportional to the number of edges in $ G $.
\end{proof}
\end{comment}

\paragraph*{Exponential Distribution.}

For a parameter $\lambda$, the probability density function of the \emph{exponential distribution} $\expdis(\lambda)$ is given by
\[
	f(x,\lambda) \coloneqq  \begin{cases} 
   \lambda e^{-\lambda x} & \text{if } x \geq 0 \\
   0       & \text{otherwise}.
  \end{cases}
\]
The mean of the exponential distribution is $1/\lambda$.


\paragraph*{Dynamic Algorithms.}
Consider a graph with $ n $ nodes undergoing updates in the form of edge insertions and edge deletions.
An \emph{incremental} algorithm is a dynamic algorithm that can only handle insertions, a \emph{decremental} algorithm can only handle deletions, and a \emph{fully dynamic} algorithm can handle both.
We follow the convention that a fully dynamic algorithm starts from an empty graph with $ n $ nodes.
The (maximum) running time spent by a dynamic algorithm for processing each update (before the next update arrives) is called \emph{update time}.
We say that a dynamic algorithm has \emph{(expected) amortized} update time $ u (n) $ if its total running time spent for processing a sequence of $ q $ updates is bounded by $ q \cdot u (n) $ (in expectation).
In this chapter, we assume that the updates to the graph are performed by an \emph{oblivious adversary} who fixes the sequences of updates in advance, i.e., the adversary is not allowed to adapt its sequence of updates as the algorithm proceeds.
This is a standard assumption in dynamic graph algorithms\footnote{For example, all known randomized dynamic spanner algorithms~\cite{Elkin11,BaswanaKS12,BodwinK16,BernsteinFH19} work under this assumption.} and in particular, it implies that for randomized dynamic algorithms the sequence of updates is independent from the random choices of the algorithm.


==> chapters/lowstretchtree/spanner.tex <==
\section{Dynamic Spanner Algorithm}\label{sec:spanner}

\subsection{Static Spanner Construction}
In the following we review and adapt the static algorithm for constructing sparse low-stretch spanners due to Elkin and Neiman~\cite{ElkinN17}. Let $G=(V,E)$ be an unweighted, undirected graph on $n$ nodes, and let $k \geq 1$ be an integer. For every $u \in V$, we denote by $N(u)$ the set of all nodes incident to $u$. Recall that $\expdis(\beta)$ denotes the exponential distribution with parameter $\beta$. In what follows, we set $\beta = \log (cn)/k$, where $c>3$ denotes the success probability. A $2 k - 1$-\emph{spanner} of $G$ is a a subgraph $H=(V,E')$ such that for every $u,v \in V$, $\dist_H(u,v) \leq 2 k - 1 \cdot \dist_G(u,v)$. We refer to $2 k - 1$ and $|E'|$ as the \emph{stretch} and \emph{size} of $H$, respectively. 

We next review some useful notation. Let $\delta_u$ be the shift value of node $u \in V$. For each $x, u \in V$, recall that $m_u(x) = \dist_G(x,u) - \delta_u$ is the shifted distance of $x$ with respect to $u$, and let $p_u(x)$ denote the neighbor of $x$ that lies on a shortest path from $x$ to $u$. Also, for every node $x \in V$, let $m(x) = \min_{u \in V} \{ m_u(x) \}$ be the minimum shifted distance. Using our clustering notation from Section~\ref{sec:LDD}, it follows that $c(x) = \arg \min_{u \in V} \{ m_u(x) \}$, and thus $m(x) = m_{c(x)}(x)$.

We now present an algorithm that constructs spanners using exponential random-shift clustering. Specifically, we initially set $H=(V,\emptyset)$, and for each node $u \in V$, we independently pick a shift value $\delta_u$ from $\expdis(\beta)$. Then, for every $x \in V$, we add to the spanner $H$ the following set of edges
\begin{equation}
C(x) = \set{(x, p_u(x))}{m_u(x) \leq m(x) + 1} \, . \label{eqn: SpannerEqn}
\end{equation}

The following theorem give bounds on the stretch and the size of the spanner output by the above algorithm.

\begin{theorem}[\cite{ElkinN17}] For any unweighted, undirected simple graph $G=(V,E)$ on $n$ nodes, any integer $k \geq 1$, $c \geq 3$, there is a randomized algorithm that with probability at least $ 1 - \tfrac{2}{c} $ computes a spanner $H$ with stretch $2k-1$ and size at most $ (cn)^{1+1/k} $.
\end{theorem}

Our analysis will rely on the following useful properties of the above algorithm.

\begin{claim}[\cite{ElkinN17}]
The expected size of $ H $ is at most $ (c n)^{1/k} \cdot n $.
\end{claim}

\begin{claim}[\cite{ElkinN17}]\label{claim:bound on random shifts}
With probability at least $1-1/c$, it holds that $\delta_u < k$ for all $u \in V$.
\end{claim}

\begin{claim}[\cite{ElkinN17}]\label{claim:bound on depth of tree} Assume $\delta_u < k$ for all $u \in V$. Then for any $x \in V$, if $u$ is the node minimizing $m_u(x)$, i.e., $u = c(x)$, then $\dist_G(u,x) < k$.
\end{claim}

As argued by Elkin and Neiman, Claim~\ref{claim:bound on depth of tree} implies that the stretch of the spanner is at most $ 2k - 1 $.
Thus, the reason reason why the stretch guarantee is probabilistic is Claim~\ref{claim:bound on random shifts}.

\paragraph*{Implementation.} In the description of the spanner construction, it is not clear how to compute in nearly-linear time the set of edges $C(x)$ in Equation~(\ref{eqn: SpannerEqn}), for every node $x \in V$. To address this, we give an equivalent definition of $C(x)$, which better decouples the properties that the edges belonging to this set satisfy. Specifically, we define the set of edges
\begin{equation}
	C'(x) = \set{(x,y)}{y \in N(x) \text{ and } m_{c(y)}(x) \leq m(x) + 1} \, ,\label{eqn: equivalentSpannerEqn}
\end{equation}
and then show that $C(x) = C'(x)$. 

To this end, we will show that (a) $C(x) \subseteq C'(x)$ and (b) $C'(x) \subseteq C(x)$. Let $(x,y) \in C(x)$, where $y = p_u(x)$. By definition of $p_u(x)$, we have that $y \in N(x)$. We next show that $m_{c(y)}(x) \leq m(x) + 1$, which in turn proves (a). Indeed, 
\[
	m_{c(y)}(x) = m_{c(y)}(y) + 1 = m(y) + 1 \leq m_u(y) + 1 = m_u(x) \leq m(x)+1,
\]
where the last inequality follows from Equation~(\ref{eqn: SpannerEqn}). For showing the other containment, i.e., proving (b), let $(x,y) \in C'(x)$. Then we need to prove that there exists some $u \in V$ such that $y=p_u(x)$ and $m_u(x) \leq m(x) +1$. This follows by simply setting $u=c(y)$ and using Equation~(\ref{eqn: equivalentSpannerEqn}).

Now, similarly to the static low-diameter decomposition in Section~\ref{sec:staticLDD}, we augment the input graph~$G$ by adding a new source $s$ to $G$ and edges $(s,x)$ of weight $(\delta_{max} - \delta_x) \geq 0$, for every $x \in V$, where $\delta_{\max} = \max_{x \in V} \{\delta_x \}$. Recall that in the resulting graph $\hat{G}=(V \cup \{s\},\hat{E},\hat{\ww})$, for every $x \in V$, the node $u$ attaining the minimum $m(x)$ is exactly the root of the sub-tree below the source $s$ that contains $u$. Thus, we could use Dijkstra's algorithm to construct the shortest path tree of $\hat{G}$, and augment it appropriately to output the edge sets $C'(x)$, which in turn give us the spanner $H$.

However, in the dynamic setting, it is crucial for our algorithm to deal only with integral edge weights. To address this, we round down all the $\delta_u$ values to $\floor{\delta_u}$ and modify the weights of the edges incident to the source $s$ in $\hat{G}$. Let $G'=(V \cup \{s\}, E',\ww')$ be the resulting graph, and let $\floor{m_u(x)}$ denote the rounded shifted distances. Whenever two rounded distances are the same, we break ties using the permutation $ \pi $ on the nodes induced by the fractional values of the random shift values. Thus, the edge set $C'(x)$ is given by
\begin{equation*} 
	C'(x) = \set{(x,y)}{y \in N(x),~\floor{m_{c(y)(x)}} \leq \floor{m(x)} + 1 \text{ and } \pi(c(y)) < \pi(c(x))}.
\end{equation*}

Finally, we observe that the definition of the above set can be further simplified by using the facts that $m_{c(y)}(x) = m_{c(y)}(y) + 1$ and $\floor{m_{c(y)}(x)} \geq \floor{m(x)}$, that is
\begin{equation} \label{eqn: roundedSpannerEqn}
\begin{aligned}
   C'(x) & = \{(x,y) \mid y \in N(x),~\floor{m(y)} = \floor{m(x)} - 1 \text{ or } \\ 
   & [\floor{m(y)} = \floor{m(x)} \text{ and } \pi(c(y)) < \pi(c(x))] \} \, . 	
\end{aligned}
\end{equation}

Interpreting the above set in terms of the shortest-path tree output by Dijkstra's algorithm, we get that for any $x \in V$, we add the edge $(x,y)$ to the spanner $H$, if $y$ is a neighbor one level above the level or $x$, or if $x$ and $y$ are at the same level, and the cluster $y$ belongs to appears before in the permutation when compared to the cluster $x$ belongs to.
By Claim~\ref{claim:bound on depth of tree} the shortest-path tree has depth at most $ 2 k $ with high probability.

Now observe that the randomized properties of this spanner construction only depend on the integer parts of the random shift values and the permutation~$ \pi $ on the nodes induced by the order statistics of the fractional parts of the random shift values.
Similar to the argument of Miller et al.~\cite{MillerPX13} for low-diameter decompositions, it can be argued that due to memorylessness of the exponential distribution, one might as well use a uniformly sampled random permutation~$ \pi $ instead to obtain a spanner with the same probabilistic properties.


\subsection{Dynamic Spanner Algorithm}

Spanners have a useful property called \emph{decomposability}: Assume we are given a graph $ G = (V, E) $ with a partition into two subgraphs $ G_1 = (V, E_1) $ and $ G_2 = (V, E_2) $.
If $ H_1 = (V, F_1) $ is a spanner of $ G_1 $ and $ H_2 = (V, F_2) $ is a spanner of $ G_2 $, both of stretch $ t $, then $ H = (V, F_1 \cup F_2) $ is a spanner of $ G $.
This property allows for a reduction that turns decremental algorithms into fully dynamic ones at the expense of logarithmic overhead in size and update time, as it has been observed by Baswana et al.~\cite{BaswanaKS12}.
\begin{lemma}[Implicit in~\cite{BaswanaKS12}]\label{lem:spanner decremental to fully dynamic}
If there is a decremental algorithm for maintaining a spanner of stretch $ t $ and expected size $ s (n) $ with total update time $ m \cdot u (m, n) $, then there is a fully dynamic algorithm for maintaining a spanner of stretch $ t $ and expected size $ s (n) \cdot O (\log{n}) $ with amortized update time $ u (m, n) \cdot O (\log{n}) $.
\end{lemma}

In the remainder of this section, we explain how the techniques we developed in Section~\ref{sec:LDD} allow for a decremental implementation of the spanner construction explained above.
\begin{theorem}
Given any unweighted, undirected graph undergoing edge deletions, there is a decremental algorithm for maintaining a spanner of stretch $ 2k - 1 $ and expected size $ O (n^{1 + 1/k}) $ that has expected total update time $ O (k m \log{n}) $.
These guarantees hold against an oblivious adversary.
\end{theorem}
Using the reduction of Lemma~\ref{lem:spanner decremental to fully dynamic}, these guarantees carry over to the fully dynamic setting.
\begin{theorem}[Restatement of Theorem~\ref{thm:fully dynamic spanner}]
Given any unweighted, undirected graph undergoing edge insertions and deletions, there is a fully dynamic algorithm for maintaining a spanner of stretch $ 2k - 1 $ and expected size $ O (n^{1 + 1/k} \log{n}) $ that has expected amortized update time $ O (k \log^2{n}) $.
These guarantees hold against an oblivious adversary.
\end{theorem}

The decremental algorithm is obtained as follows:
In a preprocessing step, the algorithm samples the random shift values for the nodes from the exponential distribution and additionally a uniformly random permutation $ \pi $ on the nodes.
The sampling of the random shift values is repeated until $ \delta_u < k $ for all $u \in V$.
By Claim~\ref{claim:bound on random shifts} this condition holds with probability at least $ 1 - 1/c $.
Thus, by the waiting time bound, we need to repeat the sampling at most a constant number of times for the condition to hold.
As each round of sampling takes time $ O (n) $, this preprocessing step requires an additional $ O (n) $ in the total update time.

We can then readily use Algorithm~\ref{alg:ES_tree} from Section~\ref{sec:decremental LDD} to maintain a shortest path tree up to depth $ 2 k $ from $ s $ in the graph $ G' $, as defined above.
For maintaining the spanner dynamically, we need to extend the algorithm to maintain the set $ C' (x) $ for every node $ x $.
Using the arguments introduced in Section~\ref{sec:decremental LDD}, this can be done in a straightforward way:
Every time a node $ x $ changes its level in the tree or changes its cluster $ c (x) $, it (1) recomputes the set $ C' (x) $ in time $ O (\deg (x)) $ and stores it in a hash set and (2) informs each neighbor about the change and updates the set $ C' (y) $ of each neighbor $ y $ by setting the entry corresponding to the edge $ (x, y) $ accordingly.
Both (1) and (2) require (expected) time $ O (\deg (x)) $.
As the maximum level in the tree is $ O (k) $ and at each node changes its clustering at a fixed level at most $ O (\log n) $ times in expectation, the expected total update time of our algorithm is $ O (k m \log{n}) $ as desired.


==> chapters/lowstretchtree/static.tex <==
\subsection{Static Low-Diameter Decomposition}~\label{sec:staticLDD}

In the following, we review the static algorithm for constructing a low-diameter decomposition clustering due to Miller et al.~\cite{MillerPX13}. Let $G=(V,E)$ be an unweighted, undirected multigraph $G$, and let $\beta \in (0,1)$ be some parameter. Our goal is to assign each node $u$ to exactly one node $c(u)$ from $V$. Let $C(u) \subset V$ denote the set of nodes assigned to node $u$, i.e., $C(u) \coloneqq \set{v \in V}{ c(v) = u}$. For each node $u$, we initially set $C(u)= \varnothing $ and pick independently a \emph{shift} value $\delta_u$ from $\expdis(\beta)$. Next, we assign each node $u$ to a node $v$, i.e., set $c(u) = v$ and add $u$ to $C(v)$, if $v$ is the node that minimizes the \emph{shifted distance} $m_v(u)\coloneqq \dist(u,v) - \delta_v$. Finally, we output all clusters that are non-empty. The above procedure is summarized in Algorithm~\ref{alg:partition}.

\begin{algorithm2e}[htb!]
\caption{Partitioning Using Exponentially Shifted Shortest Paths}
\label{alg:partition}

\BlankLine
\KwData{Multigraph $G=(V,E)$, parameter $\beta \in (0,1)$}
\KwResult{Decomposition of $G$}
\BlankLine

For each $u \in V$, set $C(u)=\varnothing$ and pick $\delta_u$ independently from $\expdis(\beta)$ \;
Assign each $u \in V$ to $c(u) \gets \arg \min_{v \in V} \{\dist(u,v) - \delta_v\}$\;
For each $v \in V$, set $C(u) \gets \set{v \in V}{c(v) = u}$\;
Return the clustering $\set{C(u)}{C(u) \neq \varnothing}$
\end{algorithm2e}

The following theorem gives bounds on the strong diameter and the number of inter-cluster edges output by the above partitioning.

\begin{theorem}[\cite{MillerPX13}, Theorem~1.2] \label{thm: Miller_LDD} Given an undirected, unweighted multigraph graph $G=(V,E)$ and a parameter $\beta \in (0,1)$, Algorithm~\ref{alg:partition} produces a $(\beta, 2 d \cdot(\log n/\beta))$-decomposition such that the guarantee on the number of inter-cluster edges holds in expectation, while the diameter bound holds with probability at least $1-1/n^d$, for any $d \geq 1$.
\end{theorem}

Here, the the diameter bound holds when the maximum shift value of any node is at most $ d \log n/\beta $, which happens with probability $1-1/n^d$.
We remark that in the work of Miller et al., the above guarantees are stated only for undirected, unweighted \emph{simple} graphs. However, by~Lemma 4.4 in~\cite{MillerPX13}, we get that each edge $e \in E$~(regardless of whether $E$ allows parallel edges) is an inter-cluster edges with probability at most $\beta$. By linearity of expectation, it follows that the (expected) number of inter-cluster edges in the resulting decomposition is at most $\beta m$, thus showing that the algorithm naturally extends to multigraphs.

For technical reasons, it is not sufficient in the analysis of our decremental LDD algorithm to apply Theorem~\ref{thm: Miller_LDD} in a black-box manner.
We thus review the crucial properties of the clustering algorithm, which we will exploit for bounding the number of changes made to inter-cluster edges in the decremental algorithm. Following~\cite{MillerPX13}, for each edge $e=(u,v) \in E$, let $w$ be the \emph{mid-point} of $e$, i.e., the imaginary node in the ``middle'' of edge $ e $ that is at distance $ \tfrac{1}{2} $ to both $ u $ and $ v $. Lemma~4.3 in \cite{MillerPX13} states that if $u$ and $v$ belong to two different clusters, i.e., $c(u) \neq c(v)$, then the shifted-distances $m_{c(u)}(w)$ and $m_{c(v)}(w)$ are within $1$ of the minimum shifted distance to $w$.

\begin{lemma}[\cite{MillerPX13}]\label{lem:inter cluster edge implies mid-point condition}
Let $e=(u,v)$ be an edge with mid-point $w$ such that $c(u) \neq c(v)$ in Algorithm~\ref{alg:partition}. Then $m_{c(u)}(w)$ and $m_{c(v)}(w)$ are within $1$ of the minimum shifted distance to $w$. 
\end{lemma}

Lemma 4.4 of~\cite{MillerPX13} shows that the probability that the smallest and the second smallest shifted distances to $w$ are within $c$ of each other is at most $c \cdot \beta$.

\begin{lemma}[\cite{MillerPX13}]\label{lem:probability of mid-point condition}
Let $ e = (u,v) $ be an edge with mid-point $ w $.
Then \[ \Pr [| m_{c(u)}(w) - m_{c(v)}(w) | \leq c] \leq c \cdot \beta. \]
\end{lemma}

Setting $c=1$, this gives the desired bound of $ \beta $ for the probability of an edge being an inter-cluster edge in Theorem~\ref{thm: Miller_LDD}.


\paragraph*{Implementation.} 
Na\"ively, we could implement Algorithm~\ref{alg:partition} by computing $c(u)$ for each node $u \in V$ in $\tilde{O}(m)$, thus leading to a $\tilde{O}(mn)$ time algorithm. In the following, using standard techniques, we show that this running time can be reduced to $\tilde{O}(m)$.

To this end, let $\delta_{\max} \coloneqq \max_{u \in V} \delta_u$. We begin with the following augmentation of the input graph $G$: add a new source $s$ to $G$ and edges $(s,u)$ of weight $(\delta_{\max} - \delta_u) \geq 0$, for every $u \in V$. Let $\hat{G}=(V \cup \{s\},\hat{E},\hat{w})$ denote the resulting graph. We claim that the sub-trees below the source $s$ in the shortest path tree of $\hat{G}$ rooted at $s$ give us the clustering output by Algorithm~\ref{alg:partition} for the graph $G$. To see this, suppose that we instead added edges of weight $-\delta_u$ to $s$, for every $u \in V$. Then it is easy to check that for every $u \in V$, distance between $s$ and $u$ is exactly $ \min_{v \in V} (\dist(u,v) - \delta_v) = \min_{v \in V} m_v(u)$. Thus the node $v$ attaining the minimum is exactly the root of the sub-tree below the source $s$ that contains $v$. Now, adding $\delta_{\max}$ to all edges incident to the source increases all distances to $s$ by $\delta_{\max}$, and thus does not affect the shortest path tree.

Now, note that we could use Dijkstra's algorithm to construct the shortest path tree of $\hat{G}$, and modify it appropriately to output the clustering. However, for reasons that will become clear in the next section, we need to modify Dijkstra's algorithm in a specific way. This modification can be viewed as mimicking a BFS computation on a graph with special \emph{integral} edge lengths. 

We start by observing that due to the random shift values, the weight of the edges incident to the source $s$ in $\hat{G}$ are not integers. Since we only want to deal with \emph{integral} weights, we round down all the $\delta_u$ values to $\floor{\delta_u}$ and modify the weights of these edges using the new rounded values. Let $G'=(V \cup \{s\}, \hat{E}, w')$ denote the modified graph. Note that due to the rounding, we need to introduce some tie-breaking scheme in $G'$, such that  every clustering of $G'$ matches exactly the same clustering in $\hat{G}$, and vice versa. Naturally, the fractional parts of the rounded values, i.e., $\delta_u - \floor{\delta_u}$, define an ordering on the nodes (if they are sorted in ascending order), and this ordering can be in turn used to break ties whenever two rounded distances are equal in $G'$. In their PRAM implementation, Miller et al.~\cite{MillerPX13} observed that this ordering can emulated by a random permutation. This is due to the fact that the shifts are generated independently, and that the exponential distribution is memoryless. 

The main motivation for using random permutations in previous works was to avoid errors that might arise from the machine precision. In our work, breaking ties according to a random permutation on the nodes is one of their algorithmic ingredients that allows us to obtain an efficient dynamic variant of the clustering. Below, we give specific implementation details about how our clustering interacts with random priorities in the static setting. 

Given the graph $G'$ and a distinguished source node $s \in V'$,  Dijkstra's classical algorithm maintains an upper-bound on the shortest-path distance between each node $u \in V$ and $s$, denoted by $\ell(u)$. Initially, it sets $\ell(u) = \infty$, for each $u \in V$ and $\ell(s) = 0$. It also marks every node unvisited. Moreover, for each node $u \in V$, the algorithm also maintains a pointer $p(u)$ (initially set to $\nil$), which denotes the parent of $u$ in the current tree rooted at $s$. Using these pointers, we can maintain the cluster pointer $c(u)$, for each $u \in V$. This follows from the observation that in order to compute the cluster of $u$, it suffices to know the cluster of its parent. Formally we have the following rule.

\begin{observation} \label{obs: clusterUpdate}
Let $p(\cdot)$ be the parent pointers. Then for each $u \in V$, we can determine the cluster pointer $c(u)$ using the following rule:

\[
	c(u) =  \begin{cases} 
    u & \text{\emph{if} } p(u)=s \\
    c(p(u))      & \text{\emph{otherwise}}.
  \end{cases}
\]
\end{observation}

Now, at each iteration, Dijkstra's algorithm selects an unvisited node $u$ with the smallest $\ell(u)$, marks it as visited, and \emph{relaxes} all its edges. In the standard relaxation, for each edge $(u,v) \in E'$ the algorithm sets $\ell(v) \gets \min\{\ell(v), \ell(u) + w'(u,v)\}$ and updates $p(v)$ accordingly. Here, we present a relaxation according to the following tie-breaking scheme. Let $\pi$ be a random permutation on $V$. For $u, v \in V$, we write $\pi(u) < \pi(v)$ if $u$ appears before $v$ in the permutation $\pi$.
Now, when relaxing an edge $(u,v) \in E'$, we set $u$ to be the parent of $v$, i.e., $p(v) = u$, and $\ell(v) = \ell(u) + w'(u,v)$, if the following holds
\begin{align} \label{eq: breakingTies}
\begin{split}
\ell(v) & > \ell(u) + w'(u,v), \text{ or} \\
\ell(v) & = \ell(u) + w'(u,v) \text{ and } \pi(c(v)) > \pi(c(u)).
\end{split}
\end{align}

After each edge relaxation, we also update the cluster pointers using  Observation~\ref{obs: clusterUpdate}. We continue the algorithm until every node is visited. As usual, we maintain the unvisited nodes in a heap $Q$, keyed by the their estimates $\ell(v)$. This procedure is summarized in Algorithm~\ref{alg:ModDijkstra}.

\begin{algorithm2e}[htb!]
\caption{Modified Dijkstra}
\label{alg:ModDijkstra}
\KwData{Graph $G'=(V \cup \{s\},E',w')$}
\KwResult{Decomposition of $G$}
\BlankLine

Generate random permutation $\pi$ on $V$\;
%\BlankLine
\ForEach{$u \in V$}{
Set $\ell(u) = \infty$\;
Set $p(u) = \nil$\;
Set $c(u) = \nil$\;
}

Set $\ell(s) = 0$\;
\BlankLine

Add every $u \in V \cup \{s\}$ into heap $Q$ with key $\ell(u)$\;
\While{heap $ Q $ is not empty}{
	    Take node $ u $ with minimum key $ \lev (u) $ from heap $ Q $ and remove it from $ Q $ \;
		\ForEach{neighbor $ v $ of $ u $}{
		\Relax{$u$, $v$, $w'$, $\fraction$} \;
		\eIf{$ p(v) = s $}{
			Set $ c (v) = v  $\;
		}{
			Set $ c (v) = c( p(v)) $\;
		}
	}
}

\Procedure{\Relax{$u$, $v$, $w'$, $\fraction$}}{
	\uIf{$\ell(v) > \ell(u) + w'(u,v)$}{
		Set $\ell(v) = \ell(u) + w'(u,v)$\;
		Set $p(v) = u$\;
		}
	\uElseIf{$\ell(v) = \ell(u) + w'(u,v)$ \emph{and} $\pi(c(v)) > \pi(c(u))$}{
     Set $p(v) = u$ \;}
}
\end{algorithm2e}


Correctness of Algorithm~\ref{alg:ModDijkstra} follows by our above discussion. Moreover, the running time of the algorithm is asymptotically bounded by the running time of Dijkstra's classical algorithm and the time to generate a random permutation. It is well known that the former runs in $\tilde{O}(m)$ time and the latter can be generated in $O(n)$ time (see e.g., Knuth Shuffle~\cite{BermanK76}), thus giving us a total $\tilde{O}(m)$ time.


==> chapters/reachabilityminors/abstract.tex <==
Graph Sparsification aims at compressing large graphs into smaller ones while preserving important characteristics of the input graph. In this chapter we study Vertex Sparsifiers, i.e., sparsifiers whose goal is to reduce the number of vertices. We focus on the following notions:

(1) Given a digraph $G=(V,E)$ and terminal vertices $K \subset V$ with $|K| = k$, a (vertex) reachability sparsifier of $G$ is a digraph $H=(V',E')$, $K \subset V'$ that preserves all reachability information among terminal pairs. In this chapter we introduce the notion of reachability-preserving minors (RPMs) , i.e., we require $H$ to be a minor of $G$. We show any directed graph $G$ admits a RPM $H$ of size $O(k^3)$, and if $G$ is planar, then the size of $H$ improves to $O(k^{2} \log k)$. We complement our upper-bound by showing that there exists an infinite family of grids such that any RPM must have $\Omega(k^{2})$ vertices.

(2) Given a weighted undirected graph $G=(V,E)$ and terminal vertices $K$ with $|K|=k$, an exact (vertex) cut sparsifier of $G$ is a graph $H$ with $K \subset V'$ that preserves the value of minimum-cuts separating any bipartition of $K$. We show that planar graphs with all the $k$ terminals lying on the same face admit exact cut sparsifiers of size $O(k^{2})$ that are also planar. Our result extends to flow and distance sparsifiers. It improves the previous best-known bound of $O(k^22^{2k})$ for cut and flow sparsifiers by an exponential factor, and matches an $\Omega(k^2)$ lower-bound for this class of graphs. 



==> chapters/reachabilityminors/cutflowdistance.tex <==
\section{An Exact Cut Sparsifier of Size $O(k^2)$} \label{sec: upperCut}
In this section we show that given a $k$-terminal planar graph, where all terminals lie on the same face, one can construct a quality-$1$ cut sparsifier of size $O(k^{2})$. Note that it suffices to consider the case when all terminals lie on the \emph{outer} face. %Our approach closely follows the work of Gitler~\cite{Gitler91} in the context of Wye-Delta reducibility of graphs, which does not consider preservation of terminal cuts. Apart from bringing his work to the vertex sparsification community, we also fill in some gaps and provide the necessary details for applying his technique to the cut setting.
%The basic approach is as follows. Given a $k$-terminal planar graph with terminals lying on the outer face, we first embed it into some large grid with terminals lying on the boundary of the grid. Subsequently, we show how to embed the resulting grid into a `more suitable' graph, which we will refer to as `half-grid'. Finally, using the Wye-Delta operations, we reduce 'half-grid'  into another graph whose number of vertices can be bounded by $O(k^{2})$. Since we shall argue that the above graph reductions preserve exactly all terminal minimum cuts, our result follows. 
%\vspace{-0.4cm}
We first present some basic tools. 
\subsection{Basic Tools}
\paragraph*{Wye-Delta Transformations. }
In this section we investigate the applicability of some graph reduction techniques that aim at reducing the number of non-terminals in a $k$-terminal graph. %Khan and Raghavendra~\cite{KhanR14} were the first to apply such techniques in the context of Vertex Cut Sparsification for tree networks. 
We start by reviewing the so-called \emph{Wye-Delta} operations in graph reductions. These operations consist of five basic rules, which we describe below. (See Fig.~\ref{fig:wyedelta} for illustrations.)%It is easy to see that each of these rules preserve exactly all terminal cuts if appropriate edge weights are used on the reduced graph. 
\begin{enumerate}
	\setlength\itemsep{0.1em}
	\item \emph{Degree-one reduction:} Delete a degree-one non-terminal and its incident edge.
	\item \emph{Series reduction:} Delete a degree-two non-terminal $y$ and its incident edges $(x,y)$ and $(y,z)$, and add a new edge $(x,z)$ of capacity $\min\{\cc(x,y), \cc(y,z)\}$.
	\item \emph{Parallel reduction:} Replace all parallel edges by a single edge whose capacity is the sum over all capacities of parallel edges.
	\item \emph{Wye-Delta transformation:} Let $x$ be a degree-three non-terminal with neighbours $\delta(x) = \{u,v,w\}$. Assume w.l.o.g.\footnote{Suppose there exist a pair $(u,v) \in \delta(x)$ with $\cc(u,x) + \cc(v,x) < \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. Then we can simply set $\cc(w,x) = \cc(u,x) + \cc(v,x)$, since any terminal minimum cut would cut the edges $(u,x)$ and $(v,x)$ instead of the edge $(w,x)$.} that for any pair $(u,v) \in \delta(x)$, $\cc(u,x) + \cc(v,x) \geq \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. Then we can delete $x$ (along with all its incident edges) and add edges $(u,v),(v,w)$ and $(w,u)$ with capacities $(\cc(u,x)+\cc(v,x)-\cc(w,x))/2$, $(\cc(v,x)+\cc(w,x)-\cc(u,x))/2$ and $(\cc(u,x)+\cc(w,x)-\cc(v,x))/2$, respectively. 
	\item \emph{Delta-Wye transformation:} Delete the edges of a triangle connecting $x$, $y$ and $z$, introduce a new non-terminal vertex $w$ and add new edges $(w,x)$, $(w,y)$ and $(w,z)$ with edge capacities $\cc(x,y) + \cc(x,z),$ $\cc(x,y) + \cc(y,z)$ and $\cc(x,z) + \cc(y,z)$ respectively.
\end{enumerate}

\input{chapters/reachabilityminors/figure_wyeDeltaTrans}

The following lemma (which follows from the above definitions) shows that the above rules preserve exactly all terminal minimum cuts.


\begin{lemma} \label{lemm: rules} Let $G$ be a $k$-terminal graph and $G'$ be a $k$-terminal graph obtained from $G$ by applying one of the rules $1-5$. Then $G'$ is a quality-$1$ cut sparsifier of $G$.
\end{lemma}

For our application, it will be useful to enrich the set of rules by introducing two new operations. These operations can be realized as series of the operations 1-5. (See Fig.~\ref{fig:edgedeletion} and \ref{fig:edgereplacement} for illustrations.)
\begin{enumerate}[resume]
	\item \emph{Edge deletion (with vertex $x$):} For a degree-three non-terminal with neighbours $u,v$, the edge $(u,v)$ can be deleted, if it exists. To achieve this, we use a Delta-Wye transformation followed by a series reduction.
	
	
	
	\item \emph{Edge replacement:} For a degree-four non-terminal vertex with neighbours $x,u,v,w$, if the edge $(x,u)$ exists, then it can be replaced by the edge $(v,w)$. To achieve this, we use a Delta-Wye transformation followed by a Wye-Delta transformation.
\end{enumerate}

\input{chapters/reachabilityminors/figure_edgeDeletion}
\input{chapters/reachabilityminors/figure_edgeReplacement}

A $k$-terminal graph $G$ is \emph{Wye-Delta} reducible to another $k$-terminal graph $H$, if $G$ is reduced to $H$ by repeatedly applying one of the operations 1-7. %We obtain the following lemma, whose proof we defer to Appendix~\ref{app: preli}.


\begin{lemma} \label{lemm: cutReducability} Let $G$ and $H$ be $k$-terminal graphs. Moreover, let $G$ be Wye-Delta reducible to $H$. Then $H$ is a quality-$1$ cut sparsifier of $G$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: cutReducability}]
	Observe that the rules 1-7 do not affect any terminal vertex and each rule preserves exactly all terminal minimum cuts by Lemma \ref{lemm: rules}. An induction on the number of rules needed to reduce $G$ to $H$ proves the claim.
\end{proof}
%\begin{proof}
%Observe that the rules 1-7 do not affect any terminal vertex and each rule preserves exactly all terminal minimum cuts by Lemma \ref{lemm: rules}. An induction on the number of rules needed to reduce $G$ to $H$ proves the claim.
%\end{proof}
%\vspace{-0.5cm}
\paragraph*{Grid Graphs.} %Throughout the paper we will be dealing with two special types of graphs. 
A \emph{grid} graph is a graph with $n \times n$ vertices $\{(u,v) : u,v = 1,\ldots, n\}$, where $(u,v)$ and $(u',v')$ are adjacent if $|u' -u| + |v'-v| = 1$. For $k < n$, a \emph{half-grid} graph with $k$ terminals is a graph $T^{n}_k = (V,E)$ with $K \subset V$ and $n(n+1)/2$ vertices $\{(i,j) : i \leq j \text{ and } i,j=1,\ldots,n  \}$, where $(i,j)$ and $(i',j')$ are connected by an edge if $|i'-i| + |j'-j| = 1$, and additional diagonal edges between $(i,i)$ and $(i+1,i+1)$ for $i = 1,\ldots, n-1$. Moreover, each terminal vertex in $T^{n}_k$ must be one of its diagonal vertices, i.e., every $x \in K$ is of the form $(m,m)$ for some $m \in \{1,\ldots,n\}$. Let $\hat{T}^{n}_{k}$ be the same graph as $T^{n}_k$ but excluding the diagonal edges. 

\paragraph*{Graph Embeddings.}\label{sec: graphEmbeddings} 
Throughout this paper, we will be dealing with the embedding of a planar graph into a square \emph{grid} graph. One way of drawing graphs in the plane are \emph{orthogonal grid-embeddings}~\cite{Valiant81}. In such a setting, the vertices correspond to distinct points and edges consist of alternating sequences of vertical and horizontal segments. Equivalently, one can view this as drawing our input graph as a subgraph of some grid. Formally, a \emph{node-embedding} $\rho$ of $G_1=(V_1,E_1)$ into $G_2=(V_2,E_2)$ is an injective mapping that maps $V_1$ into $V_2$, and $E_1$ into paths in $G_2$, i.e., $(u,v)$ maps to a path from $\rho(u)$ to $\rho(v)$, such that every pair of paths that correspond to two different edges in $G_1$ is vertex-disjoint (except possibly at the endpoints). If $G_2$ is a planar graph, then $\rho(G_1)$ and $G_1$ are also planar. Thus, if $G_1$ and $G_2$ are planar we then refer to $\rho$ as an \emph{orthogonal embedding}. Moreover, given a planar graph $G_1$ drawn in the plane, the embedding $\rho$ is called \emph{region-preserving} if $\rho(G_1)$ and $G_1$ have the same planar topological embedding.

%\input{figure_orthogonalEmbedding}

%We know turn our attention to the case when 
Let $G_1$ be a $k$-terminal graph. Since the embedding does not affect the vertices of $G_1$, the terminals of $G_1$ are also terminals in $\rho(G_1)$. Although the embedding does not consider capacity of the edges in $G_1$, we can still guarantee that such an embedding preserves all terminal minimum cuts, for which we make use of the following operation:
\begin{enumerate}
	\item \emph{Edge subdivision: } Let $(u,v)$ be an edge of capacity $\cc(u,v)$. Delete $(u,v)$, introduce a new vertex $w$ and add edges $(u,w)$ and $(w,v)$, each of capacity $\cc(u,v)$. 
\end{enumerate}

The following lemma shows that a node-embedding is a cut preserving mapping.
%The proof of the following Lemma is deferred to Appendix~\ref{app: preli}.
\begin{lemma} \label{lemm: cutembedding}
	Let $\rho$ be a node-embedding and let $G_1$ and $\rho(G_1)$ be $k$-terminal graphs defined as above. Then $\rho(G_1)$ preserves exactly all terminal minimum cuts of $G$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: cutembedding}]
	We can view each path obtained from the embedding as taking the edge corresponding to the path endpoints in $G_1$ and performing edge subdivisions finitely many times. We claim that such subdivisions preserve all terminal cuts. 
	
	Indeed, let us consider a single edge subdivision for $(u,v)$ (the general claim then follows by induction on the number of edge subdivisions). Fix $S \subset K$ and consider some $S$-separating minimum cut $(U,V \setminus U)$ in $G_1$ cutting $(u,v)$. Then, in the transformed graph $\rho(G_1)$, we can simply cut either the edge $(u,w)$ or $(w,v)$. Since by construction, the new edge has the same capacity as the subdivided edge, we get that $\capacity_{\rho(G_1)}(\delta(U)) = \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \leq \mincut_{G_1}(S,K \setminus S)$. 
	
	Furthermore, since $G_1$ is obtained by contracting two edges of the same capacity of $\rho(G_1)$, for any $S$-separating minimum cut $(U, V \setminus U)$ in $\rho(G_1)$, we have $\capacity_{\rho(G_1)}(\delta(U)) \geq \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \geq \mincut_{G_1}(S,K \setminus S)$. Combining the above gives the lemma. 
\end{proof}
%\begin{proof}
%We can view each path obtained from the embedding as taking the edge corresponding to the path endpoints in $G_1$ and performing edge subdivisions finitely many times. We claim that such subdivisions preserve all terminal cuts. 
%
%Indeed, let us consider a single edge subdivision for $(u,v)$ (the general claim then follows by induction on the number of edge subdivisions). Fix $S \subset K$ and consider some $S$-separating minimum cut $(U,V \setminus U)$ in $G_1$ cutting $(u,v)$. Then, in the transformed graph $\rho(G_1)$, we can simply cut either the edge $(u,w)$ or $(w,v)$. Since by construction, the new edge has the same capacity as the subdivided edge, we get that $\capacity_{\rho(G_1)}(\delta(U)) = \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \leq \mincut_{G_1}(S,K \setminus S)$. 
%
%Furthermore, since $G_1$ is obtained by contracting two edges of the same capacity of $\rho(G_1)$, for any $S$-separating minimum cut $(U, V \setminus U)$ in $\rho(G_1)$, we have $\capacity_{\rho(G_1)}(\delta(U)) \geq \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \geq \mincut_{G_1}(S,K \setminus S)$. Combining the above gives the lemma. 
%\end{proof}
\subsection{Our Construction}
In this section  we construct our exact cut sparsifier and prove that any planar $k$-terminal graph with all terminals lying on the same face admits a cut sparsifier of size $O(k^2)$ that is also planar.
\subsubsection{Embedding into Grids} \label{EmbeddingGrid}

It is well-known that one can obtain an orthogonal embedding of a planar graph with maximum-degree at most three into a grid (see Valiant~\cite{Valiant81}). However, our input planar graph can have arbitrarily large maximum degree. In order to be able to make use of such an embedding, we need to first reduce our input graph to a bounded-degree graph while preserving planarity and all terminal minimum cuts. We achieve this by making use of a \emph{vertex splitting} technique, which we describe below. 

Given a $k$-terminal planar graph $G'=(V',E',c')$ with $K \subset V'$ lying on the outer face, vertex splitting produces a $k$-terminal planar graph $G=(V,E,c)$ with $K \subset V$ such that the maximum degree of $G$ is at most three. Specifically, for each vertex $v$ of degree $d>3$ with neighboring vertices $u_1,\ldots,u_{d}$, we delete $v$ and introduce new vertices $v_1, \ldots, v_d$ along with edges $\{(v_i,v_{i+1}) : i=1,\ldots,d-1\}$, each of capacity $C+1$, where $C=\sum_{e \in E'} c'(e)$. Further, we replace the edges $\{(u_i,v) : i = 1,\ldots,d\}$ with $\{(u_i,v_i) : i = 1,\ldots,d\}$, each of corresponding capacity. If $v$ is a terminal vertex, we set one of the $v_i$'s to be a terminal vertex. It follows that the resulting graph $G$ is planar and terminals can be still embedded on the outer face. Note that while the degree of every vertex $v_i$ is at most $3$, the degree of any other vertex is not affected. %The proof of the claim below appears in Appendix~\ref{app: upperCut}.

\begin{claim} \label{claim: embedding}
Let $G'$ and $G$ be $k$-terminal graphs defined as above. Then $G$ preserves exactly all minimum terminal cuts of $G'$, i.e., $G$ is a quality-$1$ cut sparsifier of $G'$.
\end{claim} 
\begin{proof}%[Proof of Claim \ref{claim: embedding}]
	It suffices to prove the case where $G$ is obtained from $G'$ by a single vertex splitting. Then the claim follows by induction on the number of vertex splittings required to transform $G'$ to $G$.
	
	Let $S \subset K$ and $(U, V \setminus U)$ be an $S$-separating cut in $G$ of size $\mincut_G(S,K \setminus S)$. Suppose towards contradiction that $\delta(U)$ contains an edge of the form $(v_j,v_{j+1})$, for some $j$, which in turn gives that $\capacity(\delta(U)) \geq C + 1$. Then we can move all the points $v_i$ to one of the sides of the cut $(U, V \setminus S)$ and obtain a new $S$-separating cut in $G$ of cost at most $C$, contradicting the fact that $(U, V \setminus U)$ is a minimum terminal cut. Hence, it follows that $\delta(U)$ uses either edges that are in both $G$ and $G'$ or edges of the form $(u_i,v_i)$, which by construction have the same capacity as the edges $(u_i,v)$ in $G'$. Thus, an $S$-separating minimum cut in $G$ corresponds to an $S$-separating minimum cut in $G'$ of the same cost. Since $S$ is chosen arbitrarily, the claim follows.
\end{proof}
%\begin{proof}
%It suffices to prove the case where $G$ is obtained from $G'$ by a single vertex splitting. Then the claim follows by induction on the number of vertex splittings required to transform $G'$ to $G$.
%
%Let $S \subset K$ and $(U, V \setminus U)$ be an $S$-separating cut in $G$ of size $\mincut_G(S,K \setminus S)$. Suppose towards contradiction that $\delta(U)$ contains an edge of the form $(v_j,v_{j+1})$, for some $j$, which in turn gives that $\capacity(\delta(U)) \geq C + 1$. Then we can move all the points $v_i$ to one of the sides of the cut $(U, V \setminus S)$ and obtain a new $S$-separating cut in $G$ of cost at most $C$, contradicting the fact that $(U, V \setminus U)$ is a minimum terminal cut. Hence, it follows that $\delta(U)$ uses either edges that are in both $G$ and $G'$ or edges of the form $(u_i,v_i)$, which by construction have the same capacity as the edges $(u_i,v)$ in $G'$. Thus, an $S$-separating minimum cut in $G$ corresponds to an $S$-separating minimum cut in $G'$ of the same cost. Since $S$ is chosen arbitrarily, the claim follows.
%\end{proof}

Let $G=(V,E)$ be a $k$-terminal graph obtained by vertex splitting of all vertices of degree larger than $3$ of $G'=(V',E')$. Further, let $n' = |V'|$, $m' = |E'|$, $n = |V|$ and $m = |E|$. Then it is easy to show that $n \leq 2 m'$ and $m \leq m' + n \leq 3m'$. Since $G'$ is planar, we have that $n = O(n')$ and $m = O(n')$. Thus, by just a linear blow-up on the size of vertex and edge sets, we may assume w.l.o.g. that our input graph is a planar graph of degree at most three. 

Valiant~\cite{Valiant81} and Tamassia et al.~\cite{TamassiaT89} showed that a $k$-terminal planar graph $G$ with $n$ vertices and degree at most three admits an orthogonal region-preserving embedding into some square grid of size $O(n) \times O(n)$. By Lemma \ref{lemm: cutembedding}, we know that the resulting graph exactly preserves all terminal minimum cuts of $G$. We remark that since the embedding is region-preserving, the outer face of the input graph is embedded to the outer face of the grid. Therefore, all terminals in the embedded graph lie on the outer face of the grid. Performing appropriate edge subdivisions, we can make all the terminals lie on the boundary of some possibly larger grid. Further, we can add dummy non-terminals and zero edge capacities to transform our graph into a full-grid $H$. We observe that the latter does not affect any terminal min-cut. The above leads to the following:
\begin{lemma} \label{lemm: embeddingGrids}
Given a $k$-terminal planar graph $G$, where all terminals lie on the outer face, there exists a $k$-terminal grid graph $H$, where all terminals lie on the boundary such that $H$ preserves exactly all terminal minimum cuts of $G$. The resulting graph has $O(n^2)$  vertices and edges.
\end{lemma}

%\vspace{-0.3cm}
\subsubsection{Embedding Grids into Half-Grids}

Next, we show how to embed square grids into half-grid graphs (see Section \ref{sec: preli}), which will facilitate the application of Wye-Delta transformations. The existence of such an embedding was claimed in the thesis of Gitler~\cite{Gitler91}, but no details on its construction were given. 

Let $G$ be a $k$-terminal square grid on $n \times n$ vertices where terminals lie on the boundary of the grid. We obtain the following:
%\input{figure_halfgrid}
\begin{figure}[t] 
\begin{center}
\includegraphics[scale=1]{chapters/reachabilityminors/fhalfgrid}
\end{center}
\caption{Embedding grid into half-grid. Black vertices represent terminals while white vertices represent non-terminals. The counter-clockwise ordering starts at the top right terminal. Coloured edges and paths correspond to the mapping of the respective edges: blue for edges $((i,1),(i,2))$, red for edges $((n-1,j),(n,j))$, green for edges $((1,j),(2,j))$ and yellow for edges $((i,n-1), (i,n))$, where $i,j = 2,\ldots,n-1$. }
\label{fig: halfgridConst}
\end{figure}

\begin{lemma} \label{lemm: embeddingHalfGrid}
There exists a node embedding of the grid $G$ into $T^{\ww}_{k}$, where $\ww  = 4n-3$. 
\end{lemma}
\begin{proof}
Our construction works as follows (See Fig.~\ref{fig: HalfGridRed} for an example). We first fix an ordering on the vertices lying on the boundary of the grid in the order induced by the grid. Then we embed each vertex according to that order into the diagonal vertices of the half-grid, along with the edges that form the boundary of the grid. The sub-grid obtained by removing all boundary vertices is embedded appropriately into the upper-part of the half-grid. Finally, we show how to embed edges between the boundary and the sub-grid vertices and argue that such an embedding is indeed vertex-disjoint for any pair of paths.

\input{chapters/reachabilityminors/figure_halfgridReduction}

We start with the embedding of the vertices of $G$. Let us first consider the boundary vertices. The ordering imposed on these vertices can be viewed as starting with the upper-right vertex $(1,n)$ and visiting the rest of vertices in a counter-clockwise direction until reaching the vertex $(2,n)$. We map the vertices on the boundary as follows.
\begin{enumerate}
\setlength\itemsep{0.1em}
\item The vertex $(1,j)$ is mapped to the vertex $(n-j+1,n-j+1)$ for $j=2,\ldots,n$, 
\item The vertex $(i,1)$ is mapped to the vertex $(n+i-1,n+i-1)$ for $i=1,\ldots,n-1$,
\item The vertex $(n,j)$ is mapped to the vertex $(2n+j-2,2n+j-2)$ for $j=1,\ldots,n-1$,
\item The vertex $(i,n)$ is mapped to the vertex $(4n-i-2,4n-i-2)$  for $i=2,\ldots,n$.
\end{enumerate} 
Now we consider the vertices that belong to the induced sub-grid $S$ of $G$ of size $(n-2)^2$ when removing the boundary vertices of our input grid. We map the vertex $(i,j)$ to the vertex $(n+i-1, 2n+j-2)$ for $i,j=2,\ldots,n-1$. In other words, for every vertex of $S$ we make a vertical shift by $n-1$ units and an horizontal shift by $2n-2$ units. By construction, it is not hard to check that every vertex of $G$ is mapped to a different vertex of $T^{\ww}_{k}$ and all terminal vertices lie on the diagonal of $T^{\ww}_{k}$. 

We continue with the embedding of the edges of $G$. First, every edge between two boundary vertices in $G$ is embedded to the edge between the corresponding mapped diagonal vertices of $T^{\ww}_{k}$, except the edge between $(1,n)$ and $(2,n)$. For this edge, we define an edge embedding between the corresponding vertices $(1,1)$ and $(4n-4,4n-4)$ of $T^{\ww}_{k}$ by using the path:
\begin{align*} 
(1,1) \rightarrow (1,2) \rightarrow \ldots & \rightarrow (1,4n-3) \rightarrow (2,4n-3)  \\ 
&\rightarrow \ldots \rightarrow (4n-4,4n-3) \rightarrow (4n-4,4n-4).
\end{align*}

Next, every edge of the sub-grid $S$ is embedded in to the edge connecting the mapped endpoints of that edge in $T^{\ww}_{k}$. In other words, if $(i,j)$ and $(i',j')$ were connected by an edge $e$ in $S$, then $(n+i-1, 2n+j-2)$ and $(n+i'-1, 2n+j'-2)$ are connected by an edge $e'$ in $T^{\ww}_{k}$ and $e$ is mapped to $e'$. Finally, the only edges that remain are those connecting a boundary vertex of $G$ with a boundary vertex of $S$. We distinguish four cases depending on the edge position. 
\begin{enumerate}
\setlength\itemsep{0.1em}
\item The edge $((i,2), (i,1))$ is mapped to the horizontal path given by:
\begin{align*}
	(n+i-1,2n) & \rightarrow (n+i-1, 2n-1) \\ 
	& \rightarrow \ldots \rightarrow (n+i-1,n+i-1) \text{ for } i = 2,\ldots,n-1 
\end{align*}
\item The edge $((n-1,j), (n,j))$ is mapped to the vertical path given by:
\begin{align*}
	(2n-2,&~2n+j-2)  \rightarrow (2n-1, 2n+j-2) \\
	& \rightarrow \ldots \rightarrow (2n+j-2,2n+j-2) \text{ for } j = 2,\ldots,n-1.
\end{align*}
\item The edge $((2,j), (1,j))$ is mapped to the $L$-shaped path:
\begin{align*}
	(n+1,2n+&j-2)  \rightarrow (n, 2n+j-2) \rightarrow \ldots \rightarrow (n-j+1,2n+j-2) \\
	&  \rightarrow (n-j+1,2n+j-3)  \rightarrow \ldots \rightarrow (n-j+1,n-j+1) \\
	& \text{ for } j = 2,\ldots,n-1.
\end{align*}

\item The edge $((i,n-1), (i,n))$ is mapped to the $L$-shaped path:
\begin{align*}
	(n+i-1,3n&-3)  \rightarrow (n+i-1, 3n-2) \rightarrow \ldots \rightarrow (n+i-1,4n-i-2) \\
	&  \rightarrow (n+i,4n-i-2)  \rightarrow \ldots \rightarrow (4n-i-2,4n-i-2) \\
	& \text{ for } i = 2,\ldots,n-1.
\end{align*}
\end{enumerate} 
By construction, it follows that the paths in our edge embedding are vertex disjoint.
\end{proof}

%\vspace{-0.3cm}
\subsubsection{Reducing Half-Grids and Bringing the Piece Together}
We now review the construction of Gitler~\cite{Gitler91}, which shows how to reduce half-grids to much smaller half-grids (excluding diagonal edges) whose size depends only on $k$. For the sake of completeness, we provide a full proof here. Recall that $\hat{T}^{n}_{k}$ is the graph $T^{n}_k$ without the diagonal edges. 

\begin{lemma}[\cite{Gitler91}] \label{lemm: Gitler}
For any positive $k,n$ with $k<n$, $T^{n}_k$ is Wye-Delta reducible to $\hat{T}^{k}_{k}$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: Gitler}]
	For sake of simplicity, we assume w.l.o.g that the four vertices $(1,1)$, $(2,2)$, $(n-1,n-1)$ and $(n,n)$ are terminals\footnote{If they are not terminals, we can simply define them as terminals, thus increasing the number of terminals to $k+4 = O(k)$.}. Furthermore, we say that two terminals $(i,i)$ and $(j,j)$ are \textit{adjacent} iff $i<j$ and there is no terminal $(\ww,\ww)$ such that $i < \ww < j$. 
	
	We next describe the reduction procedure. Also see Fig.~\ref{fig: HalfGridRed} for an example. The reduction procedure starts by removing the diagonal edges of $T^{n}_k$, thus producing the graph $\hat{T}^{n}_k$ . Specifically, the two edges $((1,1),(2,2))$ and $((n-1,n-1), (n,n))$ are removed using an edge deletion operation. For each remaining diagonal edge of the form $((i,i), (i+1,i+1))$, $i=2,\ldots,n-2$ we repeatedly apply an edge replacement operation until the edge is incident to a boundary vertex $(1,j)$ or $(j,n)$ of the grid, where an edge deletion operation with one of the neighbours of $(1,j)$ resp. $(j,n)$ as vertex $x$ is applied.
	
	Now, we know that all non-terminals of the form $(i,i)$ are degree-two vertices, thus a series reduction is applied on each of them. This produces new diagonal edges, which are effectively reduced by the above procedure. We keep removing the newly-created degree-two non-terminal vertices and the newly-created edges until no further removals are possible. At this point, the only degree-$2$ vertices are terminal vertices. 
	%we arrive at a degree-four non-terminal $(i,j)$, for which the vertex $(i,i)$ on the same row and $(j,j)$ on the same column are terminals. 
	
	%The above vertex and edge removals could also produce degree-two vertices on the boundary of the half-grid, i.e., vertices of the form $(1,j)$ or $(i,n)$, excluding $(1,n)$. We apply a series reduction on every non-terminal of such form. 
	The resulting graph has a staircase structure, where for every pair of adjacent terminals $(i,i)$ and $(j,j)$, there is a non-terminal $(i,j)$ of degree three or four, namely, the intersection vertex, and a (possibly empty) sequence of degree-three non-terminals that lie on the boundary path from $(i,i)$ to $(j,j)$. For $k = i+1,\ldots,j-1$, let $(i,k)$ and $(k,j)$ be the degree-three non-terminals lying on the row and the column subpath, respectively. Additionally, for $k = i+1,\ldots,j-1$, let $C^{i}_{k}=\{(i',k) : i'=i,\ldots,1\}$, resp. $R^{j}_{k}=\{(k,j') : j'=j,\ldots,n\}$ be the vertices sharing the same column, resp. row with $(i,k)$, resp. $(k,j)$. We next show that the vertices belonging to $C^{i}_{k}$ and $R^{j}_{k}$ can be removed. 
	
	The removal process works as follows. For $k=i+1,\ldots,j-1$, we start by choosing a degree $3$ vertex $(i,k)$ and its corresponding column $C^{i}_{k}$. Then we apply a Wye-Delta transformation on $(i,k)$, thus creating two new diagonal edges. Similarly as above, we remove such edges by repeatedly applying an edge replacement operation until they have been pushed to the boundary of the grid, where an edge deletion operation is applied. In the resulting graph, the vertex $(i-1,k) \in C^{i}_{k}$ is now a degree-three non-terminal. We apply the same procedure to this vertex. Applying such a procedure to all remaining vertices of $C^{i}_{k}$, we eliminate a column of the grid. Symmetrically, the same process applies to the case when we want to remove the row $R^{j}_{k}$ corresponding to the vertex $(k,j)$.
	
	Applying the above removal process for every adjacent terminal pair and the corresponding degree-three non-terminals, we end up with the graph $\hat{T}^{k}_{k}$, where every diagonal vertex is a terminal. By definition, it follows that $\hat{T}^{k}_{k}$ has at most $O(k^2)$ vertices.
\end{proof}

Combining the above reductions leads to the following theorem:
\begin{theorem} \label{thm: CutSparsifier}
Let $G$ be a $k$-terminal planar graph where all terminals lie on the outer face. Then $G$ admits a quality-$1$ cut sparsifier of size $O(k^{2})$, which is also a planar graph.
\end{theorem}
\begin{proof}
Let $n$ denote the number of vertices in $G$. First, we apply Lemma \ref{lemm: embeddingGrids} on $G$ to obtain a grid graph $H$ with $O(n^{2})$ vertices, which preserves exactly all terminal minimum cuts of $G$. We then apply Lemma \ref{lemm: embeddingHalfGrid} on $H$ to obtain a node embedding $\rho$ into the half-grid $T^{\ww}_{k}$, where $\ww = 4n-3$. By Lemma \ref{lemm: cutembedding}, $\rho(H)$ preserves exactly all terminal minimum cuts of $H$. We can further extend $\rho(H)$ to the full half-grid $T^{\ww}_{k}$, if dummy non-terminals and zero edge capacities are added. Finally, we apply Lemma \ref{lemm: Gitler} on $T^{\ww}_{k}$ to obtain a Wye-Delta reduction to the reduced half-grid graph $\hat{T}^{k}_{k}$. It follows by Lemma \ref{lemm: cutReducability} that $\hat{T}^{k}_{k}$ is a quality-$1$ cut sparsifier of $T^{\ww}_{k}$, where the size guarantee is immediate from the definition of $\hat{T}^{k}_{k}$.
\end{proof}

%Due to space constraints, the details are referred to Appendix~\ref{sec: UpperFlow} and~\ref{sec: UpperDist}, respectively.
\section{Extensions to Planar Flow and Distance Sparsifiers} \label{sec: UpperFlow}
In this section we show how to extend our result for cut sparsifiers to flow and distance sparsifiers. 
\subsection{An Upper Bound for Flow Sparsifiers}
We first review the notion of Flow Sparsifiers. Let $d$ be a demand function over terminal pairs in $G$ such that $d(x,x')=d(x',x)$ and $d(x,x)=0$ for all $x,x' \in K$. We denote by $P_{xx'}$ the set of all paths between vertices $x$ and $x'$, for all $x,x' \in K$. Further, let $P_{e}$ be the set of all paths using edge $e$, for all $e \in E$ . A \emph{concurrent} (\textit{multi-commodity}) flow $f$ of \emph{throughput} $\lambda$ is a function over terminal paths in $G$ such that (1) $\sum_{p \in P_{xx'}} f(p) \geq \lambda d(x,x')$, for all distinct terminal pairs $x,x' \in K$ and (2) $\sum_{p \in P_e} f(p) \leq \cc(e)$, for all $e \in E$. We let $\lambda_G(d)$ denote the \emph{throughput of the concurrent flow} in $G$ that attains the largest throughput and we call a flow achieving this throughput the \emph{maximum concurrent flow}. A graph $H = (V_H, E_H, c_H)$, $K \subset V_H$ is a \emph{quality-$1$} (\emph{vertex}) \emph{flow sparsifier} of $G$ with $q \geq 1$ if for every demand function
$d$, $\lambda_G(d) \leq \lambda_H(d) \leq q \cdot \lambda_H(d).$

Next we show that given a $k$-terminal planar graph, where all terminals lie on the outer face, one can construct a quality-$1$ flow sparsifier of size $O(k^{2})$. Our result follows from combining the observation of Andoni et al.~\cite{andoni} for constructing flow-sparsifiers using flow/cut gaps and the flow/cut gap result of Okamura and Seymour~\cite{OkamuraS81}.

Given a $k$-terminal graph and a demand function $d$, recall that $\lambda_G(d)$ is the maximum fraction of $d$ that can be routed in $G$. We define the \emph{sparsity} of a cut $(U, V \setminus U)$ to be
\[
\Phi_G(U,d) := \frac{\capacity(\delta(U))}{\sum_{i,j: |\{i,j\} \cap U|=1}d_{ij}}
\]
and the \emph{sparsest cut} as $\Phi_G(d) := \min_{U \subset V} \Phi_G(U,d)$. Then the \emph{flow-cut} gap is given by
\[
\gamma(G) := \max \{\Phi_G(d) / \lambda_G(d) : d \in \mathbb{R}^{\binom{k}{2}}_{+}\}.
\]
%In what follows it will be convenient to generalize the notion of a $k$-terminal graph. Given a $k$-terminal graph $G=(V,E,c)$ with $K \subset V$, we define the \emph{demand-support} to be the graph $H=(K,F)$, where $F \subseteq K \times K$. Note that this generalizes the case when $H$ is the complete graph on the terminals $K$. We can now define the flow-cut gap according to the pair $(G,H)$:
%\[
%	\gamma(G,H) := \max \{\Phi_G(d)/\lambda_G(d) : d \in \mathbb{R}^{|E(H)|}_{+}\}.
%\]

We will make use of the following theorem:
\begin{theorem}[\cite{andoni}] \label{thm: FlowCutGap}
	Given a $k$-terminal graph $G$ with terminals $K$, let $G'$ be a quality-$\beta$ cut sparsifier for $G$ with $\beta \geq 1$. Then for every demand function $d \in \mathbb{R}^{\binom{k}{2}}_{+}$,
	\[
	\frac{1}{\gamma(G')} \leq \frac{\lambda_{G'}(d)}{\lambda_G(d)} \leq \beta \cdot \gamma(G).
	\]
	Therefore, the graph $G'$ with edge capacities scaled up by $\gamma(G')$ is a quality-$\beta \cdot \gamma(G) \cdot \gamma(G')$ flow sparsifier of size $|V(G')|$ for $G$.
\end{theorem}
This leads to the following corollary.
\begin{corollary} \label{cor: FlowSparsifiers}
	Let $G$ be a $k$-terminal planar graph where all terminals lie on the outer face. Then $G$ admits a quality-$1$ flow sparsifier of size $O(k^{2})$.
\end{corollary}
\begin{proof}
	Given a $k$-terminal planar graph where all terminals lie on the outer face, Theorem \ref{thm: CutSparsifier} shows how to construct a cut sparsifier $G'$ with quality $\beta = 1$ and size $O(k^2)$, which is also a planar graph with all the $k$ terminals lying on the outer face. Okamura and Seymour~\cite{OkamuraS81} showed that for every $k$-terminal planar graph $G$ with terminals lying on the outer face the flow-cut gap is $1$. This implies that $\gamma(G) = 1$ and $\gamma(G') = 1$. Invoking Theorem \ref{thm: FlowCutGap} we get that $G'$ is a quality-$1$ flow sparsifier of size $O(k^2)$ for $G$.
	%Okamura and Seymour~\cite{OkamuraS81} show that the flow-cut gap for a $k$-terminal planar graph $G$ when all terminal{sec: UpperDist}s lie on the outer face is $\gamma(G,H) = 1$, and Theorem \ref{thm: CutSparsifier} gives that for such $G$, one can obtain another planar graph $G'$ with quality $\beta = 1$ and size $O(k^{2})$. Since $G'$ is a planar graph with all terminals on the outer face, it follows that $\gamma(G',H)=1$, which proves what we were after. 
\end{proof}


\subsection{An Upper Bound for Distance Sparsifiers} \label{sec: UpperDist}
We first review the notion of Vertex Distance Sparsifiers. Let $G=(V,E,\ww)$ with $K \subset V$ be a $k$-terminal graph, where we replace the capacity function $\cc$ with a weight or length function $\ww : E \rightarrow \mathbb{R}_{\geq 0}$. For a terminal pair $(x,x') \in K$, let $\dist_G(x,x')$ denote the shortest path with respect to the edge lengths $\ww$ in $G$. A graph $H=(V',E',\ww')$ is a \emph{quality-$q$} (\emph{vertex}) \emph{distance sparsifier} of $G$ with $q \geq 1$ if for any $x,x' \in K$, $\dist_G(x,x') \leq \dist_H(x,x') \leq q \cdot \dist_G(x,x')$.

Next we argue that a symmetric approach applies to the construction of vertex sparsifiers that preserve distances. Concretely, we prove that given a $k$-terminal planar graph, where all terminals lie on the outer face, one can construct a quality-$1$ distance sparsifier of size $O(k^{2})$, which is also a planar graph. It is not hard to see that almost all arguments that we used about cut sparsifiers go through, except some adaptations regarding edge lengths in the Wye-Delta rules, edge subdivision operation and vertex splitting operation.

We start adapting the Wye-Delta operations. 

\begin{enumerate}
	\setlength\itemsep{0.1em}
	\item \emph{Degree-one reduction:} Delete a degree-one non-terminal and its incident edge.
	\item \emph{Series reduction:} Delete a degree-two non-terminal $y$ and its incident edges $(x,y)$ and $(y,z)$, and add a new edge $(x,z)$ of length $\ww(x,y) + \ww(y,z)$.
	\item \emph{Parallel reduction:} Replace all parallel edges by a single edge whose length is the minimum over all lengths of parallel edges.
	\item \emph{Wye-Delta transformation:} Let $x$ be a degree-three non-terminal with neighbours $\delta(x) = \{u,v,w\}$. %Assume w.l.o.g.\footnote{Suppose there exist a pair $(u,v) \in \delta(x)$ with $\cc(u,x) + \cc(v,x) < \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. Then we can simply set $\cc(w,x) = \cc(u,x) + \cc(v,x)$, since any terminal minimum cut would cut the edges $(u,x)$ and $(v,x)$ instead of the edge $(w,x)$.} that for any pair $(u,v) \in \delta(x)$, $\cc(u,x) + \cc(v,x) \geq \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. 
	Delete $x$ (along with all its incident edges) and add edges $(u,v),(v,w)$ and $(w,u)$ with lengths $\ww(u,x) + \ww(v,x)$, $\ww(v,x) + \ww(w,x)$ and $\ww(w,x) + \ww(u,x)$, respectively. 
	\item \emph{Delta-Wye transformation:} Let $x$, $y$ and $z$ be the vertices of the triangle connecting them. Assume w.l.o.g.\footnote{Suppose there exists a triangle edge $(x,y)$ with $\ww(x,y) > \ww(x,z) + \ww(y,z)$, where $z$ is the other triangle vertex. Then we can simply set $\ww(x,y) = \ww(x,z) + \ww(y,z)$, since any shortest path between terminal pairs would use the edges $(x,z)$ and $(y,z)$ instead of the edge $(x,y)$.} that for any triangle edge $(x,y)$, $\ww(x,y) \leq \ww(x,z) + \ww(y,z)$, where $z$ is the other triangle vertex. Delete the edges of the triangle, introduce a new vertex $w$ and add new edges $(w,x)$, $(w,y)$ and $(w,z)$ with edge lengths $(\ww(x,y) + \ww(x,z) - \ww(y,z))/2,$ $(\ww(x,z) + \ww(y,z) - \ww(x,u))/2$ and $(\ww(x,y) + \ww(y,z) - \ww(x,z))/2$, respectively.
\end{enumerate}
The following lemma shows that the above rules preserve exactly all shortest path distances between terminal pairs. 

\begin{lemma} Let $G$ be a $k$-terminal graph and $G'$ be a $k$-terminal graph obtained from $G$ by applying one of the rules 1-5. Then $G'$ is a quality-$1$ distance sparsifier of $G$.
\end{lemma}
We remark that there is no need to re-define the Edge deletion and replacement operations, since they are just a combination of the above rules. An analogue of Lemma \ref{lemm: cutReducability} can also be shown for distances. We now modify the Edge subdivision operation, which is used when dealing with graph embeddings (see Section \ref{sec: graphEmbeddings}).
\begin{enumerate}
	\item \emph{Edge subdivision}: Let $(u,v)$ be an edge of length $\ww(u,v)$. Delete $(u,v)$, introduce a new vertex $w$ and add edges $(u,w)$ and $(w,v)$, each of length $\ww(u,v)/2$. 
\end{enumerate}

%Let $G_1$ be a $k$-terminal graph and $\rho(G_1)$ be another $k$-terminal network obtained by some node embedding $\rho$. 
We now prove an analogue to Lemma \ref{lemm: cutembedding}.

\begin{lemma} \label{lemm: DistancePreservation}
	Let $\rho$ be a node embedding and let $G_1$ and $\rho(G_1)$ be $k$-terminal graphs as defined in Section~\ref{sec: graphEmbeddings}. Then $\rho(G_1)$ preserves exactly all shortest path distances between terminal pairs.
\end{lemma}
\begin{proof}
	We can view each path obtained from the embedding as taking the edge corresponding to that path endpoints in $G_1$ and performing edge subdivisions finitely many times. We claim that such subdivisions preserve all terminal shortest paths.
	
	Indeed, let us consider a single edge subdivison for $(u,v)$ (the general claim then follows by induction on the number of edge subdivions). Fix $x,x' \in K$ and consider some shortest path $p(x,x')$ in $G_1$ that uses $(u,v)$. We can construct in $\rho(G_1)$ a path $q(x,x')$ of the same length as follows: traverse the subpath $p(x,u)$, traverse the edges $(u,w)$ and $(w,v)$ and finally traverse the subpath $p(v,x')$. It follows that $\sum_{e \in p(x,x')} \ww(e) = \sum_{e \in q(x,x')} \ww(e)$, and thus $\dist_{\rho(G_1)}(s,t) \leq \dist_{G_1}(s,t)$.
	
	On the other hand, fix $x,x' \in K$ and consider some shortest path $p'(x,x')$ in $\rho(G_1)$ that uses the two subdivided edges $(u,w)$ and $(w,v)$ (note that it cannot use only one of them). We can construct in $G_1$ a path $q'(x,x')$ of the same length as follows: traverse the subpath $p'(x,u)$, traverse the edge $(u,v)$ and finally traverse the subpath $p'(v,x')$. It follows that $\sum_{e \in p'(x,x')} \ww(e) = \sum_{e \in q'(x,x')} \ww(e)$ and thus $\dist_{G_1}(s,t) \leq \dist_{\rho(G_1)}(s,t)$. Combining the above gives the lemma.
\end{proof}

We next consider vertex splitting for graphs whose maximum degree is larger than three. For each vertex $v$ of degree $d > 3$ with $u_1,\ldots,u_d$ adjacent to $v$, we delete $v$ and introduce new vertices $v_1, \ldots, v_d$ along with edges $\{(v_i,v_{i+1}) : i = 1,\ldots,d-1\}$, each of length $0$. Furthermore, we replace the edges $\{(u_i,v) : i=1,\ldots,d\}$ with $\{(u_i,v_i) : i = 1,\ldots, d\}$, each of corresponding length. If $v$ is a terminal vertex, we make one of the $v_i$'s be a terminal vertex. An analogue to Claim \ref{claim: embedding} gives that the resulting graph preserves all terminal shortest path distances.

We finally note that whenever we add dummy edges of capacity $0$ in the cut setting, we replace them by edges of length $D+1$ in the distance setting, where $D$ is the sum over all edge lengths in the graph we consider. Since any shortest path in the graph does not use the added edges, the terminal shortest path remain unaffected. The above discussion leads to the following theorem. 

\begin{theorem} \label{thm: DistanceSparsifier}
	Let $G$ be a $k$-terminal planar graph where all terminals lie on the outer face. Then $G$ admits a quality-$1$ distance sparsifier of size $O(k^{2})$, which is also a planar graph. 
\end{theorem}

\input{chapters/reachabilityminors/lower-bound-2}













==> chapters/reachabilityminors/introduction.tex <==
\section{Introduction}

Very large graphs or networks are ubiquitous nowadays, from social networks to information networks. One natural and effective way of processing and analyzing such graphs is to compress or sparsify the graph into a smaller one that well preserves certain properties of the original graph. Such a sparsification can be obtained by reducing the number of \emph{edges}. Typical examples include cut sparsifiers~\cite{BenczurK96}, spectral sparsifiers~\cite{SpielmanT11}, spanners~\cite{ThorupZ05} and transitive reductions~\cite{AhoGU72}, which are subgraphs defined on the same vertex set of the original graph $G$ while having much smaller number of edges and still well preserving the cut structure, spectral properties, pairwise distances and transitive closure of $G$, respectively. 

Another way of performing sparsification is by reducing the number of \emph{vertices}, which is most appealing when only the properties among a subset of vertices (which are called \emph{terminals}) are of interest~(see e.g., \cite{Moitra09,andoni,KrauthgamerNZ14}). We call such small graphs \emph{vertex sparsifiers} of the original graph. In this paper, we will particularly focus on vertex reachability sparsifiers for \emph{directed} graphs and cut (and other related) sparsifiers for \emph{undirected} graphs. 

Vertex reachability sparsifiers in directed graphs is an important and fundamental notion in Graph Sparsification, which has been implicitly studied in the dynamic graph algorithms community~\cite{Subramanian93,DiksS07}, and explicitly in~\cite{katriel2005reachability}. Specifically, given a digraph $G=(V,E)$, $K \subset V$, a digraph $H=(V',E')$, $K \subset V'$ is a (\emph{vertex}) \emph{reachability sparsifier} of $G$ if for any $x ,x' \in K$, there is a directed path from $x$ to $x'$ in $H$ iff there is a directed path from $x$ to $x'$ in $G$. If $|K|=k$, we call the digraph $G$ a \emph{$k$-terminal digraph}. Note that any $k$-terminal digraph $G$ always admits a trivial reachability vertex sparsifier $H$, which corresponds to the transitive closure restricted to the terminals. 

In this chapter, we initiate the study of \emph{reachability-preserving minors}, i.e., vertex reachability sparsifiers with $H$ required to be a minor of $G$. %Krauthgamer et al.~\cite{KrauthgamerNZ14} also consider a similar notion for distances in undirected graphs. 
The restriction on $H$ being a minor of $G$ is desirable as it makes sure that $H$ is structurally similar to $G$, e.g., any minor of a planar graph remains planar. We ask the question whether general graphs admit reachability-preserving minors whose size can be bounded independently of the input graph $G$, and study it from both the lower- and upper-bound perspective.


For the notion of cut (and other related) sparsifiers, we are given a capacitated undirected graph $G=(V,E,\cc)$, and a set of terminals $K$ and our goal is to find a (capacitated undirected) graph $H=(V',E',\cc')$ with as few vertices as possible and $K \subseteq V'$ such that the quantities like, cut value, multi-commodity flow and distance among terminal vertices in $H$ are the same as or close to the corresponding quantities in $G$. If $|K|=k$, we call the graph $G$ a \emph{$k$-terminal graph}. 

We say $H$ is a \emph{quality-$q$} (\emph{vertex}) \emph{cut sparsifier} of $G$, if for every bipartition $(U,K \setminus U)$ of the terminal set $K$, the value of the minimum cut separating $U$ from $K \setminus U$ in $G$ is within a factor of $q$ of the value of minimum cut separating $U$ from $K \setminus U$ in $H$. If $H$ is a quality-$1$ cut sparsifier, then it will be also called a \emph{mimicking network}~\cite{HagerupKNR98}. Similarly, we define flow and distance sparsifiers that (approximately) preserve multicommodity flows and distances among terminal pairs, respectively~(see Section~\ref{sec: UpperFlow} for formal definitions). These type of sparsifiers have proven useful in approximation algorithms~\cite{Moitra09} and also find applications in network routing~\cite{Chuzhoy12a}.

\paragraph*{Our Results.} Our first and main contribution is the study \sloppy of reachability-preserving minors. Although reachability is a weaker requirement in comparison to shortest path distances, directed graphs are usually much more cumbersome to deal with from the perspective of graph sparsification. Surprisingly, we show that general digraphs admit reachability-preserving minors with $O(k^{3})$ vertices, which is in contrast to the bound of $O(k^4)$ on the size of distance-preserving minors in undirected graphs by Krauthgamer et al.~\cite{KrauthgamerNZ14}. 

\begin{theorem} \label{thmi: general_reachability} Given a $k$-terminal digraph $G$, there exist a reachability-preserving minor $H$ of $G$ with size $O(k^{3})$.
\end{theorem}

It might be interesting to compare the above result with the construction of \emph{reachability preserver} by Abbound and Bodwin~\cite{AB18reachability}, where the reachability preserver for a pair-set $P$ in a graph $G$ is defined to be a \emph{subgraph} of $G$ that preserves the reachability of all pairs in $P$. The size (i.e., the number of edges) of such preservers is shown to be at least $\Omega(n^{2/(d+1)}|P|^{(d-1)/d})$, for any integer $d\geq 2$, which is in sharp contrast to our upper bound $O(|P|^{3/2})$ on the size of reachability-preserving minors by taking $P$ to be the pair-set of all terminals. 

Furthermore, by exploiting a tight integration of our techniques with the compact distance oracles for planar graphs by Thorup~\cite{ThorupJACM04}, we can show the following theorem regarding the size of reachability-preserving minors for planar digraphs. 

\begin{theorem} \label{thm: ubPlanar}
	Given a $k$-terminal planar digraph $G$, there exists a reachability-preserving minor $H$ of $G$ with size $O(k^{2} \log k)$.
\end{theorem}

We complement the above result by showing that there exist instances where the above upper-bound is tight up to a $O(\log k)$ factor. %The proof is deferred to Appendix~\ref{app: minorLB}.

%This is of particular interest, since for distance-preserving minors, even for planar graphs, the gap between the best-known upper and lower-bound is $\Omega(k^2)$.

\begin{theorem} \label{thm: lbPlanar}
	For infinitely many $k \in \mathbb{N}$ there exists a $k$-terminal acyclic directed grid $G$ such that any reachability-preserving minor of $G$ must use $\Omega(k^{2})$ non-terminals.
\end{theorem}

%\subsubsection{Cut, Flow and Distance Sparsifiers}
%\paragraph*{Cut, Flow and Distance Sparsifiers.}
Our second contribution is new algorithms for constructing quality-$1$ (exact) cut, flow and distance sparsifiers for $k$-terminal planar graphs, where all the terminals are assumed to lie on the same face. We call such $k$-terminal planar graphs \emph{Okamura-Seymour} (OS) instances. They are of particular interest in the algorithm design and optimization community, due to the classical Okamura-Seymour theorem that characterizes the existence of feasible concurrent flows in such graphs~(see e.g., \cite{OkamuraS81,chekuri09,chekuri2010flow,LeeMM13}).

We show that the size of quality-$1$ sparsifiers can be as small as $O(k^2)$ for such instances, for which only exponential (in $k$) size of cut and flow sparisifiers were known before~\cite{KrauthgamerR13,andoni}. Formally, we have the following theorem.
\begin{theorem} \label{thm: mainThm}
	For any \emph{OS} instance $G$, i.e., a $k$-terminal planar graph in which all terminals lie on the same face, there exist quality-$1$ cut, flow and distance sparsifers of size $O(k^2)$. Furthermore, the resulting sparsifiers are also planar.
\end{theorem} 

We remark that all the above sparsifiers can be constructed in polynomial time (in $n$ and $k$), but we will not optimize the running time here. As we mentioned above, previously the only known upper bound on the size of quality-$1$ cut and flow sparsifiers for OS instance was $O(k^22^{2k})$, given by~\cite{KrauthgamerR13,andoni}. Our upper bound for cut sparsifier also matches the lower bound of $\Omega(k^2)$ for OS instance given by~\cite{KrauthgamerR13}. More specifically, in \cite{KrauthgamerR13}, an OS instance (that is a grid in which all terminals lie on the boundary) is constructed, and used to show that any mimicking network for this instance needs $\Omega(k^2)$ edges, which is thus a lower bound for planar graphs (see the table below for an overview). Note that that even though our distance sparsifier is not necessarily a minor of the original graph $G$, it still shares the nice property of being planar as $G$. Furthermore, Krauthgamer and Zondiner~\cite{KrauthgamerZ12} proved that there exists a $k$-terminal planar graph $G$ (not necessarily an OS instance), such that any quality-$1$ distance sparsifier of $G$ that is planar requires at least $\Omega(k^2)$ vertices. 

\begin{table}[h]
\renewcommand{\arraystretch}{1.1}
\begin{center}
\begin{tabular}{c|c|c|c}
Graph & Type of sparsifier &  Upper Bound &  Lower Bound  \\ \hline \hline
%Cut & General & $O(2^{2^k})$~\cite{HagerupKNR98} & $2^{\Omega(k)}$~\cite{KrauthgamerR13,KhanR14}  \\ \hline
Planar & Cut (minor) & $O(k2^{2k})$~\cite{KrauthgamerR13} & $\Omega(k^{2})$~\cite{KrauthgamerR13} \\
Planar ($\gamma$) & Cut (minor) & $O(\gamma^5 2^{2 \gamma} k^4)$~\cite{krauthgamer2017refined} & $\Omega(2^{k})$~\cite{karpov2017exponential} \\
Planar OS & Cut (planar) & $\mathbf{O(k^2})$ & $\Omega(k^{2})$~\cite{KrauthgamerR13} \\ \hline 
Planar OS & Distance (minor) & $O(k^{4})$~\cite{KrauthgamerNZ14} & $\Omega(k^2)$~\cite{KrauthgamerNZ14}   \\
Planar OS &  Distnace (planar) & $\mathbf{O(k^{2})}$ & $\Omega(k^2)$~\cite{KrauthgamerZ12} 
\end{tabular}
\caption{An overview on the best-known results for mimicking networks and distance sparsifiers. The results which are \emph{not} followed by a reference are shown in this chapter.}
\end{center}
\end{table}
We further provide a lower bound on the size of any \emph{data structure} (not necessarily a graph) that approximately preserves pairwise terminal distances of \emph{general} $k$-terminal graphs, which gives a trade-off between the distance stretch and the space complexity. %The proof is deferred to Appendix \ref{sec: lowerBound}.
 
\begin{theorem}~\label{thm:incompressibility}
For any $\varepsilon > 0$ and $t \geq 2$, there exists a (sparse) $k$-terminal $n$-vertex graph such that $k=o(n)$, and any data structure that approximates pairwise terminal distances within a multiplicative factor of $t - \varepsilon$ or an additive error $2t-3$ must use $\Omega(k^{1+1/(t-1)})$ bits. 
\end{theorem}
%Therefore, our lower bound is  tight up to a factor of $2$ on the approximation ratio and a polylogarithmic factor on the space complexity due to word encoding. On the other hand, one can also modify the current lower bound $\Omega(k^{1+\frac{1}{t-\lfloor(t+2)/4\rfloor+1}})$ of the number of edges of any $(t+3)$-spanner to get a lower bound ...%It is also worth mentioning that a lower bound of $\Omega(n^{1+1/t})$ on the number of edges of any $(2t-1)$-multiplicative spanner for $n$-vertex graphs holds only under the popular Girth Conjecture of Erd{\"o}s~\cite{Erdos64}, while our lower bound is unconditional. In addition, Woodruff has also gave an unconditional lower bound $\Omega(n^{1+1/t})$ for spanners of an $n$-vertex graph with additive error $2t-1$. It is not clear if these lower bounds for spanners imply the same or similar lower bounds for the size of distance sparsifiers.

\paragraph*{Remark.} Recently and independently of our work, Krauthgamer and Rika~\cite{krauthgamer2017refined} constructed quality-$1$ cut sparsifiers of size $O(\gamma^{5}2^{2\gamma}k^4)$ for planar graphs whose terminals are incident to at most $\gamma=\gamma(G)$ faces. In comparison with our upper-bound which only considers the case $\gamma = 1$, the size of our sparsifiers from Theorem~\ref{thm: mainThm} is better by a $\Omega(k^{2})$ factor. Moreover, their work focuses on constructing sparsifiers that are minors of the originial input graph, while our construction only guarantee that the resulting sparsifiers are planar graphs. Subsequent to our work, Karpov et al.~\cite{karpov2017exponential} proved that there exists edge-weighted $k$-terminal planar graphs that require $\Omega(2^k)$ edges in any exact cut sparsifier, which implies that it is necessary to have some additional assumption (e.g., $\gamma=O(1)$) to obtain a cut sparsifier of $k^{O(1)}$ size. 

%\label{subsec:techniques}
\paragraph*{Our Techniques.} Our results for reachability-preserving minors are obtained by exploiting a technique of counting ``branching'' events between shortest paths in the directed setting (this technique was introduced by Coppersmith and Elkin~\cite{CoppersmithE06}, and has also been recently leveraged by Bodwin~\cite{Bodwin17} and Abboud and Bodwin~\cite{AB18reachability}). Using this and a consistent tie-breaking scheme for shortest paths, we can efficiently construct a RPM for general digraphs of size $O(k^4)$ and by using a more refined analysis of branching events (see \cite{AB18reachability}), we can further reduce the size to be $O(k^3)$. We then combine our construction with a decomposition for planar digraphs (see~\cite{ThorupJACM04}), to show that it suffices to maintain the reachability information among $O(k\log k)$ terminal pairs, instead of the naive $O(k^2)$ pairs, and then construct a RPM for planar digraphs with $O(k^2\log k)$ vertices. 

The lower-bound follows by constructing a special class of $k$-terminal directed grids and showing that any RPM for such grids must use $\Omega(k^2)$ vertices. Similar ideas for proving the lower bound on the size of distance-preserving minors for undirected graphs have been used by Krauthgamer et al.~\cite{KrauthgamerNZ14}.

We construct our quality-$1$ cut and distance sparsifiers by repeatedly performing \emph{Wye-Delta transformations}, which are local operations that preserve cut values and distances and have proven very powerful in analyzing electrical networks and in the theory of circular planar graphs~(see e.g., \cite{curtis98,feo1993}). Khan and Raghavendra~\cite{KhanR14} used Wye-Delta transformations to construct quality-$1$ cut sparsifiers of size $O(k)$ for trees and outerplanar graphs, while our case (i.e., the planar OS instances) is more general and complicated and previously it was not clear at all how to apply such transformations to a more broad class of graphs. Our approach is as follows. Given a $k$-terminal planar graph with terminals lying on the same face, we first embed it into some large grid with terminals lying on the boundary of the grid. Next, we show how to embed this grid into a ``more suitable'' graph, which we will refer to as ``half-grid''. Finally, using the Wye-Delta operations, we reduce the ``half-grid'' into another graph whose number of vertices can be bounded by $O(k^{2})$. Since we  argue that the above graph reductions preserve exactly all terminal minimum cuts, our result follows. Gitler~\cite{Gitler91} proposed a similar approach for studying the reducibility of multi-terminal graphs with the goal to classify all Wye-Delta reducible graphs, which is very different from our motivation of constructing small vertex sparsifiers with good quality. 

The distance sparsifiers can be constructed similarly by slightly modifying the Wye-Delta operation. Our flow sparsifiers follow from the construction of cut sparsifiers and the flow/cut gaps for OS instances (which has been initially observed by Andoni et al.~\cite{andoni}). Our lower bound on the space complexity of any compression function approximately preserving terminal pairwise distance is derived by combining extremal combinatorics construction of Steiner Triple System that was used to prove lower bounds on the size of distance approximating minors (see~\cite{cheung2016}) and the incompressibility technique from~\cite{matousek96}.

\medskip
\noindent \textbf{Related Work. } There has been a long line of work on investigating the tradeoff between the quality of the vertex sparsifier and its size~(see e.g., \cite{EnglertGKRTT14,KrauthgamerR13,andoni}). (Throughout, cut, flow and distance sparsifiers will refer to their vertex versions.) Quality-$1$ \emph{cut sparsifiers} (or equivalently, mimicking networks) were first introduced by Hagerup et al.~\cite{HagerupKNR98}, who proved that for any graph $G$, there always exists a mimicking network of size $O(2^{2^k})$. %Chaudhuri et al.~\cite{chaudhuri00} then constructed mimicking networks with $O(k)$ vertices for bounded treewidth graphs and outerplanar graphs, and they also give a lower bound of $k+1$ for the size of such networks, that even holds for a star graph~\cite{chaudhuri00}. 
Krauthgamer and Rika~\cite{KrauthgamerR13} showed how to build a mimicking network of size $O(k^22^{2k})$ for any planar graph $G$ that is minor of the input graph. They also proved a lower bound of $\Omega(k^2)$ on the number of edges of the mimicking network of planar graphs, and a lower bound of $2^{\Omega(k)}$ on the number of vertices of the mimicking network for general graphs. %Khan and Raghavendra~\cite{KhanR14} gave an improved upper bound (while still doubly exponential in $k$) for general graphs as well as a lower bound of $2^{(k-1)/2}$ for general graphs. They also give improved upper bounds (while still $O(k)$) for trees and graphs with bounded treewidth. 


Quality-$1$ vertex flow sparsifiers have been studied in~\cite{andoni, GoranciR16}, albeit only for restricted families of graphs like quasi-bipartite, series-parallel, etc. It is not known if any general undirected graph $G$ admits a constant quality flow sparsifier with size independent of $|V(G)|$ and the edge capacities. For the quality-$1$ distance sparsifiers, Krauthgamer et al.~\cite{KrauthgamerNZ14} introduced the notion of \emph{distance-preserving minors}, and showed an upper-bound of size $O(k^4)$ for general undirected graphs. They also gave a lower bound of $\Omega(k^2)$ on the size of such a minor for planar graphs. Abboud et al.~\cite{AbboudGMW17} show how to compress a planar graph metric using only $\tilde{O}(\min\{k^2,\sqrt{k \cdot n}\})$ bits. Recently,~ Chang et al.~\cite{ChangGMW18} extended their compressing scheme to a graph sparsifer which matches their bound.
%However, it is not clear whether their compression scheme can be represented by a graph on $k$ terminals which matches their bound. %The main reason of requiring the distance sparsifier $H$ being a ``minor'' of the original graph $G$ is to make sure that $H$ is structurally similar to $G$. Here we relax the requirement for planar graphs $G$ by only restricting the distance sparsifier $H$ to be planar (not necessarily a minor of $G$; see \cite{gupta01} for similar requirement for trees). 

Over the last two decades, there has been a considerable amount of work on understanding the tradeoff between the sparsifier's quality $q$ and its size for $q>1$, i.e., when the sparsifiers only \emph{approximately} preserve the corresponding properties~\cite{juliasteiner,andoni,Moitra09,leighton,charikar,EnglertGKRTT14,mm10,Gupta01,
chekuri2006embedding,ChanXKR06,KammaKN15,cheung2016,Cheung18,Filtser18,
GajjarR17,BernsteinDDKMS18}. 
%Chuzhoy~\cite{juliasteiner} gave constant quality cut and flow sparsifiers with size depending on the total capacity of the edges on the terminals. Andoni et al.~\cite{andoni} constructed quality $(1+\varepsilon)$ flow sparsifier of size $poly(k/\varepsilon)$ for quasi-bipartite networks and quality $O(\log t/\log\log t)$ flow sparsifier of size $O(t\cdot poly(k))$ for $G$ with bounded treewidth $t$. (They also constructed a \emph{sketch} (not a graph) of quality $1+\varepsilon$ and size $f(k,\varepsilon)$ (independent of $n$) for general graphs.)

%There are many other known tradeoffs between the sparsifier's quality $q$ and its size for $q>1$, i.e., when the sparsifiers only \emph{approximately} preserve the corresponding properties. Chuzhoy~\cite{juliasteiner} gave constant quality cut and flow sparsifiers with size depending on the total capacity of the edges on the terminals. Andoni et al.~\cite{andoni} constructed quality $(1+\varepsilon)$ flow sparsifier of size $poly(k/\varepsilon)$ for quasi-bipartite networks and quality $O(\log t/\log\log t)$ flow sparsifier of size $O(t\cdot poly(k))$ for $G$ with bounded treewidth $t$. (They also constructed a \emph{sketch} (not a graph) of quality $1+\varepsilon$ and size $f(k,\varepsilon)$ (independent of $n$) for general graphs.)
%
%For sparsifiers with exactly $k$ vertices (that is, supported only on the terminals), there are efficient algorithms for constructing quality $O(\log k/\log\log k)$ cut and flow sparsifiers~(\cite{moitra09,leighton,charikar,englert10,mm10}), and there exists a lower bound of $\tilde{\Omega}(\sqrt{\log k})$ on the quality of such cut or flow sparsifiers \cite{mm10} (see also~\cite{charikar,leighton,englert10}). %(improving previous $\Omega(\sqrt{\log k/\log \log k})$ \cite{mm10} $\Omega(\log^{1/4} k)$~\cite{charikar} by~\cite{leighton} and $\Omega(\log \log k)$ of a stronger vertex sparification by~\cite{leighton}) on the quality of flow sparsifiers. 
%
%%For flow sparsifiers,   For flow sparsfiers $H$ with only $k$ vertices (the terminals), Englert et al. \cite{englert10} have shown that for general graphs $G$, there exist such sparsifiers of quality $O(\log k/\log\log k)$. %; a convex combination of trees $O(\log k)$ on quality; for planar graphs, a convex combination of planar graphs $O(1)$ on quality [EGKRTT14].
%
%For vertex distance sparsifiers, there has been work on constructing \emph{minors} that approximately preserve the pairwise distances among terminals for both general graphs and planar graphs (see \cite{gupta01,chekuri2006embedding,chan06,englert10,kamma2015,cheung2016}).  

%For planar graphs, cut sparsification upper bound $O(2^{2k})$ and lower bound $\Omega(k^2)$. flow sparsification upper bound $O()$ and lower bound ?? (which follows from the lower bound for cut sparsifier?), (for the OS instance, upper bound $O(k^22^{2k})$, the lower bound ??). distance sparsification, upper bound $O(k^2)$ (even for general graphs), ``if the spasifier is required to be a minor (or similar to the original graph), then $O(k^4)$, and lower bound $\Omega(k^2)$''.

%that preserve all the values of minimum cut between every bipartition of terminals (called \emph{vertex cut sparsifiers}), all the multicommodity flows that can be routed between the terminals (called \emph{vertex flow sparsifiers}), and all the shortest-path distance between every pair of terminals (called \emph{vertex distance sparsifiers}).



==> chapters/reachabilityminors/lower-bound-2.tex <==
\subsection{Incompressibility of Distances in $k$-Terminal Graphs} \label{sec: lowerBound}

In this section we prove the following incompressibility result (i.e., Theorem~\ref{thm:incompressibility}) concerning the trade-off between quality and size of any compression function when estimating terminal distances in $k$-terminal graphs: for every $\varepsilon > 0$ and $t \geq 2$, there exists a (sparse) $k$-terminal $n$-vertex graph such that $k=o(n)$, and that any compression algorithm that approximates pairwise terminal distances within a factor of $t - \varepsilon$ or an additive error $2t-3$ must use $\Omega(k^{1+1/(t-1)})$ bits. Our lower bound is inspired by the work of Matou{\v{s}}ek~\cite{matousek96}, which has also been utilized in the context of distance oracles~\cite{ThorupZ05}. Our arguments rely on the recent extremal combinatorics construction (see~\cite{cheung2016}) that was used to prove lower bounds on the size of distance approximating minors. 

\paragraph*{Discussion on our result.} Note that for any $k$-terminal graph $G$, if we do not have any restriction on the structure of the distance sparsifier, then $G$ always admits a trivial quality $1$ distance sparsifier $H$ which is the complete weighted graph on $k$ terminals with each edge weight being equal to the distance between the two endpoints in $G$. Furthermore, by the well-known result of Awerbuch~\cite{Awerbuch85}, such a graph $H$ in turn admits a multiplicative $(2t-1)$-\emph{spanner} $H'$ with $O(k^{1+1/t})$ edges, that is, all the distances in $H$ are preserved up to a multiplicative factor of $2t-1$ in $H'$, for any $t\geq 1$. This directly implies that the $k$-terminal graph $G$ has a quality $2t-1$ distance sparsifier with $k$ vertices and $O(k^{1+1/t})$ edges. On the other hand, though \emph{unconditional} lower bounds of type similar to our result have been known for the number of edges of spanners~\cite{lazebnik1995,Woodruff2006}, we are not aware of such lower bounds for the size of \emph{data structure} that preserves pairwise terminal distances for any $k$-terminal $n$-vertex graph when $k=o(n)$. In the extreme case when $k=n$ (i.e., all the vertices are terminals), the recent work by Abboud and Bodwin~\cite{abboudBodwin16} shows that any data structure that preserves the distances with an additive error $t$ needs $\Omega(n^{4/3-\varepsilon})$ bits, for any $\varepsilon>0, t=O(n^{\delta})$ and $\delta=\delta(\varepsilon)$ (see also the follow-up work~\cite{abboud2017}).

We start by reviewing a classical notion in combinatorial design.
\begin{definition} [Steiner Triple System] Given a ground set $T=[k]$, an $(3,2)$-Steiner system (abbr. $(3,2)$-\emph{SS}) of $T$ is a collection of $3$-subsets of $T$, denoted by $\mathcal{S} = \{S_1,\ldots,S_r\}$, where $r = \binom{k}{2}\left/3\right.$, such that every $2$-subset of $T$ is contained in \emph{exactly} one of the $3$-subsets.
\end{definition}

\begin{lemma}[\cite{Wilson75}] For infinity many $k$, the set $T=[k]$ admits an $(3,2)$-\emph{SS}.
\end{lemma}

Roughly speaking, our proof proceeds by forming a $k$-terminal bipartite graph, where terminals lie on one side and non-terminals on the other. The set of non-terminals will correspond to some subset of a Steiner Triple System $\mathcal{S}$, which will satisfy some \emph{certain} property. One can equivalently view such a graph as taking union over \emph{star} graphs. Before delving into details, we need to review a couple of other useful definitions and the construction from~\cite{cheung2016}. 

\paragraph*{\textbf{Detour Graph and Cycle.}} 
Let $k$ be an integer such that $T=[k]$ admits an $(3,2)$-SS. Let $\mathcal{S}$ be such an $(3,2)$-SS. We associate $\mathcal{S}=\{S_1,\ldots,S_r\}$ with a graph whose vertex set is $\mathcal{S}$. We refer to such graph as a \emph{detouring graph}.  By the definition of Steiner system, it follows that $|S_i \cap S_j|$ is either zero or one. Thus, two vertices $S_i$ and $S_j$ are adjacent in the detouring graph iff $|S_i \cap S_j|=1$. It is also useful to label each edge $(S_i, S_j)$ with the terminal in $S_i \cap S_j$. A \emph{detouring cycle} is a cycle in the detouring graph such that no two neighbouring edges in the cycles have the same terminal label. Observe that the detouring graph has other cycles which are not detouring cycles. 

Ideally, we would like to construct detouring graphs with long detouring cycles while keeping the size of the graph as large as possible. One trade-off is given in the following lemma.

\begin{lemma}[\cite{cheung2016}] \label{lemm: detouringGraph} For any integer $t \geq 3$, given a detouring graph with vertex set $\mathcal{S}$, there exists a subset $\mathcal{S}' \subset \mathcal{S}$ of cardinality $\Omega(k^{1+1/(t-1)})$ such that the induced graph on $\mathcal{S}'$ has no detouring cycles of size $t$ or less.
\end{lemma}

Now we are ready to prove our incompressibility result regarding approximately preserving terminal pairwise distances.
\paragraph*{\textbf{Proof of Theorem~\ref{thm:incompressibility}:}} 
Let $k$ be an integer such that $T=[k]$ admits an $(3,2)$-SS $\mathcal{S}$. Fix some integer $t \geq 3$, some positive constant $c$ and use Lemma \ref{lemm: detouringGraph} to construct a subset $\mathcal{S}'$ of $\mathcal{S}$ of size $\Omega(k^{1+1/(t-1)})$ such that the induced graph on $\mathcal{S}'$ has no detouring cycles of size $t$ or less. We may assume w.l.o.g. that $\ell = |\mathcal{S}'| = c \cdot k^{1+1/(t-1)}$ (this can be achieved by repeatedly removing elements from $\mathcal{S}'$, as the property concerning the detouring cycles is not destroyed). Fix some ordering among $3$-subsets of $\mathcal{S}'$ and among terminals in each $3$-subset.

We define the $k$-terminal graph $G$ as follows:
\begin{itemize}
\item For each $e_i \in \mathcal{S}'$ create a non-terminal vertex $v_i$. Let $V_{\mathcal{S}'}$ denote the set of such vertices. The vertex set of $G$ is $T \cup V_{\mathcal{S}'}$, where $T=[k]$ denotes the set of terminals.
\item For each $e_i \in \mathcal{S}'$, connect $v_i$ to the three terminals $\{x^{i}_{1},x^{i}_{2},x^{i}_{3}\}$ belonging to $e_i$, i.e., add edges $(v_i,x^{i}_j)$, $j=1,2,3$.
\end{itemize}
Note that $G$ is sparse since both the number of vertices and edges are $\Theta(\ell)$, and it also holds that $k=o(|V(G)|)$.

For any subset $R \subseteq \mathcal{S}'$, we define the subgraph $G_R=(V(G), E_R)$ of $G$ as follows. For each $e_i \in S'$, if $e_i \in R$, perform no changes. If $e_i \not \in R$, delete the edge $(v_i,x^{i}_1)$. Note that there are $2^{\ell}$ subgraphs $G_R$. We let $\mathcal{G}$ denote the family of all such subgraphs. 

We say a terminal pair $(x,x')$ \emph{respects $\mathcal{S'}$} if in the $(3,2)$-SS $\mathcal{S}$, the unique $3$-subset $e$ that contains $x$ and $x'$ belongs to $\mathcal{S'}$. Given $R \subseteq \mathcal{S}'$ and some terminal pair $(x,x')$, we say that $R$ \emph{covers} $(x,x')$ if both $x$ and $x'$ are connected to some non-terminal $v$ in $G_R$. 

\begin{claim}~\label{claim:cover} 
	For all $R \subseteq \mathcal{S}'$ and terminal pairs $(x,x')$ covered by $R$ we have that $\dist_{G_R}(x,x')=2$.
\end{claim}
\begin{proof}
By the definition of Steiner system and the construction of $G_R$, the shortest path between $x$ and $x'$ is simply a $2$-hop path, i.e., $\dist_{G_R}(x,x') = 2$. 
\end{proof}

\begin{claim}~\label{claim:non_cover}
For all $R \subseteq \mathcal{S}'$ and any terminal pair $(x,x')$ that respects $\mathcal{S}'$ and is \emph{not} covered by $R$, we have that $\dist_{G_R}(x,x')\geq 2t$.
\end{claim}
%\begin{claim} For all $R \subseteq \mathcal{S}'$ and $(x,x')$ be any terminal pair such that in the $(3,2)$-SS $\mathcal{S}$, the unique $3$-subset $e_i=(x^i_1,x^i_2,x^i_3)$ containing $x,x'$ belongs to $S'$, i.e., $e_i\in \mathcal{S'}$\footnote{\PP there also exists $(x,x')$ whose $e_i \in \mathcal{S}\setminus\mathcal{S'}$, which might have short paths in $G_R$. However, we do not need to consider such pairs.}. If $(x,x')$ is \emph{not} covered by $R$, then we have that $\dist_{G_R}(x,x') \geq 2t$.
%\end{claim}
\begin{proof}
%By the definition of $(3,2)$-SS, $x,x'$ are contained in exactly one $3$-subset $e_i\in \mathcal{S}$. Let we consider two cases. If $e_i\in \mathcal{S}'$, then b
Since $(x,x')$ respects $\mathcal{S'}$, there exists $e_i=(x^i_1,x^i_2,x^i_3)\in \mathcal{S}'$ that contains both $x$ and $x'$. By construction of $G_R$ and the fact that $(x,x')$ is not covered by $R$, it follows that $e_i\in \mathcal{S}'\setminus R$, and one of $x,x'$ corresponds to $x^i_1$ and the other corresponds to $x^i_2$ or $x^i_3$. W.l.o.g., we assume $x=x^i_1$ and $x'=x^i_2$. Note that there is no edge connecting $x^{i}_1$ with the non-terminal $v_i$ that corresponds to $e_i$. Now by Lemma~\ref{lemm: detouringGraph}, the detouring graph induced on $\mathcal{S}'$ has no detouring cycles of size $t$ or less, which implies that any other simple path between $x^{i}_1$ and $x^{i}_2$ in $G$ must pass through at least $t-1$ other terminals. Let $w_1,\ldots,w_{t-1}$ be such terminals and let $P:=x^{i}_1 \rightarrow w_1,\ldots,w_{t-1} \rightarrow x^{i}_2$ denote the corresponding path, ignoring the non-terminals along the path. Between any consecutive terminal pairs in $P$, the shortest path is at least $2$. Thus, the length of $P$ is at least $2t$, i.e., $\dist_{G_R}(x^{i}_1,x^{i}_2) \geq 2t$.
\end{proof}

Fix any two subsets $R_1, R_2 \subseteq \mathcal{S}'$ with $R_1 \neq R_2$. It follows that there exists a $3$-subset $e_i= (x^i_1,x^i_2,x^i_3)\in \mathcal{S}'$ such that either $e \in R_1 \setminus R_2$ or $e \in R_2 \setminus R_1$. Assume w.l.o.g that $e \in R_2 \setminus R_1$. Note that $(x^i_1,x^i_2)$ respects $\mathcal{S}'$ and it is covered in $R_2$ but not in $R_1$. By~Claim~\ref{claim:cover} and~\ref{claim:non_cover}, it holds that $\dist_{G_{R_{2}}}(x^i_1,x^i_2) = 2$ and $\dist_{G_{R_1}}(x^i_1,x^i_2) \geq 2t$. In other words, there exists a set $\mathcal{G}$ of $2^{\ell}$ different subgraphs on the same set of nodes $V(G)$ satisfying the following property: for any $G_1,G_2 \in \mathcal{G}$, there exists a terminal pair $(x,x')$ such that the distances between $x$ and $x'$ in $G_1$ and $G_2$ differ by at least a $t$ factor as well as by at least $2t-2$. On the other hand, for any compression function that approximates terminal path distances within a factor of $t-\varepsilon$ or an additive error $2t-3$ and produces a bitstring with less than $\ell$ bits, there exist two different graphs $G_1,G_2 \in \mathcal{G}$ that map to the same bit string. Hence, any such compression function must use at least $\Omega(\ell) = \Omega(k^{1+1/(t-1)})$ bits if we want to preserve terminal distances within a $t-\varepsilon$ factor or an additive error $2t-3$. 

%The above claims show that there exists a set $\mathcal{G}$ of $2^{\ell}$ different subgraphs on the same set of nodes $V(G)$ satisfying the following property: for any $G_1,G_2 \in \mathcal{G}$, there exists a terminal pair $(x,x')$ such that either $\dist_{G_1}(x,x') = 2$ and $\dist_{G_2}(x,x') \geq 2t$ or $\dist_{G_2}(x,x') = 2$ and $\dist_{G_1}(x,x') \geq 2t$. 





%Hence any compressing algorithm that approximates terminal path distances within a factor of $t-\varepsilon$ gives rise to a one-way protocol solving the \textsc{Index} problem. This implies that any compression algorithm must use $\Omega(\ell)=\Omega(k^{1+1/(t-1)})$, since otherwise it would contradict the communication complexity lower bound of Lemma \ref{lemm: commComp}.

To complete our argument, we need to show the claim for quality $t=2$. The only significant modification we need is the usage of an $(3,2)$-SS in the construction of graph $G$ (instead of using a subset of it). The remaining details are similar to the above proof and we omit them here. 

\section{Conclusion}















==> chapters/reachabilityminors/preliminary.tex <==
\section{Preliminaries} \label{sec: preli}
Let $G=(V,E)$ be a directed graph with terminal set $K \subset V$, $|K|=k$, which we will refer to as a \emph{$k$-terminal digraph}. We say $G$ is a \emph{$k$-terminal} DAG if $G$ has no directed cycles. The \emph{in-degree} of a vertex $v$, denoted by $\deg_{G}^{-}(v)$, is the number of edges directed towards $v$ in $G$. A digraph $H=(V',E')$, $K \subset V'$ is a (\emph{vertex}) \emph{reachability sparsifier} of $G$ if for any $x ,x' \in K$, there is a directed path from $x$ to $x'$ in $H$ iff there is a directed path from $x$ to $x'$ in $G$. If $H$ is obtained by performing minor operations in $G$, then we say that $H$ is a \emph{reachability-preserving minor} of $G$. We define the \emph{size} of $H$ to be the number of non-terminals in $H$, i.e. $|V' \setminus K|$. 


Let $G=(V,E,\cc)$ be an undirected graph with terminal set $K \subset V$ of
cardinality $k$, where $\cc: E \rightarrow \mathbb{R}_{\geq 0}$ assigns a non-negative
capacity to each edge. We will refer to such a graph as a \emph{k-terminal graph}. 
Let $U \subset V$ and $S \subset K$. We say that a cut $(U, V \setminus U)$ is
$S$-separating if it separates the terminal subset $S$ from its complement $K
\setminus S$, i.e., $U \cap K$ is either $S$ or $K \setminus S$. We will refer to such cut as a \emph{terminal cut}. The cutset
$\delta(U)$ of a cut $(U, V \setminus U)$ represents the edges that have one
endpoint in $U$ and the other one in $V \setminus U$. The cost
$\capacity_G(\delta(U))$ of a cut $(U, V \setminus U)$ is the sum over all
capacities of the edges belonging to the cutset. We let $\text{mincut}_{G}(S, K
\setminus S)$ denote the minimum cost of any $S$-separating cut of
$G$. A graph $H = (V', E', \cc')$, $K \subset V'$ is a \emph{quality-$q$} (\emph{vertex}) \emph{cut sparsifier} of $G$ with $q \geq 1$ if for any $S \subset K,
~ \mincut_G(S, K \setminus S) \leq \mincut_H(S, K \setminus S) \leq q \cdot
\mincut_G(S, K \setminus S).$





%We say that a (\textit{multi-commodity}) flow $f$ is a \textit{routing} of the
%demands $d$, if for every terminal pair $(x,x')$ it sends $d(x,x')$ units of
%flow from $x$ to $x'$. The \textit{congestion} of an edge $e \in E$ incurred by
%the flow $f$ is defined as the ratio of the total flow sent along the edge to
%the capacity of that edge, i.e., $f(e)/c(e)$. The \textit{congestion of the
%  flow} $f$ for routing demand $d$ is the maximum congestion over all edges in
%$G$. We let $\con_{G}(d)$ denote the minimum congestion over all flows. % In other words, $\con_{G}(d)$ is the minimum value by which we need to scale all edge capacities so we can find a \textit{feasible} flow that routes the demand vector $d$ in $G$.
%%\begin{definition} [Vertex Flow Sparsifiers] \label{2:defFlowSpars}
%A graph $H = (V', E', c_H)$, $K \subset V'$ is a \emph{vertex flow
%  sparsifier} of $G$ with \emph{quality} $q \geq 1$ if for every demand vector
%$d$, $\con_H(d) \leq \con_G(d) \leq q \cdot \con_H(d). $
%%\end{definition}

%In the above definitions we refer to $|V'|$ as the \textit{size} of the sparsifier $H$.


%We use the following tools about sparsifiers throughout the paper.
%\begin{lemma}[\cite{leighton}] \label{lemma: Moitra} If $H = (V', E', c_H)$, $V'=K$ is a
%  vertex flow sparsifier of $G$, then the quality of $H$ is $q =
%  \con_{G}(d_{H})$, where $d_{H}(x,x') : = c_{H}(x,x')$ for all terminal pairs
%  $(x,x')$.
%\end{lemma}
%Let $G_1$ and $G_2$ be graphs on \textit{disjoint} set of vertices with
%terminals $K_1 = \{s_1,\ldots,s_k\}$ and $K_2 = \{t_1,\ldots,t_m\}$,
%respectively. In addition, let $\phi(s_i) = t_i$, for all $i =1,\ldots,\ell$,
%be a one-to-one correspondence between some subset of $K_1$ and $K_2$. The
%$\phi$-\emph{merge} (or $2$-\textit{sum}) of $G_1$ and $G_2$ is the graph $G$
%with terminal set $K = K_1 \cup \{t_{\ell+1},\ldots,t_m\}$ formed by
%identifying the terminals $s_i$ and $t_i$ for all $i = 1,\ldots, \ell$. This
%operation is denoted by $G := G_1 \oplus_{\phi} G_2$.
%\begin{lemma}[\cite{andoni}, Merging] \label{lemma: Merging} Let $G = G_1 \oplus_{\phi} G_2$.
%  Suppose $G_1'$ and $G_2'$ are flow sparsifiers of quality $q_1$ and $q_2$ for
%  $G_1$ and $G_2$, respectively. Then $G' = G_1' \oplus_{\phi} G_2'$ is a flow
%  sparsifier of quality $\max\{q_1, q_2\}$ for $G$.
%\end{lemma} 
%\begin{lemma}[Convex Combination of Sparsifiers] \label{lemma: ConvexComb} Let
%  $H_i = (V^{*},E_i, c_i)$, $i = 1, \ldots, m$ with $K \subset V^{*}$ be vertex
%  flow sparsifiers of $G$. In addition, let $\alpha_1, \alpha_2, ..., \alpha_m$
%  be convex multipliers corresponding to $H_i$'s such that $\sum_{i} \alpha_i =
%  1$. Then the graph $H' = \sum_{i} \alpha_i \cdot H_i $ is a vertex flow
%  sparsifier for $G$.
%\end{lemma}
%\vspace{-0.4cm}











%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> chapters/reachabilityminors/reachability.tex <==
\section{An Exact Cut Sparsifier of Size $O(k^2)$} \label{sec: upperCut}
In this section we show that given a $k$-terminal planar graph, where all terminals lie on the same face, one can construct a quality-$1$ cut sparsifier of size $O(k^{2})$. Note that it suffices to consider the case when all terminals lie on the \emph{outer} face. %Our approach closely follows the work of Gitler~\cite{Gitler91} in the context of Wye-Delta reducibility of graphs, which does not consider preservation of terminal cuts. Apart from bringing his work to the vertex sparsification community, we also fill in some gaps and provide the necessary details for applying his technique to the cut setting.
%The basic approach is as follows. Given a $k$-terminal planar graph with terminals lying on the outer face, we first embed it into some large grid with terminals lying on the boundary of the grid. Subsequently, we show how to embed the resulting grid into a `more suitable' graph, which we will refer to as `half-grid'. Finally, using the Wye-Delta operations, we reduce 'half-grid'  into another graph whose number of vertices can be bounded by $O(k^{2})$. Since we shall argue that the above graph reductions preserve exactly all terminal minimum cuts, our result follows. 
%\vspace{-0.4cm}
We first present some basic tools. 
\subsection{Basic Tools}
\paragraph*{Wye-Delta Transformations. }
In this section we investigate the applicability of some graph reduction techniques that aim at reducing the number of non-terminals in a $k$-terminal graph. %Khan and Raghavendra~\cite{KhanR14} were the first to apply such techniques in the context of Vertex Cut Sparsification for tree networks. 
We start by reviewing the so-called \emph{Wye-Delta} operations in graph reductions. These operations consist of five basic rules, which we describe below. (See Fig.~\ref{fig:wyedelta} for illustrations.)%It is easy to see that each of these rules preserve exactly all terminal cuts if appropriate edge weights are used on the reduced graph. 
\begin{enumerate}
	\setlength\itemsep{0.1em}
	\item \emph{Degree-one reduction:} Delete a degree-one non-terminal and its incident edge.
	\item \emph{Series reduction:} Delete a degree-two non-terminal $y$ and its incident edges $(x,y)$ and $(y,z)$, and add a new edge $(x,z)$ of capacity $\min\{\cc(x,y), \cc(y,z)\}$.
	\item \emph{Parallel reduction:} Replace all parallel edges by a single edge whose capacity is the sum over all capacities of parallel edges.
	\item \emph{Wye-Delta transformation:} Let $x$ be a degree-three non-terminal with neighbours $\delta(x) = \{u,v,w\}$. Assume w.l.o.g.\footnote{Suppose there exist a pair $(u,v) \in \delta(x)$ with $\cc(u,x) + \cc(v,x) < \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. Then we can simply set $\cc(w,x) = \cc(u,x) + \cc(v,x)$, since any terminal minimum cut would cut the edges $(u,x)$ and $(v,x)$ instead of the edge $(w,x)$.} that for any pair $(u,v) \in \delta(x)$, $\cc(u,x) + \cc(v,x) \geq \cc(w,x)$, where $w \in \delta(v)\setminus \{u,v\}$. Then we can delete $x$ (along with all its incident edges) and add edges $(u,v),(v,w)$ and $(w,u)$ with capacities $(\cc(u,x)+\cc(v,x)-\cc(w,x))/2$, $(\cc(v,x)+\cc(w,x)-\cc(u,x))/2$ and $(\cc(u,x)+\cc(w,x)-\cc(v,x))/2$, respectively. 
	\item \emph{Delta-Wye transformation:} Delete the edges of a triangle connecting $x$, $y$ and $z$, introduce a new non-terminal vertex $w$ and add new edges $(w,x)$, $(w,y)$ and $(w,z)$ with edge capacities $\cc(x,y) + \cc(x,z),$ $\cc(x,y) + \cc(y,z)$ and $\cc(x,z) + \cc(y,z)$ respectively.
\end{enumerate}

\input{chapters/reachabilityminors/figure_wyeDeltaTrans}

The following lemma (which follows from the above definitions) shows that the above rules preserve exactly all terminal minimum cuts.


\begin{lemma} \label{lemm: rules} Let $G$ be a $k$-terminal graph and $G'$ be a $k$-terminal graph obtained from $G$ by applying one of the rules $1-5$. Then $G'$ is a quality-$1$ cut sparsifier of $G$.
\end{lemma}

For our application, it will be useful to enrich the set of rules by introducing two new operations. These operations can be realized as series of the operations 1-5. (See Fig.~\ref{fig:edgedeletion} and \ref{fig:edgereplacement} for illustrations.)
\begin{enumerate}[resume]
	\item \emph{Edge deletion (with vertex $x$):} For a degree-three non-terminal with neighbours $u,v$, the edge $(u,v)$ can be deleted, if it exists. To achieve this, we use a Delta-Wye transformation followed by a series reduction.
	
	
	
	\item \emph{Edge replacement:} For a degree-four non-terminal vertex with neighbours $x,u,v,w$, if the edge $(x,u)$ exists, then it can be replaced by the edge $(v,w)$. To achieve this, we use a Delta-Wye transformation followed by a Wye-Delta transformation.
\end{enumerate}

\input{chapters/reachabilityminors/figure_edgeDeletion}
\input{chapters/reachabilityminors/figure_edgeReplacement}

A $k$-terminal graph $G$ is \emph{Wye-Delta} reducible to another $k$-terminal graph $H$, if $G$ is reduced to $H$ by repeatedly applying one of the operations 1-7. %We obtain the following lemma, whose proof we defer to Appendix~\ref{app: preli}.


\begin{lemma} \label{lemm: cutReducability} Let $G$ and $H$ be $k$-terminal graphs. Moreover, let $G$ be Wye-Delta reducible to $H$. Then $H$ is a quality-$1$ cut sparsifier of $G$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: cutReducability}]
	Observe that the rules 1-7 do not affect any terminal vertex and each rule preserves exactly all terminal minimum cuts by Lemma \ref{lemm: rules}. An induction on the number of rules needed to reduce $G$ to $H$ proves the claim.
\end{proof}
%\begin{proof}
%Observe that the rules 1-7 do not affect any terminal vertex and each rule preserves exactly all terminal minimum cuts by Lemma \ref{lemm: rules}. An induction on the number of rules needed to reduce $G$ to $H$ proves the claim.
%\end{proof}
%\vspace{-0.5cm}
\paragraph*{Grid Graphs.} %Throughout the paper we will be dealing with two special types of graphs. 
A \emph{grid} graph is a graph with $n \times n$ vertices $\{(u,v) : u,v = 1,\ldots, n\}$, where $(u,v)$ and $(u',v')$ are adjacent if $|u' -u| + |v'-v| = 1$. For $k < n$, a \emph{half-grid} graph with $k$ terminals is a graph $T^{n}_k = (V,E)$ with $K \subset V$ and $n(n+1)/2$ vertices $\{(i,j) : i \leq j \text{ and } i,j=1,\ldots,n  \}$, where $(i,j)$ and $(i',j')$ are connected by an edge if $|i'-i| + |j'-j| = 1$, and additional diagonal edges between $(i,i)$ and $(i+1,i+1)$ for $i = 1,\ldots, n-1$. Moreover, each terminal vertex in $T^{n}_k$ must be one of its diagonal vertices, i.e., every $x \in K$ is of the form $(m,m)$ for some $m \in \{1,\ldots,n\}$. Let $\hat{T}^{n}_{k}$ be the same graph as $T^{n}_k$ but excluding the diagonal edges. 

\paragraph*{Graph Embeddings.}\label{sec: graphEmbeddings} 
Throughout this chapter, we will be dealing with the embedding of a planar graph into a square \emph{grid} graph. One way of drawing graphs in the plane are \emph{orthogonal grid-embeddings}~\cite{Valiant81}. In such a setting, the vertices correspond to distinct points and edges consist of alternating sequences of vertical and horizontal segments. Equivalently, one can view this as drawing our input graph as a subgraph of some grid. Formally, a \emph{node-embedding} $\rho$ of $G_1=(V_1,E_1)$ into $G_2=(V_2,E_2)$ is an injective mapping that maps $V_1$ into $V_2$, and $E_1$ into paths in $G_2$, i.e., $(u,v)$ maps to a path from $\rho(u)$ to $\rho(v)$, such that every pair of paths that correspond to two different edges in $G_1$ is vertex-disjoint (except possibly at the endpoints). If $G_2$ is a planar graph, then $\rho(G_1)$ and $G_1$ are also planar. Thus, if $G_1$ and $G_2$ are planar we then refer to $\rho$ as an \emph{orthogonal embedding}. Moreover, given a planar graph $G_1$ drawn in the plane, the embedding $\rho$ is called \emph{region-preserving} if $\rho(G_1)$ and $G_1$ have the same planar topological embedding.

%\input{figure_orthogonalEmbedding}

%We know turn our attention to the case when 
Let $G_1$ be a $k$-terminal graph. Since the embedding does not affect the vertices of $G_1$, the terminals of $G_1$ are also terminals in $\rho(G_1)$. Although the embedding does not consider capacity of the edges in $G_1$, we can still guarantee that such an embedding preserves all terminal minimum cuts, for which we make use of the following operation:
\begin{enumerate}
	\item \emph{Edge subdivision: } Let $(u,v)$ be an edge of capacity $\cc(u,v)$. Delete $(u,v)$, introduce a new vertex $w$ and add edges $(u,w)$ and $(w,v)$, each of capacity $\cc(u,v)$. 
\end{enumerate}

The following lemma shows that a node-embedding is a cut preserving mapping.
%The proof of the following Lemma is deferred to Appendix~\ref{app: preli}.
\begin{lemma} \label{lemm: cutembedding}
	Let $\rho$ be a node-embedding and let $G_1$ and $\rho(G_1)$ be $k$-terminal graphs defined as above. Then $\rho(G_1)$ preserves exactly all terminal minimum cuts of $G$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: cutembedding}]
	We can view each path obtained from the embedding as taking the edge corresponding to the path endpoints in $G_1$ and performing edge subdivisions finitely many times. We claim that such subdivisions preserve all terminal cuts. 
	
	Indeed, let us consider a single edge subdivision for $(u,v)$ (the general claim then follows by induction on the number of edge subdivisions). Fix $S \subset K$ and consider some $S$-separating minimum cut $(U,V \setminus U)$ in $G_1$ cutting $(u,v)$. Then, in the transformed graph $\rho(G_1)$, we can simply cut either the edge $(u,w)$ or $(w,v)$. Since by construction, the new edge has the same capacity as the subdivided edge, we get that $\capacity_{\rho(G_1)}(\delta(U)) = \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \leq \mincut_{G_1}(S,K \setminus S)$. 
	
	Furthermore, since $G_1$ is obtained by contracting two edges of the same capacity of $\rho(G_1)$, for any $S$-separating minimum cut $(U, V \setminus U)$ in $\rho(G_1)$, we have $\capacity_{\rho(G_1)}(\delta(U)) \geq \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \geq \mincut_{G_1}(S,K \setminus S)$. Combining the above gives the lemma. 
\end{proof}
%\begin{proof}
%We can view each path obtained from the embedding as taking the edge corresponding to the path endpoints in $G_1$ and performing edge subdivisions finitely many times. We claim that such subdivisions preserve all terminal cuts. 
%
%Indeed, let us consider a single edge subdivision for $(u,v)$ (the general claim then follows by induction on the number of edge subdivisions). Fix $S \subset K$ and consider some $S$-separating minimum cut $(U,V \setminus U)$ in $G_1$ cutting $(u,v)$. Then, in the transformed graph $\rho(G_1)$, we can simply cut either the edge $(u,w)$ or $(w,v)$. Since by construction, the new edge has the same capacity as the subdivided edge, we get that $\capacity_{\rho(G_1)}(\delta(U)) = \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \leq \mincut_{G_1}(S,K \setminus S)$. 
%
%Furthermore, since $G_1$ is obtained by contracting two edges of the same capacity of $\rho(G_1)$, for any $S$-separating minimum cut $(U, V \setminus U)$ in $\rho(G_1)$, we have $\capacity_{\rho(G_1)}(\delta(U)) \geq \capacity_{G_1}(\delta(U))$, and in particular $\mincut_{\rho(G_1)}(S,K \setminus S) \geq \mincut_{G_1}(S,K \setminus S)$. Combining the above gives the lemma. 
%\end{proof}
\subsection{Our Construction}
In this section  we construct our exact cut sparsifier and prove that any planar $k$-terminal graph with all terminals lying on the same face admits a cut sparsifier of size $O(k^2)$ that is also planar.
\subsubsection{Embedding into Grids} \label{EmbeddingGrid}

It is well-known that one can obtain an orthogonal embedding of a planar graph with maximum-degree at most three into a grid (see Valiant~\cite{Valiant81}). However, our input planar graph can have arbitrarily large maximum degree. In order to be able to make use of such an embedding, we need to first reduce our input graph to a bounded-degree graph while preserving planarity and all terminal minimum cuts. We achieve this by making use of a \emph{vertex splitting} technique, which we describe below. 

Given a $k$-terminal planar graph $G'=(V',E',c')$ with $K \subset V'$ lying on the outer face, vertex splitting produces a $k$-terminal planar graph $G=(V,E,c)$ with $K \subset V$ such that the maximum degree of $G$ is at most three. Specifically, for each vertex $v$ of degree $d>3$ with neighboring vertices $u_1,\ldots,u_{d}$, we delete $v$ and introduce new vertices $v_1, \ldots, v_d$ along with edges $\{(v_i,v_{i+1}) : i=1,\ldots,d-1\}$, each of capacity $C+1$, where $C=\sum_{e \in E'} c'(e)$. Further, we replace the edges $\{(u_i,v) : i = 1,\ldots,d\}$ with $\{(u_i,v_i) : i = 1,\ldots,d\}$, each of corresponding capacity. If $v$ is a terminal vertex, we set one of the $v_i$'s to be a terminal vertex. It follows that the resulting graph $G$ is planar and terminals can be still embedded on the outer face. Note that while the degree of every vertex $v_i$ is at most $3$, the degree of any other vertex is not affected. %The proof of the claim below appears in Appendix~\ref{app: upperCut}.

\begin{claim} \label{claim: embedding}
Let $G'$ and $G$ be $k$-terminal graphs defined as above. Then $G$ preserves exactly all minimum terminal cuts of $G'$, i.e., $G$ is a quality-$1$ cut sparsifier of $G'$.
\end{claim} 
\begin{proof}%[Proof of Claim \ref{claim: embedding}]
	It suffices to prove the case where $G$ is obtained from $G'$ by a single vertex splitting. Then the claim follows by induction on the number of vertex splittings required to transform $G'$ to $G$.
	
	Let $S \subset K$ and $(U, V \setminus U)$ be an $S$-separating cut in $G$ of size $\mincut_G(S,K \setminus S)$. Suppose towards contradiction that $\delta(U)$ contains an edge of the form $(v_j,v_{j+1})$, for some $j$, which in turn gives that $\capacity(\delta(U)) \geq C + 1$. Then we can move all the points $v_i$ to one of the sides of the cut $(U, V \setminus S)$ and obtain a new $S$-separating cut in $G$ of cost at most $C$, contradicting the fact that $(U, V \setminus U)$ is a minimum terminal cut. Hence, it follows that $\delta(U)$ uses either edges that are in both $G$ and $G'$ or edges of the form $(u_i,v_i)$, which by construction have the same capacity as the edges $(u_i,v)$ in $G'$. Thus, an $S$-separating minimum cut in $G$ corresponds to an $S$-separating minimum cut in $G'$ of the same cost. Since $S$ is chosen arbitrarily, the claim follows.
\end{proof}
%\begin{proof}
%It suffices to prove the case where $G$ is obtained from $G'$ by a single vertex splitting. Then the claim follows by induction on the number of vertex splittings required to transform $G'$ to $G$.
%
%Let $S \subset K$ and $(U, V \setminus U)$ be an $S$-separating cut in $G$ of size $\mincut_G(S,K \setminus S)$. Suppose towards contradiction that $\delta(U)$ contains an edge of the form $(v_j,v_{j+1})$, for some $j$, which in turn gives that $\capacity(\delta(U)) \geq C + 1$. Then we can move all the points $v_i$ to one of the sides of the cut $(U, V \setminus S)$ and obtain a new $S$-separating cut in $G$ of cost at most $C$, contradicting the fact that $(U, V \setminus U)$ is a minimum terminal cut. Hence, it follows that $\delta(U)$ uses either edges that are in both $G$ and $G'$ or edges of the form $(u_i,v_i)$, which by construction have the same capacity as the edges $(u_i,v)$ in $G'$. Thus, an $S$-separating minimum cut in $G$ corresponds to an $S$-separating minimum cut in $G'$ of the same cost. Since $S$ is chosen arbitrarily, the claim follows.
%\end{proof}

Let $G=(V,E)$ be a $k$-terminal graph obtained by vertex splitting of all vertices of degree larger than $3$ of $G'=(V',E')$. Further, let $n' = |V'|$, $m' = |E'|$, $n = |V|$ and $m = |E|$. Then it is easy to show that $n \leq 2 m'$ and $m \leq m' + n \leq 3m'$. Since $G'$ is planar, we have that $n = O(n')$ and $m = O(n')$. Thus, by just a linear blow-up on the size of vertex and edge sets, we may assume w.l.o.g. that our input graph is a planar graph of degree at most three. 

Valiant~\cite{Valiant81} and Tamassia et al.~\cite{TamassiaT89} showed that a $k$-terminal planar graph $G$ with $n$ vertices and degree at most three admits an orthogonal region-preserving embedding into some square grid of size $O(n) \times O(n)$. By Lemma \ref{lemm: cutembedding}, we know that the resulting graph exactly preserves all terminal minimum cuts of $G$. We remark that since the embedding is region-preserving, the outer face of the input graph is embedded to the outer face of the grid. Therefore, all terminals in the embedded graph lie on the outer face of the grid. Performing appropriate edge subdivisions, we can make all the terminals lie on the boundary of some possibly larger grid. Further, we can add dummy non-terminals and zero edge capacities to transform our graph into a full-grid $H$. We observe that the latter does not affect any terminal min-cut. The above leads to the following:
\begin{lemma} \label{lemm: embeddingGrids}
Given a $k$-terminal planar graph $G$, where all terminals lie on the outer face, there exists a $k$-terminal grid graph $H$, where all terminals lie on the boundary such that $H$ preserves exactly all terminal minimum cuts of $G$. The resulting graph has $O(n^2)$  vertices and edges.
\end{lemma}

%\vspace{-0.3cm}
\subsubsection{Embedding Grids into Half-Grids}

Next, we show how to embed square grids into half-grid graphs (see Section \ref{sec: preli_RM}), which will facilitate the application of Wye-Delta transformations. The existence of such an embedding was claimed in the thesis of Gitler~\cite{Gitler91}, but no details on its construction were given. 

Let $G$ be a $k$-terminal square grid on $n \times n$ vertices where terminals lie on the boundary of the grid. We obtain the following:
%\input{figure_halfgrid}
\begin{figure}[t] 
\begin{center}
\includegraphics[scale=1]{chapters/reachabilityminors/fhalfgrid}
\end{center}
\caption{Embedding grid into half-grid. Black vertices represent terminals while white vertices represent non-terminals. The counter-clockwise ordering starts at the top right terminal. Coloured edges and paths correspond to the mapping of the respective edges: blue for edges $((i,1),(i,2))$, red for edges $((n-1,j),(n,j))$, green for edges $((1,j),(2,j))$ and yellow for edges $((i,n-1), (i,n))$, where $i,j = 2,\ldots,n-1$. }
\label{fig: halfgridConst}
\end{figure}

\begin{lemma} \label{lemm: embeddingHalfGrid}
There exists a node embedding of the grid $G$ into $T^{\ell}_{k}$, where $\ell  = 4n-3$. 
\end{lemma}
\begin{proof}
Our construction works as follows (See Fig.~\ref{fig: HalfGridRed} for an example). We first fix an ordering on the vertices lying on the boundary of the grid in the order induced by the grid. Then we embed each vertex according to that order into the diagonal vertices of the half-grid, along with the edges that form the boundary of the grid. The sub-grid obtained by removing all boundary vertices is embedded appropriately into the upper-part of the half-grid. Finally, we show how to embed edges between the boundary and the sub-grid vertices and argue that such an embedding is indeed vertex-disjoint for any pair of paths.

\input{chapters/reachabilityminors/figure_halfgridReduction}

We start with the embedding of the vertices of $G$. Let us first consider the boundary vertices. The ordering imposed on these vertices can be viewed as starting with the upper-right vertex $(1,n)$ and visiting the rest of vertices in a counter-clockwise direction until reaching the vertex $(2,n)$. We map the vertices on the boundary as follows.
\begin{enumerate}
\setlength\itemsep{0.1em}
\item The vertex $(1,j)$ is mapped to the vertex $(n-j+1,n-j+1)$ for $j=2,\ldots,n$, 
\item The vertex $(i,1)$ is mapped to the vertex $(n+i-1,n+i-1)$ for $i=1,\ldots,n-1$,
\item The vertex $(n,j)$ is mapped to the vertex $(2n+j-2,2n+j-2)$ for $j=1,\ldots,n-1$,
\item The vertex $(i,n)$ is mapped to the vertex $(4n-i-2,4n-i-2)$  for $i=2,\ldots,n$.
\end{enumerate} 
Now we consider the vertices that belong to the induced sub-grid $S$ of $G$ of size $(n-2)^2$ when removing the boundary vertices of our input grid. We map the vertex $(i,j)$ to the vertex $(n+i-1, 2n+j-2)$ for $i,j=2,\ldots,n-1$. In other words, for every vertex of $S$ we make a vertical shift by $n-1$ units and an horizontal shift by $2n-2$ units. By construction, it is not hard to check that every vertex of $G$ is mapped to a different vertex of $T^{\ell}_{k}$ and all terminal vertices lie on the diagonal of $T^{\ell}_{k}$. 

We continue with the embedding of the edges of $G$. First, every edge between two boundary vertices in $G$ is embedded to the edge between the corresponding mapped diagonal vertices of $T^{\ell}_{k}$, except the edge between $(1,n)$ and $(2,n)$. For this edge, we define an edge embedding between the corresponding vertices $(1,1)$ and $(4n-4,4n-4)$ of $T^{\ell}_{k}$ by using the path:
\begin{align*} 
(1,1) \rightarrow (1,2) \rightarrow \ldots & \rightarrow (1,4n-3) \rightarrow (2,4n-3)  \\ 
&\rightarrow \ldots \rightarrow (4n-4,4n-3) \rightarrow (4n-4,4n-4).
\end{align*}

Next, every edge of the sub-grid $S$ is embedded in to the edge connecting the mapped endpoints of that edge in $T^{\ell}_{k}$. In other words, if $(i,j)$ and $(i',j')$ were connected by an edge $e$ in $S$, then $(n+i-1, 2n+j-2)$ and $(n+i'-1, 2n+j'-2)$ are connected by an edge $e'$ in $T^{\ell}_{k}$ and $e$ is mapped to $e'$. Finally, the only edges that remain are those connecting a boundary vertex of $G$ with a boundary vertex of $S$. We distinguish four cases depending on the edge position. 
\begin{enumerate}
\setlength\itemsep{0.1em}
\item The edge $((i,2), (i,1))$ is mapped to the horizontal path given by:
\begin{align*}
	(n+i-1,2n) & \rightarrow (n+i-1, 2n-1) \\ 
	& \rightarrow \ldots \rightarrow (n+i-1,n+i-1) \text{ for } i = 2,\ldots,n-1 
\end{align*}
\item The edge $((n-1,j), (n,j))$ is mapped to the vertical path given by:
\begin{align*}
	(2n-2,&~2n+j-2)  \rightarrow (2n-1, 2n+j-2) \\
	& \rightarrow \ldots \rightarrow (2n+j-2,2n+j-2) \text{ for } j = 2,\ldots,n-1.
\end{align*}
\item The edge $((2,j), (1,j))$ is mapped to the $L$-shaped path:
\begin{align*}
	(n+1,2n+&j-2)  \rightarrow (n, 2n+j-2) \rightarrow \ldots \rightarrow (n-j+1,2n+j-2) \\
	&  \rightarrow (n-j+1,2n+j-3)  \rightarrow \ldots \rightarrow (n-j+1,n-j+1) \\
	& \text{ for } j = 2,\ldots,n-1.
\end{align*}

\item The edge $((i,n-1), (i,n))$ is mapped to the $L$-shaped path:
\begin{align*}
	(n+i-1,3n&-3)  \rightarrow (n+i-1, 3n-2) \rightarrow \ldots \rightarrow (n+i-1,4n-i-2) \\
	&  \rightarrow (n+i,4n-i-2)  \rightarrow \ldots \rightarrow (4n-i-2,4n-i-2) \\
	& \text{ for } i = 2,\ldots,n-1.
\end{align*}
\end{enumerate} 
By construction, it follows that the paths in our edge embedding are vertex disjoint.
\end{proof}

%\vspace{-0.3cm}
\subsubsection{Reducing Half-Grids and Bringing the Piece Together}
We now review the construction of Gitler~\cite{Gitler91}, which shows how to reduce half-grids to much smaller half-grids (excluding diagonal edges) whose size depends only on $k$. For the sake of completeness, we provide a full proof here. Recall that $\hat{T}^{n}_{k}$ is the graph $T^{n}_k$ without the diagonal edges. 

\begin{lemma}[\cite{Gitler91}] \label{lemm: Gitler}
For any positive $k,n$ with $k<n$, $T^{n}_k$ is Wye-Delta reducible to $\hat{T}^{k}_{k}$.
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lemm: Gitler}]
	For sake of simplicity, we assume w.l.o.g that the four vertices $(1,1)$, $(2,2)$, $(n-1,n-1)$ and $(n,n)$ are terminals\footnote{If they are not terminals, we can simply define them as terminals, thus increasing the number of terminals to $k+4 = O(k)$.}. Furthermore, we say that two terminals $(i,i)$ and $(j,j)$ are \textit{adjacent} iff $i<j$ and there is no terminal $(\ell,\ell)$ such that $i < \ell < j$. 
	
	We next describe the reduction procedure. Also see Fig.~\ref{fig: HalfGridRed} for an example. The reduction procedure starts by removing the diagonal edges of $T^{n}_k$, thus producing the graph $\hat{T}^{n}_k$ . Specifically, the two edges $((1,1),(2,2))$ and $((n-1,n-1), (n,n))$ are removed using an edge deletion operation. For each remaining diagonal edge of the form $((i,i), (i+1,i+1))$, $i=2,\ldots,n-2$ we repeatedly apply an edge replacement operation until the edge is incident to a boundary vertex $(1,j)$ or $(j,n)$ of the grid, where an edge deletion operation with one of the neighbours of $(1,j)$ resp. $(j,n)$ as vertex $x$ is applied.
	
	Now, we know that all non-terminals of the form $(i,i)$ are degree-two vertices, thus a series reduction is applied on each of them. This produces new diagonal edges, which are effectively reduced by the above procedure. We keep removing the newly-created degree-two non-terminal vertices and the newly-created edges until no further removals are possible. At this point, the only degree-$2$ vertices are terminal vertices. 
	%we arrive at a degree-four non-terminal $(i,j)$, for which the vertex $(i,i)$ on the same row and $(j,j)$ on the same column are terminals. 
	
	%The above vertex and edge removals could also produce degree-two vertices on the boundary of the half-grid, i.e., vertices of the form $(1,j)$ or $(i,n)$, excluding $(1,n)$. We apply a series reduction on every non-terminal of such form. 
	The resulting graph has a staircase structure, where for every pair of adjacent terminals $(i,i)$ and $(j,j)$, there is a non-terminal $(i,j)$ of degree three or four, namely, the intersection vertex, and a (possibly empty) sequence of degree-three non-terminals that lie on the boundary path from $(i,i)$ to $(j,j)$. For $k = i+1,\ldots,j-1$, let $(i,k)$ and $(k,j)$ be the degree-three non-terminals lying on the row and the column subpath, respectively. Additionally, for $k = i+1,\ldots,j-1$, let $C^{i}_{k}=\{(i',k) : i'=i,\ldots,1\}$, resp. $R^{j}_{k}=\{(k,j') : j'=j,\ldots,n\}$ be the vertices sharing the same column, resp. row with $(i,k)$, resp. $(k,j)$. We next show that the vertices belonging to $C^{i}_{k}$ and $R^{j}_{k}$ can be removed. 
	
	The removal process works as follows. For $k=i+1,\ldots,j-1$, we start by choosing a degree $3$ vertex $(i,k)$ and its corresponding column $C^{i}_{k}$. Then we apply a Wye-Delta transformation on $(i,k)$, thus creating two new diagonal edges. Similarly as above, we remove such edges by repeatedly applying an edge replacement operation until they have been pushed to the boundary of the grid, where an edge deletion operation is applied. In the resulting graph, the vertex $(i-1,k) \in C^{i}_{k}$ is now a degree-three non-terminal. We apply the same procedure to this vertex. Applying such a procedure to all remaining vertices of $C^{i}_{k}$, we eliminate a column of the grid. Symmetrically, the same process applies to the case when we want to remove the row $R^{j}_{k}$ corresponding to the vertex $(k,j)$.
	
	Applying the above removal process for every adjacent terminal pair and the corresponding degree-three non-terminals, we end up with the graph $\hat{T}^{k}_{k}$, where every diagonal vertex is a terminal. By definition, it follows that $\hat{T}^{k}_{k}$ has at most $O(k^2)$ vertices.
\end{proof}

Combining the above reductions leads to the following theorem:
\begin{theorem} \label{thm: CutSparsifier}
Let $G$ be a $k$-terminal planar graph where all terminals lie on the outer face. Then $G$ admits a quality-$1$ cut sparsifier of size $O(k^{2})$, which is also a planar graph.
\end{theorem}
\begin{proof}
Let $n$ denote the number of vertices in $G$. First, we apply Lemma \ref{lemm: embeddingGrids} on $G$ to obtain a grid graph $H$ with $O(n^{2})$ vertices, which preserves exactly all terminal minimum cuts of $G$. We then apply Lemma \ref{lemm: embeddingHalfGrid} on $H$ to obtain a node embedding $\rho$ into the half-grid $T^{\ell}_{k}$, where $\ell = 4n-3$. By Lemma \ref{lemm: cutembedding}, $\rho(H)$ preserves exactly all terminal minimum cuts of $H$. We can further extend $\rho(H)$ to the full half-grid $T^{\ell}_{k}$, if dummy non-terminals and zero edge capacities are added. Finally, we apply Lemma \ref{lemm: Gitler} on $T^{\ell}_{k}$ to obtain a Wye-Delta reduction to the reduced half-grid graph $\hat{T}^{k}_{k}$. It follows by Lemma \ref{lemm: cutReducability} that $\hat{T}^{k}_{k}$ is a quality-$1$ cut sparsifier of $T^{\ell}_{k}$, where the size guarantee is immediate from the definition of $\hat{T}^{k}_{k}$.
\end{proof}
